Spitzer IRS 16 micron Observations of the GOODS Fields

We present Spitzer 16 micron imaging of the Great Observatories Origins Deep Survey (GOODS) fields. We survey 150 square arcminutes in each of the two GOODS fields (North and South), to an average 3 sigma depth of 40 and 65 micro-Jy respectively. We detect about 1300 sources in both fields combined. We validate the photometry using the 3-24 micron spectral energy distribution of stars in the fields compared to Spitzer spectroscopic templates. Comparison with ISOCAM and AKARI observations in the same fields show reasonable agreement, though the uncertainties are large. We provide a catalog of photometry, with sources cross correlated with available Spitzer, Chandra, and HST data. Galaxy number counts show good agreement with previous results from ISOCAM and AKARI, with improved uncertainties. We examine the 16 to 24 micron flux ratio and find that for most sources it lies within the expected locus for starbursts and infrared luminous galaxies. A color cut of S_{16}/S_{24}>1.4 selects mostly sources which lie at 1.1<z<1.6, where the 24 micron passband contains both the redshifted 9.7 micron silicate absorption and the minimum between PAH emission peaks. We measure the integrated galaxy light of 16 micron sources, and find a lower limit on the galaxy contribution to the extragalactic background light at this wavelength to be 2.2\pm 0.2$ nW m^{-2} sr^{-1}.

==> Table1_data.tex <==
         0 &      189.319641 &       62.390766 &         11 &      84.80 &       4.24 &      60.40 &       3.02 &      55.20 &       2.94 &      40.20 &       2.16 &      145.1 &       11.3 &      225.0 &        5.5 \\
         1 &      189.310349 &       62.388977 &         12 &      11.50 &       0.58 &      14.50 &       0.73 &      19.00 &       1.50 &      12.90 &       0.99 &       55.3 &       10.4 &      200.0 &        5.7 \\
         2 &      189.326126 &       62.383057 &         20 &      38.30 &       1.92 &      49.10 &       2.46 &      55.30 &       2.83 &      39.30 &       2.06 &      107.2 &       16.5 &      483.0 &        5.7 \\
         3 &      189.294266 &       62.376274 &         20 &      40.00 &       2.00 &      47.50 &       2.38 &      39.60 &       2.11 &      44.20 &       2.30 &      240.4 &       11.5 &      386.0 &        4.9 \\
         4 &      189.330811 &       62.375191 &         24 &      10.10 &       0.51 &       6.98 &       0.36 &       7.48 &       0.63 &       6.27 &       0.63 &       53.9 &       11.5 &       26.6 &        5.6 \\
         5 &      189.284683 &       62.377537 &         15 &      33.50 &       1.68 &      30.20 &       1.51 &      21.00 &       1.40 &      20.50 &       1.24 &       96.0 &       18.3 &       89.1 &        6.2 \\
         6 &      189.301178 &       62.375061 &         21 &      10.90 &       0.55 &      10.50 &       0.53 &       8.67 &       0.75 &      11.60 &       0.82 &       75.5 &       11.7 &       60.5 &        3.6 \\
         7 &      189.317520 &       62.370590 &         27 &      28.40 &       1.42 &      24.10 &       1.21 &      20.70 &       1.15 &      34.00 &       1.78 &      129.3 &       14.6 &      133.0 &        4.9 \\
         8 &      189.314499 &       62.371925 &         26 &       1.16 &       0.08 &       1.13 &       0.10 &       0.47 &       0.52 &       3.13 &       0.56 &       56.7 &       11.3 &       50.7 &        4.0 \\
         9 &      189.306412 &       62.371181 &         22 &      50.70 &       2.54 &      37.50 &       1.88 &      32.20 &       1.70 &      30.10 &       1.60 &      339.4 &       13.7 &      436.0 &        5.8 \\
        10 &      189.266174 &       62.368641 &         19 &       7.67 &       0.39 &       5.57 &       0.30 &       4.81 &       0.84 &       4.93 &       0.72 &       62.8 &       15.0 &       18.3 &        4.6 \\
        11 &      189.292343 &       62.368526 &         18 &      32.10 &       1.61 &      29.90 &       1.50 &      21.80 &       1.23 &      23.50 &       1.30 &      130.8 &       12.8 &      125.0 &        4.0 \\
        12 &      189.351440 &       62.366024 &         21 &     242.00 &      12.10 &     199.00 &       9.95 &     131.00 &       6.57 &     214.00 &      10.71 &      365.8 &       17.6 &      395.0 &        7.7 \\
        13 &      189.351089 &       62.363888 &         21 &      18.80 &       0.94 &      14.00 &       0.70 &      12.40 &       0.77 &      14.00 &       0.87 &       62.8 &       11.8 &       60.5 &        6.2 \\
        14 &      189.281219 &       62.363293 &         15 &      47.40 &       2.37 &      51.00 &       2.55 &      52.10 &       2.66 &      59.60 &       3.03 &      129.2 &       16.5 &      240.0 &        3.4 \\
        15 &      189.276138 &       62.360157 &         22 &     101.00 &       5.05 &     103.00 &       5.15 &     117.00 &       5.88 &     123.00 &       6.17 &      219.1 &       14.1 &      303.0 &        5.2 \\
        16 &      189.306107 &       62.360352 &         25 &      10.50 &       0.53 &       8.62 &       0.44 &       6.47 &       0.56 &      13.40 &       0.84 &       53.4 &       11.3 &       85.5 &        3.6 \\
        17 &      189.240234 &       62.357346 &         25 &      20.80 &       1.04 &      17.20 &       0.87 &      18.90 &       1.22 &      24.80 &       1.41 &       71.2 &       12.8 &       10.6 &        5.1 \\
        18 &      189.241364 &       62.357990 &         29 &      18.80 &       0.94 &      21.90 &       1.10 &      35.70 &       1.94 &      40.90 &       2.15 &       70.8 &       12.0 &      210.0 &        5.0 \\
        19 &      189.274384 &       62.358295 &         20 &      35.60 &       1.78 &      26.00 &       1.30 &      25.90 &       1.40 &      23.90 &       1.31 &      289.9 &       12.6 &      364.0 &        5.5 \\
        20 &      189.281662 &       62.359962 &         22 &      36.00 &       1.80 &      26.80 &       1.34 &      22.50 &       1.24 &      18.20 &       1.06 &      155.0 &       12.4 &      206.0 &        4.7 \\
        21 &      189.272827 &       62.356556 &         23 &      87.90 &       4.40 &      63.10 &       3.16 &      54.50 &       2.77 &      43.40 &       2.23 &      385.3 &       17.0 &      513.0 &        7.5 \\
        22 &      189.309998 &       62.356476 &         24 &      36.70 &       1.84 &      27.40 &       1.37 &      21.00 &       1.14 &      20.80 &       1.16 &      198.0 &       13.5 &      216.0 &        4.5 \\
        23 &      189.280334 &       62.354317 &         23 &      25.20 &       1.26 &      19.10 &       0.96 &      16.10 &       0.94 &      13.60 &       0.85 &       81.5 &       12.0 &       95.3 &        4.5 \\
        24 &      189.317078 &       62.354118 &         20 &      75.10 &       3.76 &      62.60 &       3.13 &      44.00 &       2.24 &      43.30 &       2.22 &      344.7 &       17.0 &      322.0 &        4.4 \\
        25 &      189.288727 &       62.353016 &         24 &      65.90 &       3.30 &      48.00 &       2.40 &      37.90 &       1.95 &      45.30 &       2.32 &       82.0 &       14.2 &       90.0 &        6.0 \\
        26 &      189.310120 &       62.353397 &         22 &      30.30 &       1.52 &      21.50 &       1.08 &      18.20 &       1.01 &      15.40 &       0.92 &      176.2 &       14.2 &      212.0 &        4.6 \\
        27 &      189.367615 &       62.353096 &         29 &       3.63 &       0.19 &       4.02 &       0.22 &       2.24 &       0.46 &       4.10 &       0.56 &       45.0 &        7.4 &       24.4 &        5.8 \\
        28 &      189.270660 &       62.352474 &         26 &       4.57 &       0.23 &       7.86 &       0.40 &      16.30 &       0.95 &      32.90 &       1.73 &       54.2 &        9.1 &      121.0 &        4.6 \\
        29 &      189.363464 &       62.352116 &         31 &      50.80 &       2.54 &      43.30 &       2.17 &      32.10 &       1.67 &      79.40 &       4.00 &      161.6 &       10.5 &      165.0 &        5.3 \\
        30 &      189.275909 &       62.353241 &         24 &      18.10 &       0.91 &      18.10 &       0.91 &      13.60 &       0.83 &      17.70 &       1.03 &      101.7 &       12.6 &       77.7 &        3.6 \\
        31 &      189.277679 &       62.352192 &         21 &      16.10 &       0.81 &      15.00 &       0.75 &      12.00 &       0.76 &      11.80 &       0.78 &       76.0 &       10.0 &       49.5 &        3.4 \\
        32 &      189.223373 &       62.353222 &         24 &      14.80 &       0.74 &      13.30 &       0.67 &      11.20 &       0.98 &      20.60 &       1.25 &       50.7 &        8.9 &       78.1 &        3.8 \\
        33 &      189.255234 &       62.351688 &         36 &      30.30 &       1.52 &      24.10 &       1.21 &      25.10 &       1.36 &      27.30 &       1.47 &       53.8 &       10.9 &      272.0 &        5.6 \\
        34 &      189.360550 &       62.350456 &         27 &      13.90 &       0.70 &      11.40 &       0.58 &       7.46 &       0.58 &       8.16 &       0.65 &       73.2 &        9.8 &       59.6 &        4.6 \\
        35 &      189.252014 &       62.348610 &         26 &      18.20 &       0.91 &      16.40 &       0.82 &      12.40 &       0.80 &      12.70 &       0.83 &       86.1 &       11.5 &       66.5 &        4.5 \\
        36 &      189.335220 &       62.348377 &         21 &    2140.00 &     107.00 &    1370.00 &      68.50 &     938.00 &      46.90 &     515.00 &      25.76 &      115.2 &       11.1 &       50.1 &        4.5 \\
        37 &      189.366043 &       62.347420 &         26 &      10.50 &       0.53 &       8.72 &       0.44 &       5.88 &       0.53 &       5.79 &       0.58 &       54.6 &        9.8 &       64.8 &        5.4 \\
        38 &      189.372162 &       62.347504 &         22 &      11.50 &       0.58 &       8.45 &       0.43 &       6.68 &       0.55 &       5.32 &       0.58 &       69.6 &        8.7 &       69.6 &        5.2 \\
        39 &      189.255341 &       62.347500 &         29 &      19.50 &       0.98 &      18.50 &       0.93 &      12.10 &       0.78 &      12.00 &       0.80 &       89.8 &       11.3 &       84.4 &        4.8 \\
        40 &      189.300827 &       62.347290 &         27 &      21.50 &       1.08 &      16.10 &       0.81 &      13.80 &       0.82 &      14.10 &       0.87 &      152.0 &       13.3 &      156.0 &        4.4 \\
        41 &      189.390274 &       62.344513 &         16 &      29.20 &       1.46 &      19.70 &       0.99 &      16.10 &       0.92 &      11.20 &       0.76 &       87.0 &       12.4 &       76.7 &        6.0 \\
        42 &      189.360306 &       62.345402 &         25 &      28.90 &       1.45 &      24.70 &       1.24 &      20.20 &       1.10 &      36.50 &       1.89 &      113.1 &        8.3 &      121.0 &        5.3 \\
        43 &      189.375916 &       62.342354 &         19 &      28.30 &       1.42 &      18.80 &       0.94 &      18.80 &       1.04 &      13.30 &       0.84 &       76.7 &       10.4 &       75.7 &        4.9 \\
        44 &      189.344421 &       62.343815 &         31 &      33.50 &       1.68 &      24.30 &       1.22 &      25.40 &       1.34 &      18.90 &       1.07 &      201.5 &       11.3 &      210.0 &        5.1 \\
        45 &      189.331665 &       62.344101 &         19 &      52.70 &       2.64 &      53.40 &       2.67 &      39.30 &       2.01 &      31.40 &       1.65 &      103.1 &       11.3 &      121.0 &        4.7 \\
        46 &      189.315109 &       62.343750 &         26 &      13.70 &       0.69 &      12.50 &       0.63 &       8.52 &       0.61 &      10.50 &       0.73 &      113.3 &       10.5 &       80.1 &        5.3 \\
        47 &      189.369507 &       62.344112 &         21 &      25.40 &       1.27 &      26.60 &       1.33 &      20.40 &       1.11 &      23.10 &       1.26 &      196.2 &        8.9 &      120.0 &        6.0 \\
        48 &      189.408188 &       62.343510 &         10 &      17.40 &       0.87 &      10.10 &       0.51 &       9.74 &       0.68 &       5.77 &       0.62 &       60.1 &       11.1 &       41.5 &        5.3 \\
        49 &      189.210114 &       62.343159 &         21 &      47.60 &       2.38 &      32.00 &       1.60 &      34.60 &       1.83 &      25.10 &       1.40 &      210.3 &       12.6 &      232.0 &        4.8 \\
        50 &      189.308304 &       62.343521 &         25 &      81.70 &       4.09 &      56.30 &       2.82 &      45.90 &       2.34 &      29.00 &       1.53 &       49.7 &        9.2 &       42.6 &        5.8 \\
        51 &      189.384628 &       62.342239 &         23 &      28.90 &       1.45 &      29.40 &       1.47 &      26.40 &       1.39 &      28.60 &       1.52 &       62.8 &        8.9 &       74.5 &        5.3 \\
        52 &      189.414856 &       62.340782 &         10 &      57.60 &       2.88 &      56.20 &       2.81 &      40.30 &       2.07 &      99.40 &       5.00 &      286.4 &       14.2 &      363.0 &        5.5 \\
        53 &      189.393204 &       62.341873 &         15 &      69.50 &       3.48 &      48.20 &       2.41 &      35.30 &       1.82 &      24.20 &       1.32 &       60.8 &       12.9 &       84.8 &        5.4 \\
        54 &      189.360382 &       62.340733 &         23 &      31.10 &       1.56 &      43.30 &       2.17 &      77.10 &       3.88 &     160.00 &       8.02 &      975.6 &       29.2 &      931.0 &        8.6 \\
        55 &      189.223099 &       62.338474 &         18 &      18.30 &       0.92 &      13.60 &       0.68 &      12.90 &       0.81 &      16.30 &       0.97 &       63.0 &        9.6 &      112.0 &        4.8 \\
        56 &      189.398041 &       62.338421 &         33 &      35.10 &       1.76 &      29.00 &       1.45 &      19.80 &       1.09 &      17.10 &       1.00 &      108.9 &        8.1 &       86.8 &        4.5 \\
        57 &      189.392258 &       62.338905 &         25 &      15.30 &       0.77 &      11.60 &       0.58 &       7.94 &       0.59 &       7.16 &       0.62 &       50.9 &        7.8 &       38.6 &        5.0 \\
        58 &      189.396973 &       62.335575 &         33 &      22.40 &       1.12 &      17.30 &       0.87 &      12.70 &       0.77 &      15.20 &       0.91 &      101.9 &        7.0 &      113.0 &        4.6 \\
        59 &      189.402481 &       62.334915 &         26 &      11.40 &       0.57 &       8.42 &       0.43 &       9.46 &       0.65 &       7.38 &       0.62 &       56.0 &        7.2 &       49.3 &        4.7 \\
        60 &      189.324707 &       62.334538 &         35 &      22.20 &       1.11 &      18.30 &       0.92 &      20.20 &       1.10 &      19.60 &       1.10 &      266.9 &       13.1 &      284.0 &        6.5 \\
        61 &      189.304855 &       62.336174 &         19 &      16.60 &       0.83 &      10.60 &       0.54 &      10.80 &       0.69 &       8.07 &       0.64 &       63.1 &       12.0 &       52.9 &        5.7 \\
        62 &      189.233322 &       62.334309 &         28 &      19.80 &       0.99 &      20.10 &       1.01 &      14.30 &       0.84 &      15.50 &       0.92 &      114.0 &        9.1 &       73.5 &        4.0 \\
        63 &      189.203094 &       62.334061 &         19 &      15.40 &       0.77 &      11.30 &       0.57 &       8.28 &       0.67 &       7.36 &       0.65 &       65.4 &       10.0 &       68.2 &        4.4 \\
        64 &      189.227600 &       62.333847 &         31 &      11.40 &       0.57 &       9.00 &       0.46 &       7.03 &       0.56 &       6.51 &       0.60 &       44.8 &        7.6 &       36.5 &        4.8 \\
        65 &      189.252701 &       62.335392 &         30 &      40.40 &       2.02 &      28.40 &       1.42 &      24.20 &       1.29 &      18.20 &       1.04 &       97.8 &        9.8 &      106.0 &        3.7 \\
        66 &      189.281616 &       62.332233 &         22 &      19.40 &       0.97 &      17.20 &       0.86 &      11.40 &       0.72 &      13.00 &       0.82 &       72.3 &       13.5 &       69.7 &        5.2 \\
        67 &      189.305359 &       62.331585 &         33 &      75.60 &       3.78 &      69.20 &       3.46 &      56.20 &       2.84 &     147.00 &       7.37 &      447.2 &       17.8 &      538.0 &        6.8 \\
        68 &      189.271744 &       62.330799 &         17 &      54.40 &       2.72 &      38.80 &       1.94 &      36.90 &       1.89 &      33.90 &       1.77 &      318.1 &       22.4 &      483.0 &        6.8 \\
        69 &      189.209946 &       62.330540 &         22 &      22.70 &       1.14 &      17.30 &       0.87 &      14.30 &       0.86 &      13.20 &       0.83 &      102.1 &        8.5 &      114.0 &        5.2 \\
        70 &      189.188324 &       62.330162 &         19 &       9.53 &       0.48 &       6.64 &       0.34 &       6.00 &       0.62 &       3.85 &       0.60 &       55.7 &       10.5 &       40.8 &        5.1 \\
        71 &      189.397400 &       62.329533 &         21 &      22.00 &       1.10 &      18.70 &       0.94 &      17.10 &       0.96 &      29.80 &       1.57 &      115.6 &       12.6 &      222.0 &        4.8 \\
        72 &      189.210693 &       62.329468 &         23 &      93.90 &       4.70 &      69.00 &       3.45 &      48.20 &       2.45 &      38.50 &       1.99 &      131.1 &       11.3 &      172.0 &        5.2 \\
        73 &      189.356461 &       62.328178 &         21 &     194.00 &       0.09 &     186.00 &       0.14 &     126.00 &       0.66 &     491.00 &       0.67 &      851.9 &       43.3 &     1040.0 &       12.8 \\
        74 &      189.389557 &       62.328068 &         19 &      60.90 &       3.05 &      56.40 &       2.82 &      41.10 &       2.10 &     147.00 &       7.37 &      281.1 &       12.8 &      341.0 &        6.1 \\
        75 &      189.302429 &       62.327930 &         44 &       6.40 &       0.32 &       6.15 &       0.32 &       7.02 &       0.56 &       6.36 &       0.59 &       46.0 &        7.4 &      104.0 &        5.8 \\
        76 &      189.167145 &       62.328163 &         10 &    5160.00 &    4677.12 &    3640.00 &     182.00 &    2650.00 &     132.50 &    1440.00 &      72.00 &      350.0 &       25.5 &      185.0 &        5.0 \\
        77 &      189.211853 &       62.327671 &         27 &      12.60 &       0.63 &       9.17 &       0.46 &       4.72 &       0.50 &       5.64 &       0.56 &       53.6 &       12.0 &       51.4 &        4.9 \\
        78 &      189.350403 &       62.327526 &         18 &       9.99 &       0.50 &       6.47 &       0.33 &       6.16 &       0.53 &       5.78 &       0.58 &       41.9 &        8.1 &       55.9 &        6.2 \\
        79 &      189.235291 &       62.327114 &         25 &      11.10 &       0.56 &      14.00 &       0.70 &      21.80 &       1.17 &      43.90 &       2.25 &      263.3 &       16.5 &      716.0 &        7.4 \\
        80 &      189.373871 &       62.326229 &         25 &     194.00 &       9.70 &     151.00 &       7.55 &      96.30 &       4.83 &      75.00 &       3.78 &       65.9 &        8.1 &       63.8 &        4.2 \\
        81 &      189.339828 &       62.324299 &         18 &     112.00 &       5.60 &      93.50 &       4.68 &      71.60 &       3.61 &     377.00 &      18.86 &      436.6 &       19.6 &      379.0 &        4.8 \\
        82 &      189.267624 &       62.325352 &         30 &      19.80 &       0.99 &      14.10 &       0.71 &      11.10 &       0.69 &      10.10 &       0.71 &      102.3 &        9.4 &       84.4 &        4.7 \\
        83 &      189.232864 &       62.325447 &         27 &      17.10 &       0.86 &      13.50 &       0.68 &      12.30 &       0.74 &      15.40 &       0.91 &       61.7 &        8.0 &       51.1 &        5.2 \\
        84 &      189.295822 &       62.324558 &         37 &      76.50 &       3.83 &      61.90 &       3.10 &      42.70 &       2.18 &      44.80 &       2.29 &      381.8 &       13.5 &      357.0 &        6.8 \\
        85 &      189.267349 &       62.323410 &         26 &      25.80 &       1.29 &      17.50 &       0.88 &      15.80 &       0.89 &      13.10 &       0.82 &      103.9 &        9.2 &      130.0 &        5.3 \\
        86 &      189.189346 &       62.323418 &         20 &      22.00 &       1.10 &      19.30 &       0.97 &      14.20 &       0.86 &      17.10 &       0.99 &      203.2 &       12.0 &      169.0 &        4.8 \\
        87 &      189.281067 &       62.321999 &         27 &      27.20 &       1.36 &      18.70 &       0.94 &      15.00 &       0.86 &      12.20 &       0.78 &       78.1 &        8.3 &       93.3 &        5.2 \\
        88 &      189.413971 &       62.322010 &         35 &      13.00 &       0.65 &      12.10 &       0.61 &       9.39 &       0.64 &       8.51 &       0.64 &       53.9 &        8.7 &       40.1 &        5.7 \\
        89 &      189.397156 &       62.321640 &         19 &      76.10 &       3.81 &      52.70 &       2.64 &      50.50 &       2.56 &      53.80 &       2.73 &      279.3 &        9.4 &      496.0 &        6.6 \\
        90 &      189.178101 &       62.320911 &         22 &      21.90 &       1.10 &      15.70 &       0.79 &      13.80 &       0.83 &       9.88 &       0.70 &       73.2 &        7.8 &       90.6 &        5.3 \\
        91 &      189.310349 &       62.321331 &         27 &      15.60 &       0.78 &      15.30 &       0.77 &      11.90 &       0.74 &      11.70 &       0.77 &       67.9 &        9.4 &       71.3 &        4.9 \\
        92 &      189.163467 &       62.319660 &         25 &      18.90 &       0.95 &      17.80 &       0.89 &      13.50 &       0.82 &      13.30 &       0.83 &      146.5 &       13.3 &       83.2 &        5.1 \\
        93 &      189.418945 &       62.321327 &         36 &      14.60 &       0.73 &      13.10 &       0.66 &      10.20 &       0.66 &      12.20 &       0.78 &       93.1 &        8.9 &       98.5 &        6.5 \\
        94 &      189.427689 &       62.318157 &         21 &     161.00 &       8.05 &     115.00 &       5.75 &      91.80 &       4.61 &     207.00 &      10.36 &      129.2 &       11.5 &      204.0 &        9.4 \\
        95 &      189.422653 &       62.317741 &         25 &      16.10 &       0.81 &      15.10 &       0.76 &      16.00 &       0.90 &      37.20 &       1.92 &      198.0 &       13.5 &      296.0 &        7.7 \\
        96 &      189.163956 &       62.317196 &         25 &      28.00 &       1.40 &      20.10 &       1.01 &      17.40 &       0.97 &      15.20 &       0.89 &      172.9 &       11.3 &      208.0 &        5.6 \\
        97 &      189.429230 &       62.316891 &         15 &    3800.00 &    6602.73 &    2920.00 &     146.00 &    2020.00 &     101.00 &    1090.00 &      54.50 &      302.2 &       12.9 &      118.0 &        7.2 \\
        98 &      189.150330 &       62.318115 &         19 &      26.70 &       1.34 &      17.70 &       0.89 &      19.90 &       1.10 &      13.20 &       0.84 &       79.0 &       14.4 &      127.0 &        6.7 \\
        99 &      189.324463 &       62.315426 &         28 &      14.00 &       0.70 &      18.50 &       0.93 &      27.40 &       1.44 &      38.20 &       1.97 &       68.1 &        8.5 &      192.0 &        5.9 \\
       100 &      189.356216 &       62.313900 &         28 &      82.20 &       4.11 &      54.40 &       2.72 &      53.50 &       2.71 &      39.90 &       2.05 &      388.9 &       16.8 &      484.0 &        6.2 \\
       101 &      189.189133 &       62.316936 &         21 &      45.00 &       2.25 &      40.60 &       2.03 &      44.40 &       2.26 &      86.70 &       4.36 &      282.8 &       19.4 &      613.0 &        7.7 \\
       102 &      189.367981 &       62.315258 &         23 &      22.20 &       1.11 &      23.70 &       1.19 &      18.00 &       1.00 &      14.60 &       0.88 &       55.0 &        9.4 &       48.4 &        5.2 \\
       103 &      189.141556 &       62.313885 &         16 &      10.10 &       0.51 &      11.80 &       0.59 &       9.67 &       0.65 &      11.10 &       0.74 &       98.4 &       13.9 &       98.1 &        9.1 \\
       104 &      189.145248 &       62.313602 &         18 &       5.06 &       0.26 &       5.58 &       0.29 &       4.69 &       0.48 &       4.47 &       0.52 &       67.1 &       14.4 &       27.0 &        8.1 \\
       105 &      189.418411 &       62.314892 &         21 &      27.40 &       1.37 &      20.20 &       1.01 &      18.80 &       1.03 &      15.30 &       0.90 &      138.1 &       10.2 &      154.0 &        6.4 \\
       106 &      189.273087 &       62.314232 &         21 &      31.70 &       1.59 &      24.10 &       1.21 &      25.10 &       1.32 &      21.40 &       1.17 &      304.0 &       17.8 &      285.0 &        5.3 \\
       107 &      189.422150 &       62.314072 &         21 &      23.60 &       0.07 &      16.70 &       0.08 &      21.50 &       0.42 &      12.30 &       0.42 &       82.0 &       16.8 &      110.0 &        6.8 \\
       108 &      189.189468 &       62.313709 &         23 &      14.30 &       0.72 &      18.70 &       0.94 &      25.30 &       1.33 &      39.80 &       2.04 &       78.1 &       13.9 &      153.0 &        6.5 \\
       109 &      189.133774 &       62.312881 &         12 &      16.20 &       0.81 &      15.30 &       0.77 &      12.20 &       0.76 &      12.10 &       0.80 &       86.3 &       17.6 &       52.0 &        6.6 \\
       110 &      189.256317 &       62.311867 &         32 &     217.00 &       0.09 &     177.00 &       0.14 &     113.00 &       0.67 &     326.00 &       0.69 &      399.4 &       24.6 &      408.0 &        7.5 \\
       111 &      189.343842 &       62.310604 &         22 &      56.70 &       2.84 &      62.10 &       3.11 &      48.50 &       2.46 &      42.60 &       2.19 &      169.0 &        6.8 &      241.0 &        5.2 \\
       112 &      189.186768 &       62.310516 &         19 &      19.50 &       0.98 &      21.90 &       1.10 &      18.70 &       1.01 &      16.20 &       0.91 &       64.5 &       11.7 &      211.0 &        5.6 \\
       113 &      189.311218 &       62.310947 &         26 &       5.62 &       0.28 &       7.83 &       0.40 &      10.60 &       0.68 &      18.50 &       1.05 &       51.6 &        7.4 &      113.0 &        5.2 \\
       114 &      189.170288 &       62.310040 &         21 &      26.70 &       1.34 &      19.10 &       0.96 &      17.10 &       0.93 &      14.10 &       0.81 &      102.9 &       13.7 &      173.0 &        6.3 \\
       115 &      189.247147 &       62.308994 &         30 &       9.05 &       0.45 &      10.50 &       0.53 &      14.20 &       0.82 &      21.60 &       1.18 &      141.2 &       11.7 &      293.0 &        7.3 \\
       116 &      189.156784 &       62.308384 &         16 &      21.30 &       1.07 &      15.40 &       0.77 &      13.70 &       0.77 &      11.10 &       0.69 &       91.4 &       14.1 &       85.1 &        5.5 \\
       117 &      189.171844 &       62.307945 &         22 &      26.90 &       1.35 &      17.60 &       0.88 &      16.30 &       0.89 &      11.60 &       0.70 &      106.6 &       15.7 &      135.0 &        5.4 \\
       118 &      189.168976 &       62.309155 &         25 &      65.60 &       3.28 &      54.40 &       2.72 &      38.70 &       1.97 &      30.00 &       1.55 &       84.7 &       14.2 &       32.7 &        5.7 \\
       119 &      189.320114 &       62.306732 &         27 &      44.20 &       2.21 &      31.20 &       1.56 &      35.90 &       1.85 &      29.90 &       1.57 &      399.4 &       19.8 &      425.0 &        6.2 \\
       120 &      189.360580 &       62.307308 &         33 &      36.80 &       1.84 &      29.80 &       1.49 &      21.20 &       1.14 &      35.00 &       1.82 &       97.2 &       12.4 &       77.2 &        5.3 \\
       121 &      189.307724 &       62.307304 &         30 &       3.75 &       0.19 &       6.02 &       0.31 &       9.18 &       0.62 &      15.40 &       0.91 &       42.8 &        7.6 &       55.2 &        5.8 \\
       122 &      189.272751 &       62.306953 &         20 &      17.80 &       0.89 &      14.60 &       0.73 &      10.80 &       0.67 &      10.10 &       0.70 &       74.2 &       12.9 &       63.3 &        4.5 \\
       123 &      189.132431 &       62.305748 &         25 &      12.10 &       0.61 &       8.09 &       0.41 &       6.99 &       0.52 &       5.83 &       0.52 &       67.9 &       14.1 &       86.6 &        5.8 \\
       124 &      189.260269 &       62.305637 &         26 &      18.00 &       0.90 &      11.80 &       0.59 &      11.00 &       0.68 &       7.80 &       0.61 &       44.2 &        8.0 &       60.6 &        4.7 \\
       125 &      189.177673 &       62.305756 &         31 &      54.00 &       2.70 &      46.10 &       2.31 &      30.80 &       1.58 &      30.00 &       1.55 &      208.5 &       10.5 &      177.0 &        5.6 \\
       126 &      189.124908 &       62.304939 &         21 &      23.00 &       1.15 &      20.20 &       1.01 &      16.30 &       0.91 &      32.40 &       1.68 &      107.2 &       15.9 &      151.0 &        6.4 \\
       127 &      189.256958 &       62.303997 &         27 &      41.40 &       2.07 &      36.50 &       1.83 &      28.80 &       1.50 &      64.10 &       3.24 &      178.6 &       10.7 &      214.0 &        4.6 \\
       128 &      189.188202 &       62.304466 &         21 &       9.86 &       0.49 &      12.00 &       0.60 &      10.30 &       0.63 &      11.00 &       0.68 &       86.6 &       13.3 &       44.9 &        4.5 \\
       129 &      189.210938 &       62.303665 &         21 &      17.50 &       0.88 &      12.10 &       0.61 &      12.70 &       0.75 &      10.60 &       0.69 &       57.9 &       11.5 &       65.2 &        7.6 \\
       130 &      189.427170 &       62.303295 &         23 &      26.40 &       1.32 &      31.20 &       1.56 &      47.50 &       2.41 &      73.50 &       3.71 &      138.1 &       15.5 &      194.0 &        4.6 \\
       131 &      189.419128 &       62.302872 &         21 &      20.10 &       1.01 &      15.40 &       0.77 &      13.00 &       0.77 &      15.10 &       0.90 &      199.7 &       13.3 &      184.0 &        5.1 \\
       132 &      189.220093 &       62.302135 &         20 &     156.00 &       7.80 &     153.00 &       7.65 &     116.00 &       5.81 &     600.00 &      30.00 &      873.1 &       28.1 &      752.0 &        7.4 \\
       133 &      189.127930 &       62.301956 &         21 &      16.80 &       0.84 &      12.20 &       0.61 &       8.32 &       0.55 &       8.75 &       0.60 &       85.9 &        9.4 &       86.4 &        5.3 \\
       134 &      189.397964 &       62.301449 &         20 &     111.00 &       5.55 &      73.80 &       3.69 &      68.40 &       3.44 &      48.40 &       2.47 &      350.0 &       17.2 &      460.0 &        7.7 \\
       135 &      189.133362 &       62.299755 &         20 &      22.10 &       1.11 &      14.40 &       0.72 &      14.70 &       0.81 &      11.40 &       0.69 &       95.8 &       12.0 &      115.0 &        6.2 \\
       136 &      189.220474 &       62.299690 &         21 &      29.30 &       1.47 &      20.60 &       1.03 &      18.60 &       1.01 &      18.00 &       1.00 &      134.0 &       18.1 &      165.0 &        5.5 \\
       137 &      189.248077 &       62.299545 &         24 &      21.90 &       1.10 &      15.00 &       0.75 &      14.00 &       0.81 &      10.50 &       0.71 &      108.4 &       10.7 &      119.0 &        5.8 \\
       138 &      189.321548 &       62.301285 &         19 &      11.80 &       0.59 &       8.21 &       0.42 &       6.58 &       0.54 &       5.62 &       0.56 &       58.9 &       10.5 &       50.6 &        5.8 \\
       139 &      189.445023 &       62.297482 &         20 &      19.40 &       0.97 &      19.00 &       0.95 &      14.60 &       0.85 &      13.60 &       0.84 &      149.7 &       15.0 &      104.0 &        8.1 \\
       140 &      189.440414 &       62.296795 &         19 &      39.90 &       2.00 &      31.00 &       1.55 &      27.20 &       1.43 &      23.00 &       1.25 &       69.1 &       16.3 &       91.0 &        7.4 \\
       141 &      189.143356 &       62.297340 &         23 &      36.00 &       1.80 &      23.80 &       1.19 &      23.90 &       1.24 &      19.80 &       1.06 &      119.1 &       10.5 &      197.0 &        6.1 \\
       142 &      189.119751 &       62.297138 &         27 &      14.60 &       0.73 &      10.20 &       0.51 &       9.66 &       0.60 &       7.72 &       0.56 &       76.9 &       14.6 &       99.5 &        6.1 \\
       143 &      189.094955 &       62.298691 &         17 &      42.70 &       2.14 &      29.80 &       1.49 &      29.00 &       1.52 &      24.50 &       1.34 &      240.4 &       16.6 &      279.0 &        6.8 \\
       144 &      189.412170 &       62.296890 &         30 &      16.20 &       0.81 &      13.40 &       0.67 &       9.73 &       0.64 &       8.99 &       0.66 &       53.0 &       12.6 &       32.8 &        5.3 \\
       145 &      189.158661 &       62.296574 &         27 &     108.00 &       5.40 &      83.90 &       4.20 &      66.60 &       3.35 &      84.60 &       4.25 &      187.4 &       16.5 &      234.0 &        6.8 \\
       146 &      189.156723 &       62.296211 &         20 &      48.30 &       2.42 &      35.80 &       1.79 &      36.60 &       1.86 &      46.70 &       2.36 &      147.4 &       15.9 &      182.0 &        6.6 \\
       147 &      189.300690 &       62.298355 &         28 &      34.40 &       1.72 &      33.30 &       1.67 &      25.50 &       1.34 &      29.50 &       1.55 &      183.8 &       10.5 &      144.0 &        3.8 \\
       148 &      189.103317 &       62.295349 &         25 &      22.10 &       1.11 &      26.10 &       1.31 &      24.90 &       1.30 &      19.00 &       1.05 &       57.9 &       12.2 &      214.0 &        6.1 \\
       149 &      189.132736 &       62.295811 &         22 &      45.90 &       2.30 &      33.40 &       1.67 &      36.90 &       1.88 &      37.70 &       1.92 &      160.6 &       15.5 &      295.0 &        7.0 \\
       150 &      189.420425 &       62.295734 &         25 &      10.40 &       0.52 &      12.40 &       0.62 &      12.40 &       0.75 &      10.50 &       0.72 &       50.0 &       11.7 &      162.0 &        5.9 \\
       151 &      189.446869 &       62.295776 &         20 &      16.40 &       0.82 &      14.60 &       0.73 &       9.51 &       0.64 &      10.50 &       0.73 &       89.0 &       12.9 &       53.0 &        4.8 \\
       152 &      189.089401 &       62.297028 &         15 &      50.60 &       2.53 &      34.90 &       1.75 &      37.90 &       1.95 &      32.40 &       1.71 &      205.0 &       17.0 &      228.0 &        5.7 \\
       153 &      189.308411 &       62.295265 &         31 &       8.51 &       0.43 &       9.79 &       0.49 &       8.51 &       0.59 &       7.26 &       0.59 &       37.0 &        6.5 &       48.2 &        6.0 \\
       154 &      189.225464 &       62.293831 &         29 &      82.30 &       4.12 &      74.80 &       3.74 &      55.30 &       2.79 &     140.00 &       7.01 &      334.1 &       13.9 &      362.0 &        5.4 \\
       155 &      189.497803 &       62.292522 &         11 &      41.60 &       2.08 &      32.00 &       1.60 &      23.30 &       1.26 &      23.20 &       1.28 &      236.9 &       15.7 &      215.0 &        4.9 \\
       156 &      189.251358 &       62.291851 &         23 &      15.40 &       0.77 &      11.30 &       0.57 &      10.70 &       0.68 &       8.59 &       0.65 &       57.3 &       10.7 &       65.5 &        4.8 \\
       157 &      189.249527 &       62.293259 &         23 &      16.70 &       0.84 &      11.60 &       0.58 &      12.10 &       0.73 &       9.96 &       0.69 &       68.2 &        8.9 &       72.8 &        5.4 \\
       158 &      189.319458 &       62.292587 &         37 &      62.70 &       3.14 &      81.50 &       4.08 &     124.00 &       6.21 &     219.00 &      10.96 &      528.4 &       13.1 &     1240.0 &       15.5 \\
       159 &      189.442337 &       62.291878 &         20 &      27.20 &       1.36 &      26.40 &       1.32 &      23.80 &       1.27 &      62.30 &       3.16 &      215.6 &       14.1 &      388.0 &        7.9 \\
       160 &      189.139252 &       62.291847 &         20 &      13.60 &       0.68 &      11.20 &       0.56 &       8.42 &       0.53 &       9.42 &       0.60 &       77.4 &       12.4 &       60.5 &        4.6 \\
       161 &      189.084564 &       62.291534 &         29 &      28.10 &       1.41 &      19.10 &       0.96 &      19.30 &       1.06 &      16.10 &       0.95 &      168.6 &       10.4 &      246.0 &        8.0 \\
       162 &      189.276947 &       62.291412 &         45 &      86.40 &       4.32 &      76.90 &       3.85 &      53.20 &       2.69 &     140.00 &       7.02 &      268.6 &       12.0 &      288.0 &        4.3 \\
       163 &      189.452866 &       62.290024 &         18 &      38.20 &       1.91 &      30.80 &       1.54 &      24.80 &       1.32 &      41.70 &       2.14 &      118.8 &       11.3 &      111.0 &        5.3 \\
       164 &      189.300064 &       62.290840 &         38 &      15.00 &       0.75 &      10.20 &       0.51 &      10.00 &       0.64 &       7.26 &       0.59 &       53.8 &        6.5 &       50.2 &        5.7 \\
       165 &      189.103622 &       62.289154 &         19 &      26.30 &       1.32 &      18.40 &       0.92 &      17.60 &       0.95 &      16.40 &       0.91 &       75.5 &       13.3 &       88.4 &        5.9 \\
       166 &      189.419540 &       62.289009 &         18 &      10.80 &       0.54 &      10.30 &       0.52 &       6.60 &       0.54 &       7.51 &       0.62 &       60.8 &       11.1 &       36.6 &        5.9 \\
       167 &      189.473236 &       62.288830 &         24 &      51.90 &       2.60 &      35.00 &       1.75 &      30.60 &       1.59 &      21.40 &       1.18 &      142.2 &       12.6 &      193.0 &        7.6 \\
       168 &      189.393829 &       62.289803 &         26 &     177.00 &       8.85 &     119.00 &       5.95 &     128.00 &       6.41 &     106.00 &       5.32 &      539.1 &       22.4 &      741.0 &        7.1 \\
       169 &      189.263428 &       62.288834 &         40 &      25.50 &       1.28 &      25.60 &       1.28 &      19.50 &       1.06 &      15.10 &       0.89 &       81.6 &        6.7 &       45.0 &        3.8 \\
       170 &      189.318741 &       62.288734 &         59 &     638.00 &      31.90 &     420.00 &      21.00 &     278.00 &      13.91 &     156.00 &       7.81 &       49.1 &        8.0 &       20.9 &        7.7 \\
       171 &      189.275726 &       62.286766 &         40 &     162.00 &       8.10 &     137.00 &       6.85 &      90.80 &       4.56 &     254.00 &      12.71 &      463.0 &       17.6 &      613.0 &        9.5 \\
       172 &      189.479599 &       62.288303 &         16 &      21.40 &       1.07 &      19.40 &       0.97 &      13.60 &       0.81 &      14.40 &       0.88 &      132.0 &       14.2 &       92.9 &        7.1 \\
       173 &      189.442398 &       62.287209 &         28 &      13.70 &       0.69 &      13.00 &       0.65 &      12.30 &       0.75 &       8.71 &       0.66 &       75.5 &       12.9 &       32.4 &        5.7 \\
       174 &      189.230835 &       62.288319 &         27 &      20.40 &       1.02 &      14.70 &       0.74 &      13.20 &       0.76 &      10.10 &       0.66 &       83.1 &        7.0 &      123.0 &        5.6 \\
       175 &      189.063751 &       62.287903 &         12 &      53.30 &       2.67 &      43.90 &       2.20 &      37.40 &       1.95 &      34.10 &       1.82 &      129.7 &       13.5 &      111.0 &        7.0 \\
       176 &      189.249832 &       62.287689 &         28 &      94.60 &       4.73 &      77.80 &       3.89 &      56.60 &       2.86 &      87.90 &       4.42 &      235.1 &       10.0 &      236.0 &        5.1 \\
       177 &      189.205978 &       62.286640 &         33 &     827.00 &      41.35 &     565.00 &      28.25 &     375.00 &      18.75 &     208.00 &      10.41 &       58.9 &       10.5 &       23.6 &        6.2 \\
       178 &      189.379593 &       62.287437 &         20 &      33.50 &       1.68 &      24.00 &       1.20 &      17.30 &       0.96 &      17.00 &       0.98 &      190.9 &       11.7 &      196.0 &        4.0 \\
       179 &      189.364426 &       62.287220 &         28 &      27.00 &       1.35 &      19.30 &       0.97 &      21.30 &       1.14 &      17.00 &       0.97 &      166.3 &       11.1 &      186.0 &        4.6 \\
       180 &      189.397614 &       62.286469 &         31 &      47.60 &       2.38 &      32.90 &       1.65 &      34.80 &       1.79 &      28.10 &       1.49 &      158.0 &       12.0 &      204.0 &        6.2 \\
       181 &      189.357422 &       62.287354 &         30 &      15.50 &       0.78 &      10.70 &       0.54 &       9.63 &       0.63 &       9.01 &       0.65 &       91.2 &       13.1 &      105.0 &        4.9 \\
       182 &      189.150925 &       62.285820 &         16 &      23.40 &       1.17 &      15.30 &       0.77 &      12.80 &       0.71 &       9.40 &       0.59 &       86.8 &       12.8 &       84.0 &        4.6 \\
       183 &      189.115509 &       62.285637 &         25 &      12.90 &       0.65 &      11.40 &       0.57 &       7.13 &       0.48 &       7.39 &       0.53 &       65.4 &       11.1 &       32.7 &        5.9 \\
       184 &      189.371536 &       62.285603 &         30 &      18.90 &       0.95 &      16.30 &       0.82 &      11.10 &       0.69 &      13.20 &       0.82 &      165.3 &       10.0 &      137.0 &        6.5 \\
       185 &      189.341125 &       62.285309 &         24 &      25.10 &       1.26 &      18.80 &       0.94 &      20.40 &       1.09 &      22.10 &       1.20 &       88.2 &       15.2 &      121.0 &        5.2 \\
       186 &      189.094315 &       62.284988 &         29 &      51.40 &       2.57 &      38.40 &       1.92 &      32.60 &       1.67 &      39.30 &       2.01 &      117.9 &       12.2 &      141.0 &        5.0 \\
       187 &      189.365280 &       62.284985 &         34 &       6.77 &       0.34 &       8.60 &       0.44 &       9.11 &       0.62 &       8.86 &       0.65 &       48.5 &       10.2 &      171.0 &        5.5 \\
       188 &      189.182938 &       62.284882 &         24 &      31.50 &       1.58 &      25.10 &       1.26 &      22.70 &       1.18 &      41.50 &       2.11 &      132.4 &       13.1 &      218.0 &        6.0 \\
       189 &      189.128357 &       62.284760 &         34 &      74.90 &       3.75 &      53.10 &       2.66 &      33.30 &       1.70 &      39.20 &       1.99 &       92.1 &       10.7 &      246.0 &        7.3 \\
       190 &      189.409103 &       62.284225 &         24 &      11.90 &       0.60 &      13.90 &       0.70 &      14.80 &       0.85 &      12.60 &       0.80 &       47.2 &        9.1 &      264.0 &        6.0 \\
       191 &      189.175797 &       62.286434 &         25 &      12.60 &       0.63 &      15.10 &       0.76 &      20.30 &       1.06 &      28.50 &       1.47 &       57.7 &       10.5 &      116.0 &        7.0 \\
       192 &      189.135437 &       62.283154 &         31 &     189.00 &       0.07 &     166.00 &       0.10 &     121.00 &       0.46 &     247.00 &       0.46 &      622.1 &       39.0 &      795.0 &       12.9 \\
       193 &      189.461456 &       62.285332 &         29 &      80.80 &       4.04 &      48.60 &       2.43 &      44.30 &       2.26 &      26.50 &       1.42 &       77.4 &       10.0 &       92.5 &        5.5 \\
       194 &      189.415894 &       62.283821 &         22 &      49.50 &       2.48 &      35.80 &       1.79 &      27.90 &       1.46 &      22.80 &       1.24 &       63.1 &       13.5 &       29.0 &        5.3 \\
       195 &      189.061493 &       62.283390 &         22 &      21.10 &       1.06 &      18.60 &       0.93 &      11.90 &       0.80 &      12.60 &       0.86 &       88.6 &       12.9 &       68.0 &        7.9 \\
       196 &      189.191696 &       62.283546 &         20 &      29.90 &       1.50 &      23.10 &       1.16 &      18.20 &       0.96 &      14.80 &       0.83 &       64.0 &       12.2 &       80.8 &        4.4 \\
       197 &      189.054062 &       62.283043 &         10 &      77.60 &       3.88 &      50.00 &       2.50 &      50.20 &       2.59 &      40.00 &       2.11 &      251.0 &       24.6 &      357.0 &        9.1 \\
       198 &      189.161407 &       62.285122 &         19 &      21.50 &       1.08 &      14.50 &       0.73 &      15.80 &       0.85 &      12.70 &       0.73 &       84.1 &       11.8 &      112.0 &        5.7 \\
       199 &      189.299927 &       62.283146 &         76 &      19.60 &       0.98 &      15.90 &       0.80 &      12.60 &       0.74 &      12.80 &       0.78 &      145.6 &        7.6 &      112.0 &        5.4 \\
       200 &      189.384109 &       62.282944 &         29 &      83.00 &       4.15 &      59.10 &       2.96 &      47.20 &       2.40 &      40.50 &       2.08 &      380.0 &       16.5 &      461.0 &        6.6 \\
       201 &      189.229156 &       62.282913 &         20 &      48.60 &       2.43 &      36.50 &       1.83 &      29.80 &       1.53 &      36.50 &       1.87 &      134.0 &       11.5 &      106.0 &        5.8 \\
       202 &      189.146835 &       62.281845 &         15 &      31.20 &       1.56 &      23.30 &       1.17 &      22.70 &       1.18 &      17.30 &       0.94 &      166.9 &       12.8 &      180.0 &        4.9 \\
       203 &      189.232620 &       62.282124 &         24 &      17.40 &       0.87 &      13.60 &       0.68 &      11.70 &       0.69 &       9.83 &       0.64 &       68.1 &        8.1 &       67.2 &        4.9 \\
       204 &      189.278610 &       62.283916 &         43 &     159.00 &       7.95 &     188.00 &       9.40 &     242.00 &      12.11 &     302.00 &      15.11 &      570.8 &       21.6 &      913.0 &        9.4 \\
       205 &      189.261658 &       62.282150 &         41 &       9.19 &       0.46 &       6.65 &       0.34 &       5.30 &       0.48 &       3.63 &       0.50 &       48.9 &        6.8 &       40.6 &        5.9 \\
       206 &      189.343597 &       62.280926 &         24 &      17.40 &       0.87 &      11.90 &       0.60 &      10.30 &       0.65 &       8.36 &       0.62 &       82.0 &       12.8 &       94.4 &        5.2 \\
       207 &      189.180557 &       62.281254 &         31 &      42.50 &       2.13 &      30.70 &       1.54 &      27.60 &       1.42 &      22.00 &       1.16 &      205.0 &       12.6 &      255.0 &        5.7 \\
       208 &      189.284058 &       62.283085 &         41 &      71.70 &       3.59 &      67.60 &       3.38 &      58.70 &       2.96 &     151.00 &       7.56 &      431.3 &       13.7 &      532.0 &        6.8 \\
       209 &      189.429855 &       62.280090 &         19 &      30.20 &       1.51 &      20.60 &       1.03 &      17.60 &       0.98 &      13.30 &       0.83 &      105.5 &       11.5 &      144.0 &        4.8 \\
       210 &      189.434296 &       62.281059 &         21 &      13.40 &       0.67 &      12.70 &       0.64 &       8.50 &       0.61 &      10.60 &       0.73 &      113.5 &       13.5 &       93.6 &        5.3 \\
       211 &      189.319107 &       62.278721 &         35 &      62.00 &       3.10 &      71.60 &       3.58 &      70.50 &       3.55 &      53.10 &       2.69 &      162.1 &       12.2 &      508.0 &        6.3 \\
       212 &      189.263840 &       62.279591 &         41 &      10.10 &       0.51 &       6.63 &       0.34 &       6.84 &       0.52 &       4.19 &       0.50 &       38.2 &        9.4 &       30.4 &        4.7 \\
       213 &      189.245071 &       62.277164 &         34 &      73.90 &       3.70 &      65.20 &       3.26 &      44.10 &       2.23 &     130.00 &       6.51 &      249.2 &       11.8 &      278.0 &        5.8 \\
       214 &      189.269302 &       62.281044 &         42 &      40.90 &       2.05 &      39.00 &       1.95 &      30.70 &       1.59 &      72.60 &       3.66 &      160.3 &        8.9 &      181.0 &        4.4 \\
       215 &      189.517868 &       62.278290 &         13 &      26.80 &       1.34 &      23.80 &       1.19 &      19.90 &       1.11 &      30.90 &       1.63 &       76.9 &       13.3 &      124.0 &        4.8 \\
       216 &      189.416992 &       62.279869 &         29 &      16.60 &       0.83 &      16.90 &       0.85 &      17.20 &       0.96 &      19.70 &       1.10 &      130.1 &       11.7 &       88.1 &        5.1 \\
       217 &      189.104050 &       62.278065 &         40 &    2700.00 &     135.00 &    1610.00 &      80.50 &    1090.00 &      54.50 &     609.00 &      30.45 &      153.2 &       13.5 &       65.0 &        5.7 \\
       218 &      189.176773 &       62.279152 &         29 &      13.70 &       0.69 &       8.75 &       0.44 &       7.96 &       0.51 &       5.54 &       0.45 &       73.2 &       10.0 &       64.9 &        4.8 \\
       219 &      189.263367 &       62.277863 &         43 &       9.62 &       0.48 &       5.95 &       0.30 &       6.24 &       0.50 &       3.19 &       0.48 &       39.6 &        8.3 &        4.2 &        4.2 \\
       220 &      189.298325 &       62.277878 &         58 &      10.30 &       0.52 &       9.05 &       0.46 &       5.92 &       0.50 &       5.14 &       0.53 &       40.9 &        6.5 &       30.6 &        5.6 \\
       221 &      189.469696 &       62.276676 &         20 &      29.70 &       1.49 &      24.10 &       1.21 &      20.40 &       1.11 &      20.20 &       1.13 &      155.9 &       17.9 &      127.0 &        5.9 \\
       222 &      189.191513 &       62.278969 &         31 &      10.60 &       0.53 &       9.93 &       0.50 &       6.62 &       0.46 &       8.49 &       0.56 &       75.5 &        8.7 &       38.3 &        4.6 \\
       223 &      189.142426 &       62.278175 &         26 &      18.20 &       0.91 &      15.30 &       0.77 &      14.00 &       0.77 &      27.00 &       1.40 &       53.0 &       10.0 &       95.9 &        4.3 \\
       224 &      189.208298 &       62.276978 &         19 &      18.80 &       0.94 &      15.20 &       0.76 &      11.60 &       0.66 &      21.10 &       1.12 &       64.9 &       11.8 &       69.6 &        6.1 \\
       225 &      189.478836 &       62.276447 &         19 &       8.90 &       0.45 &       9.37 &       0.47 &       7.31 &       0.57 &       8.76 &       0.67 &      115.2 &        9.6 &       50.9 &        5.7 \\
       226 &      189.088531 &       62.277767 &         21 &       9.55 &       0.48 &       7.88 &       0.40 &       5.97 &       0.47 &       9.83 &       0.64 &       54.6 &       12.0 &      131.0 &        5.3 \\
       227 &      189.269882 &       62.278370 &         35 &      13.30 &       0.67 &      10.20 &       0.51 &       8.12 &       0.57 &       8.58 &       0.63 &       75.3 &        7.8 &       79.0 &        3.5 \\
       228 &      189.074875 &       62.276428 &         30 &      97.50 &       4.88 &      86.60 &       4.33 &      86.90 &       4.37 &     101.00 &       5.07 &      265.1 &       15.9 &      656.0 &        7.1 \\
       229 &      189.130981 &       62.275833 &         20 &      14.20 &       0.71 &      17.10 &       0.86 &      14.00 &       0.77 &      13.40 &       0.76 &       77.9 &       12.0 &       96.5 &        3.6 \\
       230 &      189.259354 &       62.275299 &         46 &      12.80 &       0.64 &       9.92 &       0.50 &       9.80 &       0.61 &       9.04 &       0.63 &       40.7 &        6.7 &       46.2 &        5.7 \\
       231 &      189.446136 &       62.275558 &         26 &     165.00 &       8.25 &     128.00 &       6.40 &     113.00 &       5.67 &     148.00 &       7.42 &      300.5 &       12.0 &      381.0 &        5.8 \\
       232 &      189.431183 &       62.275475 &         28 &      22.80 &       1.14 &      19.70 &       0.99 &      14.70 &       0.85 &      30.90 &       1.62 &       69.5 &        9.2 &       86.2 &        5.2 \\
       233 &      189.464371 &       62.275349 &         19 &      13.90 &       0.70 &      12.40 &       0.62 &       8.80 &       0.62 &      10.10 &       0.71 &       54.6 &       10.7 &       23.8 &        6.3 \\
       234 &      189.469666 &       62.274502 &         21 &     226.00 &      11.30 &     246.00 &      12.30 &     257.00 &      12.86 &     495.00 &      24.76 &     1145.3 &       37.0 &     1720.0 &       11.4 \\
       235 &      189.408081 &       62.275169 &         21 &   10500.00 &    3920.00 &    9040.00 &       0.40 &    9140.00 &       0.98 &    4860.00 &       0.69 &     1378.6 &       42.0 &      681.0 &       10.3 \\
       236 &      189.335846 &       62.274891 &         36 &      22.30 &       1.12 &      15.10 &       0.76 &      15.50 &       0.87 &      13.00 &       0.79 &      102.9 &       10.4 &      110.0 &        6.1 \\
       237 &      189.135239 &       62.274441 &         18 &      42.10 &       2.11 &      29.30 &       1.47 &      25.60 &       1.32 &      19.30 &       1.03 &      141.4 &       16.5 &      175.0 &        4.8 \\
       238 &      189.278061 &       62.274647 &         47 &      27.20 &       1.36 &      19.10 &       0.96 &      16.50 &       0.92 &      11.90 &       0.75 &       80.6 &        9.1 &       80.7 &        5.3 \\
       239 &      189.094406 &       62.274899 &         30 &      20.30 &       1.02 &      27.50 &       1.38 &      35.50 &       1.81 &      26.60 &       1.39 &      105.2 &       11.1 &      417.0 &        8.2 \\
       240 &      189.488678 &       62.274292 &         19 &      23.00 &       1.15 &      28.00 &       1.40 &      39.30 &       2.01 &      59.50 &       3.02 &       93.7 &       14.2 &      163.0 &        5.0 \\
       241 &      189.351227 &       62.275520 &         30 &      27.00 &       1.35 &      18.30 &       0.92 &      17.50 &       0.96 &      12.20 &       0.77 &      163.9 &       10.7 &      158.0 &        6.2 \\
       242 &      189.145248 &       62.274517 &         20 &      55.90 &       2.80 &      38.60 &       1.93 &      40.20 &       2.03 &      36.00 &       1.84 &      369.4 &       21.5 &      510.0 &        7.1 \\
       243 &      189.249649 &       62.274452 &         41 &      50.80 &       2.54 &      38.10 &       1.91 &      26.70 &       1.38 &      20.70 &       1.11 &       59.2 &        6.5 &       67.1 &        6.5 \\
       244 &      189.267776 &       62.273575 &         51 &      21.40 &       1.07 &      18.90 &       0.95 &      15.00 &       0.84 &      29.60 &       1.54 &       88.4 &        6.5 &       87.0 &        4.4 \\
       245 &      189.204453 &       62.272392 &         18 &      21.10 &       1.06 &      15.20 &       0.76 &      12.30 &       0.69 &      14.40 &       0.81 &       70.2 &       11.1 &       48.9 &        5.6 \\
       246 &      189.379837 &       62.272301 &         21 &      82.90 &       4.15 &      60.50 &       3.03 &      50.40 &       2.56 &      48.10 &       2.45 &      549.7 &       25.7 &      622.0 &        7.2 \\
       247 &      189.484436 &       62.273056 &         20 &      15.00 &       0.75 &      13.70 &       0.69 &       9.63 &       0.65 &      23.40 &       1.27 &       67.5 &       10.5 &       64.4 &        5.5 \\
       248 &      189.364426 &       62.272739 &         16 &    1010.00 &      50.50 &     740.00 &      37.00 &     482.00 &      24.10 &     266.00 &      13.31 &       65.4 &       10.5 &       20.5 &        5.1 \\
       249 &      189.048096 &       62.272072 &         14 &      34.60 &       1.73 &      37.40 &       1.87 &      28.40 &       1.52 &      28.30 &       1.52 &      296.9 &       16.3 &      172.0 &        7.8 \\
       250 &      189.197510 &       62.272324 &         21 &      16.00 &       0.80 &      12.60 &       0.63 &       9.83 &       0.58 &      14.30 &       0.80 &       56.7 &        9.6 &       49.5 &        4.6 \\
       251 &      189.088348 &       62.271767 &         32 &      70.60 &       3.53 &      44.80 &       2.24 &      39.90 &       2.03 &      26.50 &       1.39 &       75.9 &       14.6 &      107.0 &        6.7 \\
       252 &      189.251648 &       62.271328 &         36 &      39.40 &       1.97 &      29.00 &       1.45 &      31.30 &       1.60 &      28.30 &       1.47 &      376.4 &       14.1 &      501.0 &        7.6 \\
       253 &      189.137589 &       62.271202 &         19 &      18.90 &       0.95 &      12.10 &       0.61 &      10.60 &       0.62 &       6.35 &       0.48 &       69.3 &       11.5 &       62.7 &        5.6 \\
       254 &      189.365311 &       62.271263 &         17 &      40.90 &       2.05 &      28.90 &       1.45 &      24.90 &       1.31 &      29.10 &       1.53 &       57.9 &       12.6 &      124.0 &        6.3 \\
       255 &      189.282257 &       62.271099 &         42 &      80.70 &       4.04 &      58.00 &       2.90 &      45.50 &       2.31 &      33.70 &       1.75 &      155.3 &        9.4 &      202.0 &        6.5 \\
       256 &      189.350555 &       62.269920 &         29 &      11.40 &       0.57 &      12.80 &       0.64 &      10.50 &       0.66 &      10.60 &       0.71 &       50.5 &       10.7 &      128.0 &        5.6 \\
       257 &      189.193039 &       62.270733 &         19 &      20.60 &       1.03 &      16.60 &       0.83 &      13.70 &       0.75 &      23.40 &       1.22 &       67.5 &        9.2 &       69.4 &        4.7 \\
       258 &      189.311508 &       62.271324 &         47 &      17.80 &       0.89 &      21.50 &       1.08 &      19.20 &       1.04 &      19.00 &       1.05 &       66.9 &        9.1 &      124.0 &        5.8 \\
       259 &      189.384140 &       62.269497 &         18 &      74.40 &       3.72 &      51.50 &       2.58 &      44.70 &       2.28 &      32.90 &       1.72 &      183.8 &       14.2 &      221.0 &        7.7 \\
       260 &      189.122238 &       62.270325 &         35 &      81.70 &       4.09 &      57.00 &       2.85 &      54.80 &       2.76 &      55.70 &       2.81 &      126.4 &       10.0 &      218.0 &        4.9 \\
       261 &      189.390182 &       62.268475 &         24 &      25.70 &       1.29 &      14.90 &       0.75 &      19.60 &       1.07 &      13.20 &       0.82 &       86.4 &       13.7 &      120.0 &        5.6 \\
       262 &      189.462051 &       62.266884 &         21 &     119.00 &       5.95 &      98.60 &       4.93 &      65.40 &       3.30 &      53.50 &       2.72 &      164.5 &       11.8 &      186.0 &        5.4 \\
       263 &      189.131882 &       62.267773 &         19 &      45.40 &       2.27 &      29.50 &       1.48 &      32.90 &       1.68 &      25.60 &       1.33 &      288.1 &       15.5 &      314.0 &        6.9 \\
       264 &      189.087387 &       62.268631 &         51 &      15.80 &       0.79 &      14.60 &       0.73 &       9.28 &       0.60 &       8.73 &       0.61 &       36.0 &        8.3 &       28.5 &        4.3 \\
       265 &      189.250229 &       62.268288 &         19 &      16.60 &       0.83 &      11.80 &       0.59 &       8.49 &       0.54 &       9.05 &       0.60 &       87.1 &       12.9 &      101.0 &        7.2 \\
       266 &      189.282745 &       62.268250 &         39 &      79.90 &       4.00 &      56.50 &       2.83 &      47.30 &       2.39 &      41.10 &       2.10 &      362.3 &       10.9 &      447.0 &        7.9 \\
       267 &      189.450592 &       62.269535 &         21 &      13.80 &       0.69 &      15.40 &       0.77 &      13.80 &       0.82 &       9.94 &       0.70 &       65.9 &       10.2 &       33.6 &        5.1 \\
       268 &      189.153214 &       62.267956 &         33 &      25.60 &       1.28 &      17.30 &       0.87 &      14.10 &       0.77 &       9.66 &       0.60 &       76.0 &        9.4 &       83.7 &        5.1 \\
       269 &      189.306641 &       62.267696 &         54 &      34.30 &       1.72 &      28.20 &       1.41 &      24.50 &       1.28 &      23.20 &       1.24 &      183.8 &        9.6 &      202.0 &        5.6 \\
       270 &      189.078018 &       62.266994 &         24 &      26.20 &       1.31 &      21.00 &       1.05 &      16.00 &       0.90 &      15.60 &       0.90 &      129.2 &        9.2 &      153.0 &        5.2 \\
       271 &      189.114456 &       62.268047 &         24 &      33.20 &       1.66 &      28.40 &       1.42 &      19.60 &       1.04 &      17.50 &       0.95 &       77.3 &        9.4 &       73.9 &        5.9 \\
       272 &      189.165771 &       62.266762 &         38 &      62.10 &       3.11 &      48.40 &       2.42 &      37.10 &       1.88 &      26.60 &       1.38 &       45.2 &        6.5 &       54.5 &        7.3 \\
       273 &      189.309708 &       62.266365 &         56 &      42.10 &       2.11 &      31.30 &       1.57 &      34.70 &       1.78 &      31.60 &       1.64 &      140.1 &        7.8 &      153.0 &        5.2 \\
       274 &      189.270294 &       62.267101 &         34 &       9.45 &       0.47 &      11.60 &       0.58 &      13.60 &       0.77 &      15.70 &       0.89 &       64.0 &        9.1 &       65.0 &        4.6 \\
       275 &      189.082520 &       62.266998 &         33 &      14.70 &       0.74 &      13.70 &       0.69 &      10.40 &       0.65 &      10.10 &       0.67 &       83.6 &        8.7 &       49.9 &        4.6 \\
       276 &      189.088943 &       62.262741 &         26 &      40.70 &       2.04 &      36.20 &       1.81 &      24.50 &       1.29 &      23.50 &       1.25 &      149.5 &       10.7 &      109.0 &        4.9 \\
       277 &      189.469650 &       62.264866 &         27 &      29.10 &       1.46 &      26.90 &       1.35 &      18.60 &       1.03 &      16.70 &       0.98 &       63.8 &        6.5 &       70.6 &        4.5 \\
       278 &      189.412704 &       62.266441 &         34 &      18.10 &       0.91 &      13.60 &       0.68 &      11.80 &       0.73 &      10.30 &       0.72 &       92.8 &       11.7 &       95.2 &        5.2 \\
       279 &      189.072662 &       62.264221 &         24 &      22.10 &       1.11 &      22.20 &       1.11 &      15.70 &       0.89 &      49.30 &       2.51 &      126.6 &        9.8 &      124.0 &        5.9 \\
       280 &      189.372025 &       62.264107 &         21 &      31.40 &       1.57 &      21.20 &       1.06 &      18.70 &       1.02 &      16.00 &       0.93 &      101.9 &       10.9 &      176.0 &        5.5 \\
       281 &      189.384628 &       62.263847 &         17 &      15.60 &       0.78 &      16.80 &       0.84 &      10.90 &       0.69 &      12.20 &       0.78 &       84.9 &       10.5 &       59.2 &        6.4 \\
       282 &      189.326721 &       62.264915 &         54 &      36.20 &       1.81 &      28.60 &       1.43 &      22.60 &       1.20 &      30.30 &       1.58 &       81.8 &        6.7 &       94.8 &        6.7 \\
       283 &      189.145493 &       62.263561 &         32 &      25.80 &       1.29 &      16.70 &       0.84 &      14.80 &       0.81 &      11.10 &       0.66 &       72.4 &        9.8 &       99.4 &        5.1 \\
       284 &      189.306931 &       62.262558 &         61 &       9.70 &       0.49 &      13.00 &       0.65 &      19.20 &       1.04 &      16.50 &       0.95 &       35.2 &        6.8 &      149.0 &        6.1 \\
       285 &      189.175858 &       62.262623 &         26 &     116.00 &       5.80 &      95.40 &       4.77 &     108.00 &       5.41 &     125.00 &       6.26 &      595.6 &       23.9 &      866.0 &       10.3 \\
       286 &      189.243271 &       62.263523 &         27 &      12.40 &       0.62 &      11.00 &       0.55 &       7.62 &       0.50 &      14.00 &       0.79 &       61.7 &        7.6 &      102.0 &        5.4 \\
       287 &      189.032303 &       62.261780 &         23 &      15.40 &       0.77 &      16.80 &       0.84 &      11.40 &       0.76 &      13.50 &       0.87 &      142.8 &       13.1 &       99.0 &        5.7 \\
       288 &      189.033493 &       62.264858 &         18 &      20.60 &       1.03 &      18.40 &       0.92 &      16.60 &       0.98 &      24.40 &       1.35 &       57.1 &       10.4 &      126.0 &        5.8 \\
       289 &      189.167206 &       62.260921 &         34 &      23.20 &       1.16 &      21.20 &       1.06 &      14.80 &       0.80 &      14.40 &       0.80 &      117.4 &       10.0 &       85.9 &        7.1 \\
       290 &      189.093674 &       62.262337 &         29 &      71.20 &       3.56 &      48.80 &       2.44 &      58.70 &       2.96 &      69.10 &       3.48 &      371.1 &        9.2 &      725.0 &        6.8 \\
       291 &      189.161575 &       62.263107 &         31 &      15.60 &       0.78 &      10.10 &       0.51 &       9.33 &       0.56 &       6.14 &       0.47 &       72.4 &        7.4 &       64.1 &        5.7 \\
       292 &      189.290863 &       62.263222 &         53 &       0.86 &       0.06 &       1.29 &       0.09 &       2.94 &       0.39 &      10.90 &       0.70 &       48.1 &        8.0 &       64.0 &        5.7 \\
       293 &      189.043198 &       62.262630 &         20 &      41.20 &       2.06 &      29.90 &       1.50 &      25.30 &       1.35 &      20.50 &       1.15 &      220.9 &       12.2 &      271.0 &        6.1 \\
       294 &      189.302917 &       62.262836 &         65 &      32.50 &       1.63 &      23.10 &       1.16 &      23.40 &       1.24 &      21.80 &       1.18 &      226.2 &        9.2 &      310.0 &        6.8 \\
       295 &      189.261368 &       62.262115 &         27 &     141.00 &       7.05 &     130.00 &       6.50 &     139.00 &       6.96 &     162.00 &       8.11 &      344.7 &       14.2 &      484.0 &        6.6 \\
       296 &      189.207779 &       62.261623 &         27 &      23.30 &       1.17 &      16.50 &       0.83 &      13.50 &       0.74 &      10.50 &       0.64 &       70.2 &        9.2 &       90.0 &        5.9 \\
       297 &      189.195282 &       62.261284 &         24 &      29.50 &       1.48 &      19.90 &       1.00 &      17.50 &       0.93 &      12.50 &       0.72 &      112.1 &        9.1 &      148.0 &        7.0 \\
       298 &      189.181351 &       62.258972 &         28 &       9.66 &       0.48 &       6.41 &       0.32 &       6.61 &       0.45 &       4.40 &       0.42 &       42.2 &        7.4 &       45.6 &        6.1 \\
       299 &      189.489822 &       62.260441 &         24 &       7.50 &       0.38 &       8.98 &       0.46 &       7.33 &       0.57 &       7.99 &       0.65 &       94.7 &        9.6 &       51.5 &        6.3 \\
       300 &      189.373016 &       62.259247 &         33 &       9.62 &       0.48 &       9.51 &       0.48 &       6.95 &       0.54 &       7.47 &       0.60 &       43.5 &        8.3 &       20.8 &        5.6 \\
       301 &      189.374573 &       62.258015 &         37 &       6.13 &       0.31 &       5.84 &       0.30 &       4.12 &       0.46 &       4.72 &       0.53 &       69.8 &        9.4 &       44.4 &        6.6 \\
       302 &      189.409515 &       62.258266 &         29 &      65.70 &       3.29 &      57.70 &       2.89 &      40.10 &       2.05 &      37.30 &       1.93 &      203.2 &       10.0 &      163.0 &        3.8 \\
       303 &      189.192795 &       62.257732 &         29 &      80.20 &       4.01 &      54.20 &       2.71 &      54.90 &       2.76 &      43.50 &       2.20 &      475.4 &       17.2 &      537.0 &        6.9 \\
       304 &      189.095581 &       62.257378 &         18 &      47.00 &       2.35 &      52.10 &       2.61 &      76.90 &       3.87 &     136.00 &       6.81 &      351.7 &       12.9 &      549.0 &        9.1 \\
       305 &      189.165466 &       62.257298 &         22 &      46.50 &       2.33 &      40.70 &       2.04 &      28.70 &       1.47 &      69.10 &       3.47 &      163.9 &       11.5 &      161.0 &        5.4 \\
       306 &      189.072235 &       62.258205 &         28 &      63.00 &       3.15 &      42.70 &       2.14 &      44.50 &       2.27 &      32.50 &       1.69 &      392.4 &       12.9 &      502.0 &        7.7 \\
       307 &      189.266754 &       62.256462 &         40 &       7.67 &       0.38 &       6.72 &       0.34 &       4.47 &       0.39 &      10.40 &       0.64 &       27.9 &        5.6 &       25.5 &        5.6 \\
       308 &      189.101303 &       62.257008 &         28 &      25.00 &       1.25 &      17.00 &       0.85 &      18.40 &       1.00 &      13.70 &       0.81 &      112.9 &       11.7 &      151.0 &        6.6 \\
       309 &      189.517715 &       62.257195 &         18 &      25.60 &       1.28 &      29.50 &       1.48 &      28.70 &       1.51 &      22.10 &       1.25 &       71.2 &       12.0 &      180.0 &        7.7 \\
       310 &      189.426132 &       62.255127 &         21 &     115.00 &       5.75 &      77.70 &       3.89 &      78.20 &       3.93 &     295.00 &      14.76 &      364.1 &       15.7 &      992.0 &        6.3 \\
       311 &      189.492188 &       62.254669 &         26 &      31.70 &       1.59 &      22.80 &       1.14 &      19.30 &       1.06 &      15.90 &       0.96 &       79.6 &       15.7 &      131.0 &        5.2 \\
       312 &      189.358246 &       62.255276 &         27 &      18.50 &       0.93 &      12.90 &       0.65 &      14.50 &       0.83 &      11.90 &       0.76 &       79.4 &       11.8 &      153.0 &        5.6 \\
       313 &      189.360718 &       62.255051 &         28 &      49.50 &       2.48 &      35.30 &       1.77 &      34.40 &       1.77 &      33.60 &       1.74 &      164.2 &       10.9 &      156.0 &        5.2 \\
       314 &      189.304749 &       62.255108 &         47 &      16.80 &       0.84 &      12.10 &       0.61 &      12.20 &       0.72 &      10.30 &       0.69 &      146.0 &        7.4 &      165.0 &        5.9 \\
       315 &      189.102982 &       62.252895 &         20 &      99.60 &       4.98 &      61.00 &       3.05 &      53.90 &       2.72 &      31.30 &       1.63 &       85.9 &       10.4 &       82.0 &        6.0 \\
       316 &      189.299057 &       62.254120 &         52 &      23.90 &       1.20 &      20.30 &       1.02 &      14.10 &       0.79 &      32.60 &       1.69 &       67.7 &        5.6 &       89.1 &        6.2 \\
       317 &      189.420563 &       62.254791 &         23 &     156.00 &       7.80 &     125.00 &       6.25 &      85.90 &       4.32 &     110.00 &       5.52 &      224.4 &       15.0 &      245.0 &        5.3 \\
       318 &      189.284912 &       62.254066 &         42 &      28.30 &       1.42 &      19.20 &       0.96 &      20.10 &       1.06 &      15.30 &       0.86 &      182.1 &        9.8 &      199.0 &        6.5 \\
       319 &      189.484055 &       62.253727 &         28 &     263.00 &      13.15 &     193.00 &       9.65 &     116.00 &       5.82 &      95.10 &       4.78 &       54.2 &       10.2 &       62.9 &        8.7 \\
       320 &      189.465881 &       62.255608 &         19 &      32.60 &       1.63 &      35.90 &       1.80 &      32.10 &       1.66 &      37.10 &       1.92 &      238.6 &        8.3 &      226.0 &        4.8 \\
       321 &      189.447372 &       62.253551 &         36 &      50.10 &       2.51 &      32.60 &       1.63 &      37.40 &       1.92 &      27.20 &       1.45 &      203.2 &       10.4 &      239.0 &        6.2 \\
       322 &      189.318268 &       62.253410 &         43 &     120.00 &       6.00 &      81.90 &       4.10 &      69.20 &       3.48 &      61.00 &       3.09 &      111.7 &       17.0 &      198.0 &        9.4 \\
       323 &      189.307129 &       62.253124 &         49 &      35.70 &       1.79 &      28.20 &       1.41 &      26.60 &       1.38 &      33.80 &       1.75 &      109.4 &        7.0 &      150.0 &        6.1 \\
       324 &      189.067078 &       62.253792 &         22 &      12.70 &       0.64 &      18.10 &       0.91 &      28.50 &       1.49 &      40.80 &       2.10 &       55.9 &       10.0 &      326.0 &        8.0 \\
       325 &      189.258102 &       62.252884 &         30 &      16.10 &       0.81 &      10.90 &       0.55 &       8.67 &       0.53 &       7.58 &       0.52 &       59.1 &        7.2 &       83.4 &        6.7 \\
       326 &      189.482193 &       62.251862 &         17 &     689.00 &       0.15 &     538.00 &       0.21 &     380.00 &       0.93 &     983.00 &       0.98 &      774.1 &       51.8 &      665.0 &       16.4 \\
       327 &      189.080078 &       62.253510 &         30 &      19.60 &       0.98 &      12.60 &       0.63 &      12.20 &       0.74 &       7.99 &       0.62 &       79.2 &       11.1 &       78.9 &        5.4 \\
       328 &      189.135315 &       62.253647 &         18 &      37.50 &       1.88 &      24.70 &       1.24 &      24.50 &       1.27 &      20.30 &       1.09 &      137.9 &        8.7 &      152.0 &        7.4 \\
       329 &      189.138046 &       62.253803 &         22 &      16.80 &       0.84 &      13.90 &       0.70 &      12.70 &       0.72 &      19.90 &       1.07 &       45.6 &        7.4 &       40.3 &        6.8 \\
       330 &      189.288086 &       62.252220 &         40 &      27.00 &       1.35 &      24.90 &       1.25 &      18.20 &       0.97 &      18.10 &       0.99 &      142.0 &        7.8 &      123.0 &        5.8 \\
       331 &      189.499481 &       62.251778 &         21 &      21.00 &       1.05 &      17.90 &       0.90 &      11.80 &       0.74 &      11.40 &       0.81 &      134.0 &       10.0 &       96.5 &        5.2 \\
       332 &      189.041000 &       62.251129 &         24 &      29.90 &       1.50 &      21.30 &       1.07 &      19.90 &       1.08 &      16.60 &       0.97 &      141.2 &       13.5 &      174.0 &        6.5 \\
       333 &      189.170029 &       62.251301 &         24 &      35.90 &       1.80 &      24.60 &       1.23 &      19.20 &       1.01 &      14.80 &       0.82 &       83.3 &       17.8 &       98.8 &        5.8 \\
       334 &      189.005280 &       62.250546 &         14 &      15.80 &       0.79 &      12.00 &       0.60 &       9.88 &       0.72 &      21.00 &       1.20 &      147.7 &       15.9 &      186.0 &        6.2 \\
       335 &      189.373169 &       62.249744 &         26 &      22.30 &       1.12 &      16.10 &       0.81 &      11.70 &       0.71 &      11.40 &       0.74 &       61.0 &       11.7 &       82.2 &        5.7 \\
       336 &      189.184784 &       62.248058 &         30 &      17.20 &       0.86 &      17.30 &       0.87 &      15.30 &       0.82 &      16.40 &       0.89 &       83.4 &        8.3 &       77.9 &        6.0 \\
       337 &      189.494934 &       62.249516 &         25 &      88.40 &       4.42 &      74.80 &       3.74 &      51.60 &       2.62 &      45.30 &       2.34 &      176.6 &        8.1 &      167.0 &        5.6 \\
       338 &      189.253830 &       62.249489 &         36 &      15.20 &       0.76 &      13.90 &       0.70 &       9.46 &       0.56 &      10.20 &       0.62 &       61.8 &       10.0 &       45.6 &        4.9 \\
       339 &      189.440491 &       62.249065 &         24 &      19.20 &       0.96 &      14.80 &       0.74 &      11.50 &       0.72 &      10.70 &       0.73 &       79.4 &       11.1 &       98.5 &        5.9 \\
       340 &      189.174744 &       62.249058 &         30 &      28.60 &       1.43 &      19.40 &       0.97 &      18.00 &       0.95 &      12.40 &       0.72 &       98.6 &        8.9 &      124.0 &        6.2 \\
       341 &      189.160583 &       62.248672 &         26 &      16.40 &       0.82 &      10.80 &       0.54 &       9.78 &       0.58 &       7.58 &       0.53 &       78.1 &       10.4 &       80.6 &        5.5 \\
       342 &      189.305786 &       62.247334 &         37 &      76.60 &       3.83 &      56.20 &       2.81 &      47.10 &       2.38 &      34.50 &       1.78 &      201.5 &       10.4 &      238.0 &        6.8 \\
       343 &      189.186737 &       62.248714 &         34 &      10.20 &       0.51 &       6.97 &       0.35 &       6.79 &       0.46 &       5.32 &       0.45 &       41.9 &        8.0 &       34.5 &        5.6 \\
       344 &      189.240814 &       62.248615 &         28 &      49.00 &       2.45 &      34.60 &       1.73 &      36.30 &       1.84 &      30.00 &       1.54 &      282.8 &       11.1 &      373.0 &        7.8 \\
       345 &      189.347778 &       62.246765 &         34 &      74.90 &       3.75 &      62.10 &       3.11 &      39.60 &       2.02 &     105.00 &       5.27 &      180.3 &        8.7 &      157.0 &        4.5 \\
       346 &      189.413162 &       62.248528 &         34 &      51.50 &       2.58 &      34.90 &       1.75 &      38.60 &       1.98 &      29.50 &       1.55 &      353.5 &       15.0 &      373.0 &        4.2 \\
       347 &      189.414612 &       62.250607 &         29 &      21.50 &       1.08 &      14.10 &       0.71 &      15.80 &       0.90 &      11.90 &       0.77 &      131.3 &        7.8 &      128.0 &        4.0 \\
       348 &      189.321686 &       62.248371 &         30 &      10.40 &       0.52 &       7.22 &       0.37 &       6.97 &       0.52 &       5.91 &       0.56 &       75.3 &       10.9 &       75.7 &        5.4 \\
       349 &      189.342545 &       62.246971 &         36 &      39.10 &       1.96 &      25.70 &       1.29 &      24.60 &       1.30 &      17.70 &       1.00 &      171.4 &       11.3 &      174.0 &        5.8 \\
       350 &      189.191025 &       62.246395 &         23 &      13.80 &       0.69 &      18.10 &       0.91 &      19.90 &       1.04 &      24.80 &       1.29 &       58.9 &       10.9 &       64.5 &        9.5 \\
       351 &      189.239426 &       62.247536 &         29 &      64.50 &       3.23 &      54.40 &       2.72 &      36.20 &       1.83 &      29.90 &       1.53 &       48.1 &        9.2 &        3.7 &        7.7 \\
       352 &      189.249695 &       62.247196 &         30 &      54.30 &       2.72 &      35.70 &       1.79 &      43.20 &       2.18 &      35.20 &       1.79 &      418.8 &       19.6 &      472.0 &        6.1 \\
       353 &      189.116150 &       62.246937 &         29 &      77.20 &       3.86 &      47.30 &       2.37 &      41.70 &       2.12 &      23.80 &       1.27 &       52.8 &       10.5 &       45.6 &        6.3 \\
       354 &      189.167496 &       62.246502 &         33 &      11.00 &       0.55 &      10.50 &       0.53 &       7.33 &       0.49 &       7.47 &       0.52 &       59.7 &       10.2 &       37.0 &        5.9 \\
       355 &      189.195328 &       62.246460 &         21 &      45.80 &       2.29 &      32.10 &       1.61 &      30.00 &       1.53 &      29.80 &       1.53 &      136.3 &       28.1 &      422.0 &       29.1 \\
       356 &      189.464096 &       62.244049 &         20 &      29.50 &       1.48 &      32.90 &       1.65 &      30.30 &       1.58 &      24.50 &       1.34 &       64.3 &        8.0 &      219.0 &        6.3 \\
       357 &      189.061249 &       62.248329 &         30 &      19.00 &       0.95 &      15.10 &       0.76 &      10.70 &       0.68 &      10.50 &       0.71 &       85.7 &       12.6 &       86.8 &        5.4 \\
       358 &      189.405975 &       62.246281 &         25 &      10.10 &       0.51 &       8.13 &       0.41 &       9.11 &       0.62 &       8.41 &       0.64 &       62.2 &        7.8 &       66.4 &        5.4 \\
       359 &      189.268097 &       62.246170 &         17 &       5.99 &       0.30 &       6.85 &       0.35 &      14.30 &       0.78 &      40.00 &       2.03 &      206.8 &       13.1 &      380.0 &        4.8 \\
       360 &      189.490631 &       62.246960 &         20 &      15.20 &       0.76 &      15.90 &       0.80 &      12.00 &       0.75 &       9.77 &       0.76 &       60.3 &        9.2 &       56.1 &        5.5 \\
       361 &      189.324020 &       62.244251 &         28 &      23.20 &       1.16 &      21.30 &       1.07 &      15.40 &       0.86 &      38.90 &       2.00 &      116.8 &       10.2 &      112.0 &        5.5 \\
       362 &      189.124557 &       62.244698 &         34 &      15.90 &       0.80 &      10.00 &       0.50 &       9.62 &       0.61 &       7.34 &       0.57 &       46.8 &        9.4 &       45.5 &        5.3 \\
       363 &      189.442474 &       62.244587 &         19 &      35.30 &       1.77 &      23.60 &       1.18 &      24.50 &       1.30 &      24.40 &       1.32 &      122.3 &        8.3 &      118.0 &        7.2 \\
       364 &      189.127838 &       62.244270 &         38 &      21.70 &       1.09 &      20.80 &       1.04 &      15.10 &       0.84 &      13.50 &       0.80 &       50.3 &       11.1 &       55.2 &        5.7 \\
       365 &      189.051834 &       62.243992 &         29 &      34.70 &       1.74 &      35.60 &       1.78 &      24.90 &       1.31 &      27.30 &       1.45 &      129.5 &        8.9 &      147.0 &        5.6 \\
       366 &      189.055130 &       62.243835 &         25 &      48.90 &       2.45 &      40.70 &       2.04 &      28.70 &       1.50 &      26.30 &       1.41 &      183.8 &       10.2 &      150.0 &        5.6 \\
       367 &      189.149521 &       62.243336 &         27 &      24.80 &       1.24 &      21.50 &       1.08 &      16.40 &       0.89 &      19.40 &       1.05 &      189.1 &       12.9 &      198.0 &       14.3 \\
       368 &      189.410873 &       62.242001 &         29 &      13.70 &       0.69 &       9.55 &       0.48 &       9.60 &       0.64 &       6.84 &       0.59 &       47.4 &       10.4 &       91.3 &        5.5 \\
       369 &      189.485214 &       62.242451 &         14 &      40.00 &       2.00 &      31.80 &       1.59 &      21.20 &       1.16 &      20.50 &       1.19 &      166.5 &       12.2 &      130.0 &        6.6 \\
       370 &      189.245193 &       62.243019 &         29 &      87.10 &       4.36 &      59.00 &       2.95 &      57.70 &       2.90 &      47.20 &       2.38 &       98.8 &       11.8 &      198.0 &        6.7 \\
       371 &      189.441177 &       62.243050 &         21 &     104.00 &       5.20 &      95.20 &       4.76 &      65.50 &       3.30 &     208.00 &      10.41 &      388.9 &       13.1 &      444.0 &        9.2 \\
       372 &      189.128632 &       62.242626 &         36 &      20.20 &       1.01 &      17.20 &       0.86 &      12.70 &       0.74 &      24.50 &       1.30 &       59.4 &        8.3 &       70.9 &        5.6 \\
       373 &      189.140625 &       62.241913 &         32 &      81.80 &       4.09 &      61.40 &       3.07 &      55.60 &       2.80 &      57.60 &       2.91 &      146.7 &       10.0 &      170.0 &       12.1 \\
       374 &      189.371140 &       62.242435 &         32 &      40.80 &       2.04 &      34.60 &       1.73 &      25.30 &       1.33 &      21.50 &       1.17 &       86.1 &        8.7 &       98.7 &        5.1 \\
       375 &      189.137833 &       62.243668 &         23 &      17.30 &       0.87 &      16.00 &       0.80 &      12.60 &       0.73 &      15.00 &       0.85 &      137.9 &        8.1 &      108.0 &        5.6 \\
       376 &      189.384415 &       62.242168 &         28 &      23.80 &       1.19 &      19.90 &       1.00 &      15.20 &       0.86 &      25.80 &       1.37 &       62.6 &        6.3 &       75.2 &        5.6 \\
       377 &      189.365921 &       62.243626 &         26 &      55.50 &       2.78 &      40.30 &       2.02 &      34.80 &       1.79 &      31.10 &       1.63 &      263.3 &       11.7 &      338.0 &        6.1 \\
       378 &      189.040649 &       62.239590 &         25 &      66.80 &       3.34 &      41.90 &       2.10 &      41.60 &       2.12 &      29.40 &       1.55 &      281.1 &       12.8 &      294.0 &        5.7 \\
       379 &      189.269363 &       62.241432 &         16 &      62.40 &       3.12 &      42.50 &       2.13 &      40.00 &       2.02 &      35.80 &       1.83 &      131.3 &       13.1 &      173.0 &        4.7 \\
       380 &      189.403641 &       62.241379 &         35 &      10.70 &       0.54 &      12.40 &       0.62 &      16.30 &       0.91 &      24.60 &       1.32 &       77.8 &        8.9 &      119.0 &        4.9 \\
       381 &      189.125366 &       62.241077 &         33 &      41.00 &       2.05 &      43.40 &       2.17 &      34.20 &       1.75 &      29.00 &       1.52 &      111.0 &        8.7 &      188.0 &        5.8 \\
       382 &      189.262192 &       62.239883 &         25 &      65.50 &       3.28 &      48.50 &       2.43 &      39.30 &       1.99 &      39.40 &       2.00 &       85.1 &       13.3 &      108.0 &        5.8 \\
       383 &      189.395691 &       62.240860 &         38 &      21.00 &       1.05 &      17.30 &       0.87 &      12.60 &       0.75 &      13.50 &       0.82 &      134.5 &        9.2 &      120.0 &        5.1 \\
       384 &      189.201279 &       62.240707 &         24 &      86.00 &       4.30 &      59.80 &       2.99 &      56.40 &       2.84 &     381.00 &      19.05 &      309.3 &       13.5 &      454.0 &        5.7 \\
       385 &      189.226639 &       62.242863 &         37 &      10.90 &       0.55 &       7.93 &       0.40 &       9.18 &       0.55 &       8.98 &       0.56 &       62.6 &        7.0 &      101.0 &        5.4 \\
       386 &      189.399765 &       62.240498 &         40 &      13.00 &       0.65 &      10.30 &       0.52 &       7.63 &       0.56 &       6.33 &       0.57 &       44.8 &        8.0 &       42.4 &        4.1 \\
       387 &      189.046906 &       62.239117 &         20 &      35.10 &       1.76 &      23.50 &       1.18 &      21.50 &       1.16 &      20.90 &       1.16 &       88.2 &        9.8 &      147.0 &        6.2 \\
       388 &      188.999542 &       62.239689 &         19 &     117.00 &       5.85 &      81.40 &       4.07 &      59.70 &       3.02 &      44.10 &       2.27 &      128.1 &       14.2 &      214.0 &        6.9 \\
       389 &      189.148315 &       62.239990 &         31 &      64.90 &       3.25 &      97.30 &       4.87 &     172.00 &       8.61 &     284.00 &      14.21 &      680.4 &       27.8 &     1520.0 &       14.4 \\
       390 &      189.161987 &       62.239784 &         29 &      23.10 &       1.16 &      16.10 &       0.81 &      13.80 &       0.77 &      11.80 &       0.70 &       76.1 &        8.3 &       82.9 &        5.9 \\
       391 &      189.370926 &       62.241653 &         31 &      15.60 &       0.78 &      12.40 &       0.62 &      11.30 &       0.70 &      11.10 &       0.73 &       98.0 &       10.2 &       91.3 &        5.2 \\
       392 &      189.371674 &       62.240124 &         30 &      24.30 &       1.22 &      19.00 &       0.95 &      17.70 &       0.98 &      15.80 &       0.92 &      142.6 &        8.9 &      100.0 &        6.9 \\
       393 &      189.457153 &       62.239513 &         24 &      76.00 &       3.80 &      60.40 &       3.02 &      48.40 &       2.46 &      80.40 &       4.06 &      213.8 &        9.6 &      247.0 &        4.7 \\
       394 &      189.283951 &       62.239620 &         23 &     122.00 &       6.10 &      80.70 &       4.04 &      66.70 &       3.35 &      41.50 &       2.11 &       85.1 &       15.4 &       84.3 &        6.8 \\
       395 &      189.058289 &       62.237572 &         23 &      60.30 &       3.02 &      49.60 &       2.48 &      38.00 &       1.95 &     210.00 &      10.51 &      249.2 &       11.1 &      251.0 &        6.6 \\
       396 &      189.171555 &       62.239185 &         33 &      20.40 &       1.02 &      15.40 &       0.77 &      12.60 &       0.71 &      15.20 &       0.85 &       65.6 &        8.0 &       50.5 &        5.8 \\
       397 &      189.361252 &       62.238598 &         32 &      49.30 &       2.47 &      41.60 &       2.08 &      29.20 &       1.52 &      24.70 &       1.32 &      130.6 &        9.4 &      136.0 &        6.7 \\
       398 &      189.384842 &       62.238503 &         34 &      34.90 &       1.75 &      30.50 &       1.53 &      21.00 &       1.13 &      21.30 &       1.16 &      130.9 &       10.0 &      114.0 &        4.5 \\
       399 &      189.274490 &       62.239799 &         14 &      60.70 &       3.04 &      43.80 &       2.19 &      33.40 &       1.70 &      25.70 &       1.34 &      125.3 &       11.3 &      155.0 &        5.2 \\
       400 &      189.091568 &       62.237598 &         18 &      25.00 &       1.25 &      23.60 &       1.18 &      17.90 &       0.99 &      18.80 &       1.06 &      146.9 &       12.2 &       97.9 &        5.6 \\
       401 &      189.201202 &       62.238007 &         25 &      11.30 &       0.57 &      11.60 &       0.58 &      14.50 &       0.78 &      13.80 &       0.77 &       49.5 &        7.8 &      165.0 &        6.3 \\
       402 &      189.315491 &       62.237980 &         24 &      17.00 &       0.85 &      11.30 &       0.57 &      12.50 &       0.72 &       8.65 &       0.60 &       77.1 &       10.0 &       76.6 &        6.1 \\
       403 &      189.088852 &       62.238106 &         18 &      77.60 &       3.88 &      56.60 &       2.83 &      49.60 &       2.52 &      42.40 &       2.18 &      119.1 &       11.5 &      119.0 &        5.7 \\
       404 &      189.072586 &       62.237888 &         22 &      23.50 &       1.18 &      16.60 &       0.83 &      12.10 &       0.73 &      49.80 &       2.54 &       63.6 &       11.5 &       80.7 &        6.1 \\
       405 &      189.206268 &       62.235207 &         36 &      35.80 &       1.79 &      22.90 &       1.15 &      23.90 &       1.23 &      17.90 &       0.96 &      147.7 &       10.0 &      186.0 &        7.1 \\
       406 &      189.442200 &       62.236988 &         23 &      69.90 &       3.50 &      47.40 &       2.37 &      36.20 &       1.86 &      27.70 &       1.48 &      137.0 &       10.9 &      172.0 &        5.8 \\
       407 &      189.144348 &       62.239285 &         37 &       9.21 &       0.46 &      10.90 &       0.55 &      10.60 &       0.64 &      12.40 &       0.74 &       50.0 &       10.5 &      101.0 &        7.2 \\
       408 &      189.196564 &       62.237289 &         22 &       7.24 &       0.36 &       5.08 &       0.26 &       4.93 &       0.39 &       3.43 &       0.39 &       43.1 &        8.0 &       22.8 &        6.4 \\
       409 &      189.345566 &       62.238811 &         34 &      33.90 &       1.70 &      25.60 &       1.28 &      19.80 &       1.07 &      17.70 &       1.01 &      140.5 &        9.2 &      147.0 &        5.7 \\
       410 &      189.000702 &       62.235790 &         22 &     109.00 &       5.45 &      73.90 &       3.70 &      66.30 &       3.35 &     375.00 &      18.76 &      281.1 &       12.9 &      335.0 &        7.8 \\
       411 &      189.459335 &       62.233067 &         10 &      17.40 &       0.87 &      20.00 &       1.00 &      20.00 &       1.10 &      22.00 &       1.24 &      108.2 &       14.8 &       74.3 &        7.2 \\
       412 &      189.468399 &       62.235588 &         13 &      25.80 &       1.29 &      20.80 &       1.04 &      15.00 &       0.88 &      16.10 &       1.00 &      156.3 &       14.2 &      121.0 &        5.7 \\
       413 &      189.074066 &       62.235508 &         25 &      51.20 &       2.56 &      55.40 &       2.77 &      49.90 &       2.53 &      39.00 &       2.01 &      137.5 &        9.8 &      429.0 &        7.4 \\
       414 &      189.239090 &       62.235538 &         33 &      23.00 &       1.15 &      25.40 &       1.27 &      21.30 &       1.11 &      18.60 &       0.99 &      113.6 &       13.5 &      115.0 &        5.8 \\
       415 &      189.135895 &       62.235485 &         45 &      18.40 &       0.92 &      20.50 &       1.03 &      17.20 &       0.94 &      18.10 &       1.01 &      144.6 &       10.2 &      109.0 &        4.8 \\
       416 &      189.405426 &       62.236469 &         28 &      25.50 &       1.28 &      16.70 &       0.84 &      16.20 &       0.91 &      10.70 &       0.71 &       94.5 &        9.4 &      124.0 &        5.9 \\
       417 &      189.252182 &       62.234951 &         24 &      43.60 &       2.18 &      35.20 &       1.76 &      25.70 &       1.32 &      36.70 &       1.87 &       98.2 &       11.5 &      121.0 &        6.4 \\
       418 &      189.105789 &       62.234650 &         40 &     704.00 &      35.20 &     490.00 &      24.50 &     341.00 &      17.06 &     181.00 &       9.06 &       55.2 &        7.2 &       24.3 &        6.9 \\
       419 &      189.193085 &       62.234627 &         22 &      92.00 &       4.60 &      82.80 &       4.14 &      87.40 &       4.38 &     100.00 &       5.01 &      130.3 &       11.1 &      213.0 &        5.2 \\
       420 &      189.262161 &       62.234688 &         19 &      14.90 &       0.75 &      15.20 &       0.76 &      12.60 &       0.70 &      16.70 &       0.91 &       88.6 &       13.3 &       20.7 &        7.8 \\
       421 &      189.124847 &       62.234180 &         27 &      34.90 &       1.75 &      22.60 &       1.13 &      22.40 &       1.19 &      13.90 &       0.84 &      125.3 &        9.4 &      124.0 &        6.5 \\
       422 &      189.153122 &       62.234268 &         29 &       5.61 &       0.28 &       3.79 &       0.20 &       3.96 &       0.41 &       3.13 &       0.44 &       44.8 &        5.7 &       33.2 &        4.8 \\
       423 &      189.409485 &       62.233479 &         27 &      24.70 &       1.24 &      19.00 &       0.95 &      18.70 &       1.02 &      23.80 &       1.28 &       55.9 &        9.2 &      115.0 &        6.0 \\
       424 &      189.073181 &       62.233917 &         28 &      13.40 &       0.67 &       8.28 &       0.42 &       8.83 &       0.60 &       5.74 &       0.57 &       54.6 &        9.8 &       27.5 &        4.9 \\
       425 &      189.261414 &       62.233768 &         21 &      55.40 &       2.77 &      51.70 &       2.59 &      36.70 &       1.86 &      44.20 &       2.24 &      441.9 &       17.8 &      349.0 &        8.8 \\
       426 &      189.142838 &       62.233463 &         33 &      36.30 &       1.82 &      37.40 &       1.87 &      28.60 &       1.48 &      27.90 &       1.46 &      247.4 &       11.7 &      161.0 &        5.5 \\
       427 &      189.334778 &       62.231457 &         31 &      36.60 &       1.83 &      26.00 &       1.30 &      23.20 &       1.22 &      17.70 &       0.99 &      123.6 &        9.8 &      140.0 &        5.2 \\
       428 &      188.983978 &       62.234104 &         21 &      55.60 &       2.78 &      41.80 &       2.09 &      29.90 &       1.57 &      24.00 &       1.32 &       63.0 &        8.0 &       59.9 &        6.0 \\
       429 &      188.992462 &       62.231674 &         35 &      42.10 &       2.11 &      38.40 &       1.92 &      31.10 &       1.62 &      29.80 &       1.58 &      175.1 &        8.1 &      125.0 &        7.5 \\
       430 &      189.344055 &       62.232433 &         36 &      42.80 &       2.14 &      32.40 &       1.62 &      24.20 &       1.27 &      28.40 &       1.50 &      300.5 &        9.2 &      317.0 &        6.2 \\
       431 &      189.321991 &       62.232368 &         25 &      15.20 &       0.76 &      12.60 &       0.63 &       8.56 &       0.55 &      17.60 &       0.97 &       59.2 &        7.4 &       55.3 &        5.5 \\
       432 &      188.947754 &       62.231739 &         10 &      29.50 &       1.48 &      33.20 &       1.66 &      25.40 &       1.40 &      26.00 &       1.44 &      135.9 &       15.7 &      168.0 &        6.6 \\
       433 &      189.397568 &       62.231716 &         28 &      27.80 &       1.39 &      30.10 &       1.51 &      23.50 &       1.24 &      22.80 &       1.23 &       97.0 &        7.6 &       63.1 &        4.6 \\
       434 &      189.082092 &       62.231434 &         23 &      41.20 &       2.06 &      32.30 &       1.62 &      19.90 &       1.08 &      23.70 &       1.28 &       48.7 &        7.6 &       29.0 &        5.8 \\
       435 &      189.215790 &       62.231628 &         20 &      47.70 &       2.39 &      35.90 &       1.80 &      36.90 &       1.87 &      41.30 &       2.09 &      174.9 &        9.8 &      202.0 &        6.0 \\
       436 &      189.219803 &       62.231850 &         22 &      14.70 &       0.74 &      14.50 &       0.73 &      10.90 &       0.62 &      12.60 &       0.72 &       62.6 &       13.3 &       97.3 &        5.4 \\
       437 &      189.225418 &       62.231770 &         20 &      13.00 &       0.65 &       8.49 &       0.43 &       7.56 &       0.48 &       5.12 &       0.43 &       65.2 &        9.2 &       51.4 &        5.9 \\
       438 &      189.317719 &       62.229687 &         24 &      19.90 &       1.00 &      16.80 &       0.84 &      12.10 &       0.69 &      26.00 &       1.36 &       80.0 &        8.9 &       98.3 &        4.7 \\
       439 &      189.321487 &       62.231167 &         27 &      18.80 &       0.94 &      16.20 &       0.81 &      11.70 &       0.68 &      13.30 &       0.78 &       85.7 &        7.2 &       72.7 &        5.3 \\
       440 &      189.393921 &       62.232323 &         25 &      94.90 &       4.75 &      64.00 &       3.20 &      55.20 &       2.79 &      40.70 &       2.09 &      249.2 &       10.0 &      306.0 &        6.2 \\
       441 &      188.953049 &       62.231743 &         21 &      14.80 &       0.74 &      10.00 &       0.51 &       9.38 &       0.73 &       6.24 &       0.68 &       55.2 &       11.1 &       62.4 &        6.7 \\
       442 &      188.959579 &       62.231655 &         34 &      27.90 &       1.40 &      20.40 &       1.02 &      20.10 &       1.14 &      16.40 &       1.00 &      175.9 &       11.7 &      207.0 &        6.6 \\
       443 &      189.082718 &       62.229927 &         28 &      29.10 &       1.46 &      22.60 &       1.13 &      22.10 &       1.18 &      27.50 &       1.46 &      107.4 &        8.1 &      119.0 &        6.3 \\
       444 &      189.359238 &       62.229717 &         43 &      99.50 &       4.98 &      71.70 &       3.59 &      54.90 &       2.77 &      32.90 &       1.72 &       40.1 &        5.0 &       25.6 &        6.7 \\
       445 &      189.179825 &       62.229851 &         38 &      10.20 &       0.51 &       9.08 &       0.46 &       6.59 &       0.46 &       6.39 &       0.49 &       44.0 &        6.7 &       34.4 &        5.5 \\
       446 &      189.265686 &       62.231167 &         21 &      26.10 &       1.31 &      18.40 &       0.92 &      14.50 &       0.79 &      12.60 &       0.72 &      104.1 &       12.4 &       93.4 &        6.5 \\
       447 &      189.096115 &       62.229473 &         26 &      42.60 &       2.13 &      38.10 &       1.91 &      34.20 &       1.76 &      72.90 &       3.68 &      236.9 &       11.8 &      288.0 &        8.5 \\
       448 &      189.152771 &       62.229618 &         63 &      70.30 &       3.52 &      73.50 &       3.68 &      87.80 &       4.41 &     106.00 &       5.32 &      341.1 &       10.5 &      475.0 &        5.8 \\
       449 &      189.366257 &       62.229485 &         45 &      21.00 &       1.05 &      24.30 &       1.22 &      23.40 &       1.24 &      17.50 &       1.00 &       56.4 &        8.0 &      258.0 &        5.6 \\
       450 &      189.185532 &       62.229828 &         37 &      13.20 &       0.66 &      12.10 &       0.61 &       8.55 &       0.53 &       8.29 &       0.55 &       54.6 &        6.8 &       43.9 &        5.3 \\
       451 &      189.389069 &       62.227852 &         29 &      61.00 &       3.05 &      41.70 &       2.09 &      31.70 &       1.64 &     110.00 &       5.52 &       89.6 &       11.5 &      157.0 &        5.9 \\
       452 &      189.415756 &       62.227131 &         31 &      96.40 &       4.82 &      65.80 &       3.29 &      53.20 &       2.69 &      40.50 &       2.08 &       87.0 &        8.9 &      106.0 &        5.4 \\
       453 &      189.452560 &       62.229092 &         10 &      36.20 &       1.81 &      25.00 &       1.25 &      21.40 &       1.16 &      17.10 &       1.04 &      155.2 &       17.0 &      206.0 &        6.4 \\
       454 &      189.339371 &       62.229511 &         39 &      45.60 &       2.28 &      36.20 &       1.81 &      27.10 &       1.40 &      27.00 &       1.42 &      212.1 &        9.1 &      235.0 &        7.5 \\
       455 &      189.338028 &       62.228718 &         40 &      16.60 &       0.83 &      11.90 &       0.60 &      10.10 &       0.62 &      11.20 &       0.71 &       39.9 &        7.6 &       18.0 &        5.8 \\
       456 &      189.336914 &       62.227867 &         34 &      11.30 &       0.57 &       8.34 &       0.42 &       6.24 &       0.47 &       6.39 &       0.54 &       55.9 &        8.7 &       50.9 &        4.7 \\
       457 &      189.260437 &       62.228317 &         26 &      12.60 &       0.63 &       9.24 &       0.46 &       8.73 &       0.53 &       8.86 &       0.57 &       49.7 &       11.1 &       34.3 &        6.0 \\
       458 &      189.294159 &       62.228237 &         24 &      13.30 &       0.67 &       8.87 &       0.45 &       9.19 &       0.56 &       7.36 &       0.52 &       58.3 &        9.1 &       82.6 &        9.7 \\
       459 &      189.152115 &       62.228008 &         57 &      52.60 &       2.63 &      37.20 &       1.86 &      35.90 &       1.83 &      32.10 &       1.66 &       90.8 &        9.8 &      101.0 &        4.6 \\
       460 &      189.008545 &       62.227562 &         28 &      25.30 &       1.27 &      17.70 &       0.89 &      15.30 &       0.88 &      12.80 &       0.83 &      129.3 &        8.0 &      161.0 &        7.1 \\
       461 &      189.160431 &       62.227486 &         53 &      45.70 &       2.29 &      34.10 &       1.71 &      23.50 &       1.23 &      20.40 &       1.10 &       44.2 &        5.6 &       47.3 &        6.0 \\
       462 &      189.331863 &       62.227051 &         35 &      85.30 &       4.27 &      66.10 &       3.31 &      53.60 &       2.70 &      70.70 &       3.56 &      150.2 &        7.8 &      187.0 &        4.8 \\
       463 &      188.974442 &       62.227036 &         23 &      66.00 &       3.30 &      48.80 &       2.44 &      46.40 &       2.37 &      38.60 &       2.00 &      424.1 &       13.9 &      553.0 &       13.0 \\
       464 &      188.970474 &       62.227997 &         26 &      36.30 &       1.82 &      25.80 &       1.29 &      22.30 &       1.21 &      18.50 &       1.07 &      162.8 &       11.8 &      217.0 &        8.0 \\
       465 &      189.307800 &       62.226444 &         22 &      23.80 &       1.19 &      15.20 &       0.76 &      14.00 &       0.77 &      10.10 &       0.63 &       75.9 &       12.4 &       74.6 &        5.7 \\
       466 &      189.044052 &       62.226196 &         26 &      19.60 &       0.98 &      12.80 &       0.64 &      12.70 &       0.77 &       9.88 &       0.72 &       67.5 &       10.2 &       75.9 &        5.6 \\
       467 &      189.155228 &       62.226192 &         59 &      29.80 &       1.49 &      21.50 &       1.08 &      20.30 &       1.08 &      13.90 &       0.82 &      116.3 &        8.5 &      109.0 &        5.6 \\
       468 &      189.304626 &       62.226044 &         19 &      13.60 &       0.68 &       9.08 &       0.46 &       8.74 &       0.54 &       6.46 &       0.50 &       76.7 &       10.9 &       80.4 &        6.9 \\
       469 &      188.982758 &       62.225739 &         22 &      18.40 &       0.92 &      17.30 &       0.87 &      11.00 &       0.71 &      14.00 &       0.88 &      122.3 &        8.3 &       81.4 &        6.1 \\
       470 &      189.175430 &       62.225384 &         49 &       7.16 &       0.36 &       8.73 &       0.44 &      12.30 &       0.70 &      11.40 &       0.69 &       58.1 &        7.6 &      209.0 &        5.6 \\
       471 &      189.360107 &       62.225082 &         32 &      24.00 &       1.20 &      25.80 &       1.29 &      21.70 &       1.15 &      14.30 &       0.86 &       47.9 &        6.7 &       88.5 &        5.1 \\
       472 &      189.364059 &       62.225861 &         36 &       5.87 &       0.30 &       6.47 &       0.33 &       5.35 &       0.48 &       3.71 &       0.52 &       35.6 &        5.6 &       41.6 &        5.3 \\
       473 &      189.275925 &       62.225780 &         19 &      24.80 &       1.24 &      16.50 &       0.83 &      16.10 &       0.86 &      11.10 &       0.66 &       66.9 &        9.8 &       71.7 &        6.5 \\
       474 &      189.402115 &       62.225536 &         29 &      38.90 &       1.95 &      25.90 &       1.30 &      20.40 &       1.10 &      14.60 &       0.87 &       46.5 &        8.9 &       63.0 &        5.6 \\
       475 &      189.297272 &       62.225307 &         27 &      39.10 &       1.96 &      44.80 &       2.24 &      51.80 &       2.61 &      36.30 &       1.85 &       92.5 &        8.3 &      537.0 &        9.3 \\
       476 &      189.167938 &       62.225273 &         47 &      20.10 &       1.01 &      16.20 &       0.81 &      14.70 &       0.81 &      23.50 &       1.24 &       68.4 &        7.2 &      125.0 &        5.6 \\
       477 &      189.257721 &       62.225140 &         30 &      18.60 &       0.93 &      16.70 &       0.84 &      11.50 &       0.65 &      12.10 &       0.70 &       87.3 &        9.6 &       76.0 &        6.9 \\
       478 &      189.168808 &       62.226318 &         41 &      14.80 &       0.74 &      15.70 &       0.79 &      13.10 &       0.74 &      13.70 &       0.79 &       61.5 &        7.6 &       77.4 &        5.6 \\
       479 &      189.029755 &       62.224644 &         20 &      62.10 &       3.11 &      52.60 &       2.63 &      44.20 &       2.25 &      85.80 &       4.32 &      203.2 &       12.6 &      260.0 &        6.6 \\
       480 &      189.378784 &       62.224438 &         31 &      20.40 &       1.02 &      15.20 &       0.76 &      13.30 &       0.78 &      13.00 &       0.81 &      101.3 &       10.2 &       67.6 &        6.1 \\
       481 &      188.938080 &       62.223530 &         27 &      18.80 &       0.94 &      17.30 &       0.87 &      12.90 &       0.85 &      11.00 &       0.81 &       55.3 &        9.8 &        0.0 &        0.0 \\
       482 &      189.376266 &       62.223972 &         30 &      43.70 &       2.19 &      32.20 &       1.61 &      25.60 &       1.34 &      27.40 &       1.45 &      245.7 &       10.5 &      281.0 &        7.2 \\
       483 &      189.299973 &       62.223816 &         26 &       9.45 &       0.47 &      11.50 &       0.58 &      15.70 &       0.85 &      11.60 &       0.69 &       47.4 &        7.6 &      219.0 &        6.6 \\
       484 &      189.039612 &       62.223057 &         19 &      10.70 &       0.54 &       7.99 &       0.41 &       6.05 &       0.53 &       6.33 &       0.61 &       74.1 &       13.1 &       76.1 &        6.3 \\
       485 &      189.251236 &       62.223232 &         38 &       8.42 &       0.42 &       9.36 &       0.47 &       7.16 &       0.47 &       8.83 &       0.57 &       65.9 &       10.5 &       48.7 &        6.8 \\
       486 &      189.258484 &       62.223061 &         34 &      24.00 &       1.20 &      19.60 &       0.98 &      13.60 &       0.75 &      24.40 &       1.27 &       53.2 &        8.9 &       46.4 &        6.6 \\
       487 &      189.204437 &       62.222736 &         22 &      13.70 &       0.69 &      10.10 &       0.51 &       7.77 &       0.49 &       7.47 &       0.52 &       51.4 &        9.4 &       62.3 &        6.6 \\
       488 &      189.327744 &       62.222675 &         26 &      48.40 &       2.42 &      37.60 &       1.88 &      30.40 &       1.56 &      44.00 &       2.24 &      105.7 &        9.4 &      146.0 &        5.6 \\
       489 &      189.212814 &       62.222389 &         20 &      35.50 &       1.78 &      26.30 &       1.32 &      18.30 &       0.96 &      67.50 &       3.39 &       76.0 &       15.7 &       81.1 &        6.4 \\
       490 &      188.956879 &       62.221489 &         18 &      23.00 &       1.15 &      17.40 &       0.87 &      15.20 &       0.89 &      15.20 &       0.94 &       60.1 &       11.7 &       51.7 &        6.2 \\
       491 &      189.091293 &       62.223125 &         22 &      27.40 &       1.37 &      25.10 &       1.26 &      15.70 &       0.89 &      16.60 &       0.96 &      115.8 &       11.3 &       85.8 &        6.1 \\
       492 &      189.139999 &       62.222183 &         56 &      53.40 &       2.67 &      35.50 &       1.78 &      36.00 &       1.85 &      24.70 &       1.32 &      281.1 &        9.6 &      320.0 &        6.0 \\
       493 &      189.060287 &       62.221916 &         28 &      81.50 &       4.08 &      62.30 &       3.12 &      48.50 &       2.46 &      54.90 &       2.79 &      147.7 &        9.2 &      160.0 &        6.6 \\
       494 &      189.207169 &       62.220264 &         24 &      41.10 &       2.06 &      40.40 &       2.02 &      36.50 &       1.85 &      94.80 &       4.75 &      236.9 &       13.7 &      337.0 &       10.9 \\
       495 &      189.206177 &       62.221333 &         22 &      25.70 &       1.29 &      24.60 &       1.23 &      18.60 &       0.98 &      29.90 &       1.54 &      134.6 &       14.2 &       66.0 &        7.9 \\
       496 &      189.210251 &       62.221138 &         20 &      26.80 &       1.34 &      19.30 &       0.97 &      20.70 &       1.08 &      19.80 &       1.05 &      199.7 &       14.8 &      199.0 &        5.7 \\
       497 &      189.143158 &       62.220112 &         52 &      15.00 &       0.75 &      10.50 &       0.53 &      11.00 &       0.69 &       7.93 &       0.61 &       88.8 &        6.8 &       84.9 &        5.0 \\
       498 &      189.177933 &       62.218437 &         45 &      33.20 &       1.66 &      28.20 &       1.41 &      20.90 &       1.10 &      23.50 &       1.24 &      110.7 &        7.2 &      202.0 &        4.2 \\
       499 &      189.171387 &       62.220676 &         46 &      14.80 &       0.74 &      10.50 &       0.53 &       8.25 &       0.54 &       6.89 &       0.54 &       59.2 &        6.3 &       59.9 &        4.3 \\
       500 &      189.319672 &       62.219501 &         28 &      14.80 &       0.74 &       9.79 &       0.49 &       8.90 &       0.55 &       5.85 &       0.48 &       81.0 &        8.7 &       91.1 &        5.5 \\
       501 &      189.344818 &       62.219322 &         22 &      15.10 &       0.76 &      17.70 &       0.89 &      14.40 &       0.80 &      13.40 &       0.79 &       48.9 &        8.9 &      130.0 &        5.3 \\
       502 &      188.949799 &       62.218903 &         20 &      30.80 &       1.54 &      23.10 &       1.16 &      19.90 &       1.10 &      16.90 &       1.01 &       79.4 &       13.1 &      128.0 &        5.7 \\
       503 &      189.004105 &       62.217224 &         20 &      22.80 &       1.14 &      19.10 &       0.96 &      14.70 &       0.86 &      20.80 &       1.17 &      198.0 &       15.5 &      142.0 &        6.4 \\
       504 &      188.939316 &       62.218460 &         17 &       9.54 &       0.48 &       9.90 &       0.50 &       7.32 &       0.62 &       6.48 &       0.65 &       61.4 &       12.4 &       32.0 &        6.7 \\
       505 &      189.142319 &       62.218277 &         43 &      15.40 &       0.77 &      12.00 &       0.60 &      13.50 &       0.79 &      10.80 &       0.71 &      128.3 &        5.9 &      135.0 &        5.9 \\
       506 &      189.185852 &       62.217926 &         49 &      41.80 &       2.09 &      33.10 &       1.66 &      27.00 &       1.39 &      35.10 &       1.80 &       89.0 &        8.9 &      110.0 &        4.8 \\
       507 &      189.382492 &       62.217606 &         42 &      38.60 &       1.93 &      28.70 &       1.44 &      25.50 &       1.34 &      21.40 &       1.18 &      206.8 &        7.6 &      250.0 &        5.7 \\
       508 &      189.113800 &       62.216068 &         34 &      25.70 &       1.29 &      22.50 &       1.13 &      15.20 &       0.87 &      17.70 &       1.01 &      158.9 &        8.0 &      140.0 &        6.8 \\
       509 &      189.089874 &       62.216747 &         14 &      40.70 &       2.04 &      25.80 &       1.29 &      26.40 &       1.38 &      18.10 &       1.03 &      119.3 &       11.1 &      120.0 &        6.3 \\
       510 &      189.396774 &       62.216373 &         27 &      28.80 &       1.44 &      32.00 &       1.60 &      25.50 &       1.34 &      24.50 &       1.33 &      145.6 &       13.1 &      122.0 &        4.9 \\
       511 &      189.396347 &       62.218594 &         33 &      23.50 &       1.18 &      15.60 &       0.78 &      13.80 &       0.81 &      13.90 &       0.86 &       51.1 &        9.4 &       43.1 &        4.5 \\
       512 &      189.079758 &       62.217171 &         18 &      26.20 &       1.31 &      24.60 &       1.23 &      18.00 &       0.99 &      23.10 &       1.26 &      236.9 &       13.9 &      220.0 &        8.2 \\
       513 &      189.206848 &       62.215981 &         26 &      20.40 &       1.02 &      18.60 &       0.93 &      15.40 &       0.83 &      33.00 &       1.69 &       81.8 &       10.4 &      108.0 &        6.0 \\
       514 &      189.331696 &       62.215622 &         17 &      22.20 &       1.11 &      15.40 &       0.77 &      13.20 &       0.74 &      12.00 &       0.71 &       93.1 &        9.8 &      147.0 &        6.5 \\
       515 &      189.231552 &       62.212631 &         27 &      22.80 &       1.14 &      14.40 &       0.72 &      13.40 &       0.74 &       8.06 &       0.54 &       67.7 &        9.2 &       69.6 &        7.3 \\
       516 &      189.224579 &       62.215008 &         33 &      61.50 &       3.08 &      39.60 &       1.98 &      39.90 &       2.02 &      28.90 &       1.49 &      162.8 &        9.6 &      200.0 &        6.4 \\
       517 &      189.081314 &       62.214569 &         17 &     113.00 &       5.65 &      95.30 &       4.77 &      92.20 &       4.63 &     161.00 &       8.07 &      539.1 &       21.8 &      971.0 &       10.9 \\
       518 &      189.110931 &       62.214462 &         36 &      32.90 &       1.65 &      23.30 &       1.17 &      21.80 &       1.17 &      20.20 &       1.12 &       92.5 &        9.1 &       85.2 &        6.7 \\
       519 &      189.176743 &       62.214539 &         63 &      12.90 &       0.65 &      11.40 &       0.57 &       8.04 &       0.54 &       7.81 &       0.58 &       58.5 &        6.5 &       52.7 &        6.7 \\
       520 &      189.284790 &       62.214619 &         21 &      20.60 &       1.03 &      13.20 &       0.66 &      11.90 &       0.67 &       8.21 &       0.54 &       74.4 &        9.6 &       80.4 &        6.0 \\
       521 &      189.390335 &       62.214085 &         27 &       9.58 &       0.48 &       7.27 &       0.37 &       5.51 &       0.49 &       5.20 &       0.58 &       73.0 &        6.3 &       58.9 &        5.7 \\
       522 &      189.161957 &       62.215908 &         45 &      59.90 &       3.00 &      50.00 &       2.50 &      35.60 &       1.82 &      34.00 &       1.76 &      261.6 &        8.9 &      236.0 &        4.7 \\
       523 &      189.183273 &       62.213894 &         57 &      54.20 &       2.71 &      42.30 &       2.12 &      49.50 &       2.50 &      59.70 &       3.01 &      284.6 &        9.4 &      434.0 &        5.8 \\
       524 &      189.335815 &       62.213673 &         18 &      40.80 &       2.04 &      27.20 &       1.36 &      26.00 &       1.34 &     146.00 &       7.31 &       73.9 &       17.0 &       92.7 &        6.7 \\
       525 &      189.338730 &       62.213097 &         16 &     382.00 &       0.11 &     257.00 &       0.14 &     211.00 &       0.64 &     994.00 &       0.68 &      487.8 &       34.2 &      584.0 &       13.3 \\
       526 &      189.325302 &       62.213390 &         19 &      32.60 &       1.63 &      23.10 &       1.16 &      19.70 &       1.04 &      15.70 &       0.87 &      173.5 &        8.3 &      188.0 &        6.1 \\
       527 &      189.146973 &       62.213165 &         49 &       8.01 &       0.40 &       9.68 &       0.49 &       7.22 &       0.54 &       5.85 &       0.54 &       38.3 &        7.6 &       33.3 &        3.9 \\
       528 &      189.236069 &       62.212677 &         30 &      85.80 &       4.29 &      58.50 &       2.93 &      46.20 &       2.33 &      28.40 &       1.47 &       54.0 &        9.6 &       22.2 &        7.1 \\
       529 &      189.383865 &       62.212894 &         32 &      96.00 &       4.80 &      71.60 &       3.58 &      51.10 &       2.59 &      39.00 &       2.01 &      109.9 &        7.4 &      137.0 &        5.5 \\
       530 &      188.995636 &       62.213108 &         29 &      14.40 &       0.72 &      10.30 &       0.52 &       7.12 &       0.57 &       8.04 &       0.66 &       67.5 &        8.3 &       70.5 &        5.3 \\
       531 &      189.209320 &       62.211033 &         46 &      28.80 &       1.44 &      24.20 &       1.21 &      18.10 &       0.96 &      34.00 &       1.74 &       96.0 &        8.7 &      130.0 &        7.1 \\
       532 &      188.974014 &       62.212692 &         31 &      16.60 &       0.83 &      11.80 &       0.59 &      10.30 &       0.68 &       8.44 &       0.68 &       65.6 &       11.3 &       74.7 &        5.6 \\
       533 &      189.136520 &       62.212196 &         37 &      49.50 &       2.48 &      35.30 &       1.77 &      33.60 &       1.73 &      28.40 &       1.50 &      107.6 &        6.3 &      121.0 &        7.3 \\
       534 &      189.156830 &       62.211353 &         41 &      20.90 &       1.05 &      17.80 &       0.89 &      12.60 &       0.75 &      21.50 &       1.17 &       73.5 &        8.3 &       65.4 &        3.7 \\
       535 &      189.336441 &       62.211849 &         19 &      31.30 &       1.57 &      21.20 &       1.06 &      23.80 &       1.23 &     158.00 &       7.91 &      160.3 &       21.8 &      213.0 &        7.7 \\
       536 &      189.143799 &       62.211391 &         44 &      64.50 &       3.23 &      71.30 &       3.57 &      58.00 &       2.93 &      70.50 &       3.55 &      922.6 &       23.1 &      444.0 &        5.5 \\
       537 &      189.166397 &       62.213875 &         51 &      58.30 &       2.92 &      40.00 &       2.00 &      42.60 &       2.16 &      32.00 &       1.66 &      418.8 &       13.3 &      511.0 &        6.8 \\
       538 &      189.283401 &       62.211205 &         23 &      26.50 &       1.33 &      23.60 &       1.18 &      14.30 &       0.78 &      12.30 &       0.71 &       83.8 &       11.3 &       53.7 &        6.8 \\
       539 &      189.377899 &       62.211014 &         32 &       8.48 &       0.43 &       6.52 &       0.33 &       6.64 &       0.50 &       7.12 &       0.60 &       57.9 &        8.0 &       58.7 &        6.0 \\
       540 &      189.117737 &       62.210419 &         39 &      20.90 &       1.05 &      16.50 &       0.83 &      14.50 &       0.83 &      17.30 &       0.99 &       58.9 &        6.7 &       56.1 &        6.8 \\
       541 &      189.066223 &       62.210365 &         18 &      59.50 &       2.98 &      54.70 &       2.74 &      38.00 &       1.95 &     147.00 &       7.37 &      318.1 &       13.5 &      391.0 &        6.4 \\
       542 &      189.085495 &       62.210579 &         21 &      18.60 &       0.93 &      18.80 &       0.94 &      14.00 &       0.82 &      13.00 &       0.82 &       83.3 &       11.8 &       58.7 &        7.0 \\
       543 &      189.291199 &       62.210632 &         31 &      74.70 &       3.74 &      43.80 &       2.19 &      43.30 &       2.19 &      37.70 &       1.92 &      176.2 &       10.5 &      218.0 &        6.5 \\
       544 &      189.093155 &       62.211483 &         19 &      47.80 &       2.39 &      36.40 &       1.82 &      29.90 &       1.55 &      36.60 &       1.89 &       72.6 &       11.5 &       91.3 &        6.1 \\
       545 &      189.092438 &       62.210335 &         18 &      35.70 &       1.79 &      24.30 &       1.22 &      24.00 &       1.27 &      21.50 &       1.18 &       70.7 &       11.1 &      106.0 &        6.3 \\
       546 &      189.154251 &       62.208569 &         40 &      12.50 &       0.63 &      11.30 &       0.57 &      12.70 &       0.75 &      33.60 &       1.74 &      163.0 &        8.1 &      212.0 &        3.9 \\
       547 &      189.151611 &       62.210369 &         41 &      31.10 &       1.56 &      22.40 &       1.12 &      16.20 &       0.90 &      10.50 &       0.70 &       45.8 &        7.0 &       74.3 &        4.3 \\
       548 &      189.165039 &       62.208420 &         66 &       5.83 &       0.29 &       7.26 &       0.37 &      10.00 &       0.64 &      18.40 &       1.03 &       39.3 &        7.2 &       48.5 &        4.4 \\
       549 &      189.131836 &       62.212040 &         39 &      18.60 &       0.93 &      13.80 &       0.69 &      10.80 &       0.68 &      11.10 &       0.73 &       82.0 &        8.3 &      113.0 &        5.8 \\
       550 &      189.132828 &       62.211231 &         38 &      13.60 &       0.68 &      11.00 &       0.55 &      10.20 &       0.65 &      11.90 &       0.76 &       37.6 &        6.5 &        9.3 &        5.4 \\
       551 &      189.129883 &       62.210087 &         40 &      12.10 &       0.61 &      11.10 &       0.56 &       9.34 &       0.62 &      17.20 &       0.98 &       44.4 &        9.4 &       83.3 &        5.1 \\
       552 &      189.289642 &       62.209206 &         32 &    3290.00 &     164.50 &    1990.00 &      99.50 &    1350.00 &      67.50 &     754.00 &      37.70 &      183.8 &       12.4 &       78.2 &        5.7 \\
       553 &      188.973007 &       62.208912 &         16 &      27.80 &       1.39 &      18.50 &       0.93 &      17.40 &       0.98 &      11.50 &       0.78 &      111.5 &       10.7 &      130.0 &        6.4 \\
       554 &      189.009094 &       62.210602 &         21 &      37.10 &       1.86 &      23.20 &       1.16 &      22.30 &       1.20 &      14.80 &       0.91 &       62.2 &       10.7 &      150.0 &        6.5 \\
       555 &      188.992966 &       62.207775 &         27 &      26.60 &       1.33 &      17.70 &       0.89 &      15.30 &       0.89 &      11.50 &       0.78 &       85.1 &        7.8 &      109.0 &        5.8 \\
       556 &      189.089798 &       62.207458 &         25 &      48.80 &       2.44 &      43.80 &       2.19 &      32.40 &       1.68 &      72.50 &       3.66 &      185.6 &       10.7 &      226.0 &        7.0 \\
       557 &      189.002563 &       62.208721 &         28 &      11.50 &       0.58 &       9.72 &       0.49 &       7.59 &       0.59 &      13.00 &       0.84 &       46.5 &        9.1 &       37.5 &        7.3 \\
       558 &      189.340729 &       62.207035 &         24 &      17.50 &       0.88 &      14.70 &       0.74 &      11.60 &       0.66 &      20.70 &       1.10 &       84.5 &       10.0 &       64.1 &        6.0 \\
       559 &      189.145706 &       62.206722 &         38 &     188.00 &       9.40 &     130.00 &       6.50 &     121.00 &       6.06 &      89.00 &       4.47 &      316.3 &       10.9 &      345.0 &        6.9 \\
       560 &      189.310013 &       62.205875 &         27 &      15.10 &       0.76 &      11.70 &       0.59 &       8.28 &       0.52 &       7.56 &       0.52 &       67.9 &        8.9 &       65.9 &        6.0 \\
       561 &      189.026825 &       62.207256 &         32 &       9.27 &       0.47 &       7.84 &       0.40 &       5.24 &       0.51 &       5.35 &       0.59 &       35.4 &        6.7 &       30.7 &        5.2 \\
       562 &      189.204453 &       62.205894 &         49 &      11.70 &       0.59 &       8.23 &       0.42 &       7.93 &       0.53 &       5.47 &       0.50 &       52.8 &        8.9 &       67.7 &        6.4 \\
       563 &      189.215530 &       62.205673 &         39 &      21.80 &       1.09 &      21.30 &       1.07 &      17.60 &       0.94 &      46.80 &       2.37 &       96.3 &        7.8 &      132.0 &        6.8 \\
       564 &      189.003067 &       62.204315 &         29 &      26.20 &       1.31 &      22.50 &       1.13 &      17.70 &       0.99 &      34.70 &       1.81 &      125.3 &       10.5 &      176.0 &        7.8 \\
       565 &      189.153381 &       62.203651 &         54 &     118.00 &       5.90 &      78.70 &       3.94 &      68.50 &       3.45 &      47.20 &       2.41 &      300.5 &        8.3 &      386.0 &        4.5 \\
       566 &      189.090332 &       62.205105 &         31 &      14.40 &       0.72 &      10.20 &       0.51 &       7.23 &       0.56 &       7.37 &       0.62 &       71.4 &        6.3 &       86.4 &        6.2 \\
       567 &      189.260986 &       62.204575 &         24 &      40.50 &       2.03 &      34.90 &       1.75 &      23.20 &       1.20 &      20.10 &       1.07 &       93.5 &       11.5 &       68.8 &        6.1 \\
       568 &      189.345779 &       62.205017 &         37 &      15.90 &       0.80 &      11.60 &       0.58 &      11.50 &       0.66 &      11.20 &       0.68 &       57.3 &        9.8 &       47.7 &        7.1 \\
       569 &      189.209076 &       62.204716 &         48 &      35.70 &       1.79 &      25.60 &       1.28 &      18.80 &       1.00 &      15.50 &       0.88 &       43.6 &        8.9 &       33.9 &        7.4 \\
       570 &      189.178848 &       62.204533 &         51 &      29.30 &       1.47 &      25.50 &       1.28 &      19.00 &       1.03 &      38.30 &       1.97 &      108.9 &       10.0 &      118.0 &        5.2 \\
       571 &      189.343430 &       62.204594 &         34 &      66.60 &       3.33 &      50.10 &       2.51 &      46.50 &       2.35 &      43.60 &       2.21 &      528.4 &       10.7 &      572.0 &        6.9 \\
       572 &      189.284409 &       62.204098 &         31 &      18.90 &       0.95 &      17.30 &       0.87 &      18.70 &       0.99 &      11.50 &       0.68 &       41.5 &        7.8 &       20.9 &        6.3 \\
       573 &      188.983704 &       62.205441 &         21 &      74.40 &       3.72 &      56.10 &       2.81 &      51.80 &       2.63 &      82.20 &       4.14 &      282.8 &       15.9 &      430.0 &        6.0 \\
       574 &      189.202667 &       62.204399 &         50 &      28.10 &       1.41 &      31.70 &       1.59 &      31.30 &       1.61 &      23.50 &       1.25 &       57.9 &        8.7 &      291.0 &        7.4 \\
       575 &      189.316498 &       62.203682 &         24 &      57.30 &       2.87 &      44.90 &       2.25 &      33.70 &       1.71 &      35.70 &       1.82 &      173.9 &       10.4 &      187.0 &        8.2 \\
       576 &      189.072189 &       62.203548 &         24 &      70.40 &       3.52 &      52.10 &       2.61 &      37.90 &       1.95 &      28.70 &       1.52 &       69.1 &        9.8 &      114.0 &        4.3 \\
       577 &      189.143631 &       62.203609 &         44 &     271.00 &      13.55 &     213.00 &      10.65 &     189.00 &       9.46 &     328.00 &      16.41 &      839.6 &       19.6 &     1310.0 &        9.4 \\
       578 &      189.293381 &       62.204838 &         26 &      27.10 &       1.36 &      17.70 &       0.89 &      16.40 &       0.88 &      10.40 &       0.63 &       63.0 &        9.6 &       54.6 &        5.5 \\
       579 &      189.005493 &       62.203312 &         27 &      24.50 &       1.23 &      17.50 &       0.88 &      17.30 &       0.97 &      16.50 &       0.98 &       52.5 &        8.9 &       45.3 &        6.3 \\
       580 &      189.038879 &       62.205063 &         32 &      22.40 &       1.12 &      14.90 &       0.75 &      15.40 &       0.89 &      10.80 &       0.75 &       70.0 &        8.9 &       80.1 &        6.3 \\
       581 &      189.407608 &       62.203259 &         11 &      17.80 &       0.89 &      14.20 &       0.72 &      10.30 &       0.70 &      11.00 &       0.87 &       91.6 &       14.6 &       62.7 &        5.0 \\
       582 &      189.360062 &       62.203773 &         19 &      26.20 &       1.31 &      22.90 &       1.15 &      17.20 &       0.92 &      35.20 &       1.81 &       71.2 &        8.1 &       84.5 &        6.7 \\
       583 &      189.342178 &       62.202904 &         36 &      39.10 &       1.96 &      27.70 &       1.39 &      24.70 &       1.28 &      19.40 &       1.04 &      134.6 &        9.2 &      163.0 &        6.4 \\
       584 &      189.126678 &       62.202381 &         26 &      24.40 &       1.22 &      21.50 &       1.08 &      16.20 &       0.90 &      32.30 &       1.68 &       98.6 &        8.3 &       94.2 &        5.1 \\
       585 &      189.245850 &       62.202469 &         24 &      65.40 &       3.27 &      43.90 &       2.20 &      39.00 &       1.98 &      28.70 &       1.48 &      220.9 &        9.2 &      273.0 &        6.5 \\
       586 &      189.039902 &       62.199615 &         24 &      57.50 &       2.88 &      35.60 &       1.78 &      31.70 &       1.65 &      21.20 &       1.18 &       96.2 &        9.6 &      111.0 &        5.1 \\
       587 &      189.037689 &       62.201561 &         29 &      65.30 &       3.27 &      44.90 &       2.25 &      38.30 &       1.97 &      26.40 &       1.42 &      103.4 &        8.5 &      109.0 &        4.3 \\
       588 &      189.404404 &       62.201366 &         21 &     151.00 &       7.55 &     132.00 &       6.60 &     103.00 &       5.17 &     213.00 &      10.67 &      590.3 &       20.4 &      763.0 &        8.0 \\
       589 &      189.174820 &       62.201496 &         48 &      26.30 &       1.32 &      22.70 &       1.14 &      17.50 &       0.96 &      33.10 &       1.72 &       93.1 &        9.6 &       93.9 &        6.1 \\
       590 &      189.042252 &       62.201221 &         32 &      14.00 &       0.70 &      12.80 &       0.64 &       9.42 &       0.64 &       9.80 &       0.72 &       66.5 &        7.8 &       49.3 &        4.1 \\
       591 &      189.087723 &       62.202328 &         45 &      48.60 &       2.43 &      32.10 &       1.61 &      33.20 &       1.71 &      26.90 &       1.44 &      224.4 &       10.4 &      247.0 &        7.0 \\
       592 &      189.087524 &       62.201088 &         37 &      39.10 &       1.96 &      31.20 &       1.56 &      24.60 &       1.30 &      40.50 &       2.09 &       78.8 &       11.8 &       75.4 &        6.9 \\
       593 &      189.154343 &       62.199909 &         55 &      25.20 &       1.26 &      17.10 &       0.86 &      17.70 &       0.97 &      12.50 &       0.79 &       69.1 &        7.4 &       84.5 &        4.2 \\
       594 &      189.316513 &       62.199699 &         27 &     274.00 &      13.70 &     175.00 &       8.75 &     123.00 &       6.16 &      95.20 &       4.77 &      158.0 &        9.1 &      227.0 &        6.2 \\
       595 &      189.022461 &       62.200592 &         23 &      42.60 &       2.13 &      32.50 &       1.63 &      23.80 &       1.27 &      29.80 &       1.58 &       96.2 &       11.7 &       67.0 &        4.6 \\
       596 &      189.032623 &       62.200165 &         17 &      33.10 &       1.66 &      24.20 &       1.21 &      19.60 &       1.08 &      23.40 &       1.28 &       62.0 &       12.9 &       54.1 &        4.7 \\
       597 &      189.077881 &       62.198387 &         37 &      35.60 &       1.78 &      23.90 &       1.20 &      25.70 &       1.36 &      18.80 &       1.07 &      182.1 &        8.7 &      171.0 &        5.2 \\
       598 &      189.081177 &       62.199741 &         39 &      12.70 &       0.64 &       8.66 &       0.44 &       8.20 &       0.59 &       5.94 &       0.59 &       65.2 &        6.8 &       88.4 &        7.0 \\
       599 &      189.011993 &       62.200348 &         41 &      17.10 &       0.86 &      11.80 &       0.59 &      10.50 &       0.69 &       6.56 &       0.62 &       64.0 &        8.5 &       90.4 &        6.1 \\
       600 &      189.115601 &       62.199608 &         25 &       6.24 &       0.31 &       7.36 &       0.37 &      10.30 &       0.65 &      19.00 &       1.06 &       61.5 &        7.6 &      105.0 &        7.3 \\
       601 &      189.248398 &       62.198166 &         25 &      19.80 &       0.99 &      14.30 &       0.72 &      10.50 &       0.61 &      11.10 &       0.67 &      104.3 &       10.5 &      118.0 &        6.7 \\
       602 &      189.274521 &       62.198246 &         17 &      86.00 &       4.30 &      58.90 &       2.95 &      54.80 &       2.76 &      44.50 &       2.25 &      512.5 &       23.1 &      665.0 &        9.6 \\
       603 &      189.359818 &       62.198017 &         24 &      17.30 &       0.87 &      11.90 &       0.60 &      10.30 &       0.61 &       8.92 &       0.60 &       95.3 &        9.1 &      132.0 &        6.5 \\
       604 &      189.380676 &       62.197964 &         25 &      20.20 &       1.01 &      13.30 &       0.67 &      11.80 &       0.70 &      15.70 &       0.93 &       59.4 &       11.5 &      332.0 &        6.7 \\
       605 &      189.254623 &       62.197685 &         40 &      12.10 &       0.61 &      13.40 &       0.67 &      11.80 &       0.67 &      10.60 &       0.65 &       36.4 &        6.7 &       67.4 &        7.1 \\
       606 &      189.159653 &       62.197468 &         40 &      40.90 &       2.05 &      27.20 &       1.36 &      29.80 &       1.54 &      20.50 &       1.13 &      201.5 &       16.5 &      220.0 &        3.7 \\
       607 &      189.157486 &       62.197029 &         42 &      42.30 &       2.12 &      31.30 &       1.57 &      30.10 &       1.56 &      22.80 &       1.24 &      157.8 &       18.9 &      175.0 &        3.2 \\
       608 &      189.024292 &       62.196678 &         25 &      43.70 &       2.19 &      46.60 &       2.33 &      38.90 &       2.00 &      31.90 &       1.68 &      105.8 &        9.2 &      171.0 &        5.0 \\
       609 &      189.392349 &       62.194344 &         13 &      72.50 &       3.63 &      56.70 &       2.84 &      45.90 &       2.34 &     217.00 &      10.87 &      348.2 &       22.2 &      580.0 &       11.0 \\
       610 &      189.256607 &       62.196198 &         24 &      54.70 &       2.74 &      69.00 &       3.45 &      69.00 &       3.47 &      54.40 &       2.75 &      201.5 &       11.3 &      739.0 &       10.7 \\
       611 &      189.205246 &       62.196827 &         47 &      23.10 &       1.16 &      17.40 &       0.87 &      13.00 &       0.75 &      10.60 &       0.70 &       60.3 &        8.5 &       89.4 &        5.8 \\
       612 &      189.036713 &       62.195461 &         20 &      66.60 &       3.33 &      68.50 &       3.43 &      52.20 &       2.65 &      53.20 &       2.71 &      408.3 &       15.9 &      273.0 &        6.0 \\
       613 &      189.180008 &       62.196663 &         40 &      48.30 &       2.42 &      35.50 &       1.78 &      24.70 &       1.30 &      22.30 &       1.22 &       85.1 &       13.1 &      119.0 &        5.4 \\
       614 &      188.998169 &       62.197014 &         24 &      27.70 &       1.39 &      29.70 &       1.49 &      23.10 &       1.24 &      20.90 &       1.17 &      152.0 &        9.2 &      103.0 &        5.7 \\
       615 &      189.172531 &       62.195091 &         47 &      57.70 &       2.89 &      59.90 &       3.00 &      48.70 &       2.47 &      40.40 &       2.08 &      139.1 &       10.9 &      226.0 &        5.0 \\
       616 &      189.169434 &       62.193237 &         45 &      22.60 &       1.13 &      17.80 &       0.89 &      12.60 &       0.75 &      11.70 &       0.76 &      123.6 &       10.5 &      105.0 &        4.2 \\
       617 &      189.293961 &       62.194801 &         31 &      41.60 &       2.08 &      26.60 &       1.33 &      25.80 &       1.33 &      19.00 &       1.02 &      167.7 &        9.2 &      178.0 &        5.8 \\
       618 &      189.069962 &       62.194618 &         40 &      22.80 &       1.14 &      16.80 &       0.84 &      12.20 &       0.75 &      12.40 &       0.80 &      111.0 &        7.8 &      115.0 &        4.7 \\
       619 &      189.192490 &       62.195011 &         39 &      97.70 &       4.89 &      72.60 &       3.63 &      52.20 &       2.64 &      44.60 &       2.28 &      245.7 &       11.7 &      293.0 &        5.5 \\
       620 &      189.020523 &       62.194866 &         26 &      42.90 &       2.15 &      30.20 &       1.51 &      24.00 &       1.28 &      17.00 &       1.00 &      106.0 &        8.5 &       60.6 &        6.6 \\
       621 &      189.016388 &       62.194687 &         29 &    2660.00 &     133.00 &    1630.00 &      81.50 &    1110.00 &      55.50 &     586.00 &      29.30 &      138.7 &       10.5 &       76.1 &        7.1 \\
       622 &      189.052078 &       62.194588 &         31 &     135.00 &       6.75 &     123.00 &       6.15 &      95.50 &       4.80 &     375.00 &      18.76 &      761.7 &       40.9 &     1310.0 &       19.2 \\
       623 &      189.050110 &       62.194122 &         28 &     161.00 &       8.05 &     159.00 &       7.95 &     111.00 &       5.57 &     270.00 &      13.51 &      291.6 &       38.3 &      203.0 &       16.3 \\
       624 &      189.222397 &       62.194351 &         22 &      33.60 &       1.68 &      36.40 &       1.82 &      28.90 &       1.49 &      41.80 &       2.13 &      436.6 &       10.0 &      336.0 &        7.5 \\
       625 &      189.330658 &       62.194241 &         28 &      11.80 &       0.59 &      11.80 &       0.59 &       8.43 &       0.53 &       9.44 &       0.60 &       66.7 &       10.5 &       67.9 &        5.3 \\
       626 &      189.004944 &       62.191292 &         21 &      19.80 &       0.99 &      13.50 &       0.68 &      13.90 &       0.82 &       8.82 &       0.69 &       81.2 &        9.4 &       79.0 &        6.6 \\
       627 &      189.063858 &       62.192944 &         36 &      38.20 &       1.91 &      29.00 &       1.45 &      22.20 &       1.19 &      19.40 &       1.10 &       98.2 &        8.1 &      151.0 &        4.4 \\
       628 &      189.327225 &       62.193939 &         23 &      17.10 &       0.86 &      15.10 &       0.76 &      11.00 &       0.63 &      12.50 &       0.72 &      117.2 &        9.6 &       74.9 &        5.2 \\
       629 &      189.313507 &       62.193336 &         38 &      18.00 &       0.90 &      16.20 &       0.81 &      11.50 &       0.65 &      13.60 &       0.77 &      129.9 &        8.0 &       98.0 &        5.3 \\
       630 &      189.209503 &       62.193108 &         36 &      17.10 &       0.86 &      13.60 &       0.68 &       8.93 &       0.58 &       7.85 &       0.61 &       41.9 &        7.8 &       39.0 &        5.2 \\
       631 &      189.139450 &       62.192810 &         32 &      17.30 &       0.87 &      12.70 &       0.64 &      11.60 &       0.71 &      10.40 &       0.72 &       87.0 &       10.2 &       81.9 &        5.3 \\
       632 &      189.289810 &       62.192589 &         23 &      12.00 &       0.60 &       8.83 &       0.44 &       8.27 &       0.52 &       6.77 &       0.49 &       57.8 &       10.0 &       71.6 &        5.1 \\
       633 &      189.172409 &       62.191540 &         44 &      71.30 &       3.57 &      54.50 &       2.73 &      39.50 &       2.02 &      42.70 &       2.19 &      236.9 &       11.5 &      320.0 &        8.3 \\
       634 &      189.329819 &       62.192009 &         21 &      70.40 &       3.52 &      49.00 &       2.45 &      45.50 &       2.30 &      44.10 &       2.24 &      205.0 &        9.6 &      196.0 &        6.5 \\
       635 &      189.338989 &       62.191933 &         27 &      37.20 &       1.86 &      41.00 &       2.05 &      36.70 &       1.86 &      31.70 &       1.63 &      104.1 &        9.4 &      210.0 &        6.3 \\
       636 &      189.326111 &       62.192551 &         19 &      19.50 &       0.98 &      23.10 &       1.16 &      21.50 &       1.12 &      17.30 &       0.94 &       69.3 &       11.8 &      107.0 &        5.7 \\
       637 &      189.153687 &       62.193024 &         38 &     162.00 &       0.09 &     111.00 &       0.13 &     113.00 &       0.66 &     519.00 &       0.70 &      385.3 &       20.5 &      755.0 &        9.6 \\
       638 &      189.256516 &       62.191341 &         23 &      50.40 &       2.52 &      32.70 &       1.64 &      34.50 &       1.76 &      28.30 &       1.47 &      275.7 &       15.0 &      278.0 &        7.2 \\
       639 &      189.070404 &       62.190769 &         24 &      32.00 &       1.60 &      25.70 &       1.29 &      18.90 &       1.04 &      18.50 &       1.06 &      185.6 &        8.9 &      136.0 &        6.2 \\
       640 &      189.227692 &       62.190865 &         28 &      46.80 &       2.34 &      42.50 &       2.13 &      28.90 &       1.49 &     119.00 &       5.97 &      198.0 &       10.4 &      186.0 &        6.5 \\
       641 &      189.078094 &       62.188732 &         19 &      38.00 &       1.90 &      33.60 &       1.68 &      30.40 &       1.58 &      29.00 &       1.54 &      103.4 &       12.8 &      270.0 &        7.3 \\
       642 &      189.116089 &       62.190174 &         39 &      22.00 &       1.10 &      15.90 &       0.80 &      12.60 &       0.75 &      12.50 &       0.80 &       62.4 &       10.2 &       44.9 &        5.8 \\
       643 &      189.258530 &       62.189693 &         23 &      70.50 &       3.53 &      48.50 &       2.43 &      39.80 &       2.02 &     193.00 &       9.66 &      146.3 &       11.3 &      193.0 &        6.2 \\
       644 &      189.283234 &       62.189323 &         21 &      15.90 &       0.80 &      19.40 &       0.97 &      20.10 &       1.05 &      14.80 &       0.82 &       46.0 &        9.1 &      175.0 &        5.5 \\
       645 &      189.198776 &       62.188953 &         18 &      17.90 &       0.90 &      15.80 &       0.79 &      11.40 &       0.70 &      11.40 &       0.75 &      118.1 &       10.5 &       71.5 &        4.9 \\
       646 &      189.044373 &       62.187004 &         26 &      16.50 &       0.83 &      11.30 &       0.57 &      12.50 &       0.76 &       7.78 &       0.64 &      100.6 &       10.9 &      111.0 &        5.3 \\
       647 &      189.221741 &       62.187992 &         28 &      62.70 &       3.14 &      45.20 &       2.26 &      39.90 &       2.03 &      34.90 &       1.80 &      281.1 &       12.8 &      363.0 &        7.1 \\
       648 &      188.995865 &       62.187359 &         25 &       8.25 &       0.41 &       6.39 &       0.33 &       6.22 &       0.54 &       5.69 &       0.60 &       56.0 &        9.1 &       57.5 &        6.2 \\
       649 &      189.077530 &       62.187523 &         24 &     107.00 &       5.35 &      83.00 &       4.15 &      72.70 &       3.66 &      75.70 &       3.82 &      318.1 &       16.1 &      404.0 &        5.4 \\
       650 &      189.087433 &       62.187248 &         25 &      42.50 &       2.13 &      32.40 &       1.62 &      26.80 &       1.40 &      28.30 &       1.50 &      203.2 &       14.6 &      229.0 &        7.4 \\
       651 &      189.131088 &       62.187172 &         26 &      43.70 &       2.19 &      33.20 &       1.66 &      27.20 &       1.42 &      37.20 &       1.93 &      390.6 &       19.1 &      480.0 &        5.9 \\
       652 &      189.261871 &       62.186192 &         19 &      38.50 &       1.93 &      26.80 &       1.34 &      24.50 &       1.27 &      23.00 &       1.21 &      117.2 &        8.5 &      112.0 &        6.4 \\
       653 &      189.160751 &       62.186543 &         35 &      24.20 &       1.21 &      17.70 &       0.89 &      14.30 &       0.82 &      11.80 &       0.77 &       79.0 &        8.5 &      118.0 &        6.1 \\
       654 &      189.162170 &       62.188450 &         41 &       6.85 &       0.35 &       4.92 &       0.25 &       4.19 &       0.46 &       2.80 &       0.51 &       35.6 &        6.5 &        2.1 &        4.4 \\
       655 &      189.102371 &       62.186497 &         59 &      46.10 &       2.31 &      28.90 &       1.45 &      27.90 &       1.46 &      21.80 &       1.20 &       45.8 &        9.2 &       65.2 &        6.1 \\
       656 &      189.158432 &       62.188091 &         40 &      50.70 &       2.54 &      39.70 &       1.99 &      29.10 &       1.51 &      30.10 &       1.58 &      281.1 &       11.5 &      328.0 &        7.1 \\
       657 &      189.013565 &       62.186367 &         17 &     133.00 &       6.65 &      90.60 &       4.53 &     109.00 &       5.47 &      99.70 &       5.01 &      719.3 &       37.4 &     1250.0 &       10.1 \\
       658 &      189.152771 &       62.186520 &         30 &       4.87 &       0.25 &       3.47 &       0.19 &       2.69 &       0.43 &       3.09 &       0.53 &       52.6 &       12.8 &       53.9 &        5.8 \\
       659 &      189.066925 &       62.185490 &         22 &      18.10 &       0.91 &      25.20 &       1.26 &      32.70 &       1.69 &      53.80 &       2.74 &       96.2 &        9.8 &      174.0 &        5.8 \\
       660 &      189.100021 &       62.186050 &         47 &      19.20 &       0.96 &      13.70 &       0.69 &      14.50 &       0.84 &      11.90 &       0.78 &       80.6 &        8.1 &       69.8 &        6.0 \\
       661 &      189.088745 &       62.186047 &         30 &     130.00 &       6.50 &      96.50 &       4.83 &      71.60 &       3.61 &      60.40 &       3.06 &      208.5 &       11.7 &      261.0 &        8.6 \\
       662 &      189.092606 &       62.185135 &         38 &      16.70 &       0.84 &      13.50 &       0.68 &       7.89 &       0.58 &      16.40 &       0.97 &       44.2 &        8.1 &       21.2 &        6.0 \\
       663 &      188.993927 &       62.184052 &         12 &      73.80 &       3.69 &      46.70 &       2.34 &      43.50 &       2.22 &      28.60 &       1.53 &      115.6 &       12.8 &      123.0 &        5.4 \\
       664 &      189.128296 &       62.183033 &         21 &      25.10 &       1.26 &      22.80 &       1.14 &      13.40 &       0.79 &      52.00 &       2.65 &       87.5 &       13.7 &      106.0 &        6.2 \\
       665 &      189.211395 &       62.182976 &         28 &      16.00 &       0.80 &      12.80 &       0.64 &       9.36 &       0.62 &      14.00 &       0.85 &       53.9 &        9.4 &       49.6 &        4.5 \\
       666 &      188.980942 &       62.182434 &         11 &      30.50 &       1.53 &      22.20 &       1.11 &      21.80 &       1.18 &      18.30 &       1.07 &       77.3 &       14.8 &       80.4 &        5.0 \\
       667 &      189.068802 &       62.182301 &         23 &      33.00 &       1.65 &      27.00 &       1.35 &      17.90 &       0.99 &      17.80 &       1.02 &      159.6 &        9.8 &      141.0 &        5.9 \\
       668 &      189.254486 &       62.181767 &         37 &      15.50 &       0.78 &      17.60 &       0.88 &      14.80 &       0.82 &      14.10 &       0.82 &       75.1 &        7.0 &      108.0 &        7.4 \\
       669 &      189.322937 &       62.182487 &         24 &       7.34 &       0.37 &       6.39 &       0.32 &       3.52 &       0.37 &      14.40 &       0.81 &       54.8 &       13.3 &       30.3 &        4.7 \\
       670 &      189.284729 &       62.182232 &         38 &      63.50 &       3.18 &      65.20 &       3.26 &      51.40 &       2.59 &     169.00 &       8.46 &      454.2 &       12.2 &      673.0 &       10.3 \\
       671 &      189.141693 &       62.181843 &         26 &      19.20 &       0.96 &      12.40 &       0.62 &      12.50 &       0.75 &       8.89 &       0.68 &       82.5 &       12.2 &       68.3 &        5.3 \\
       672 &      189.137863 &       62.181927 &         20 &      14.30 &       0.72 &      10.90 &       0.55 &       8.00 &       0.58 &       7.80 &       0.65 &       66.9 &       11.5 &       66.5 &        5.3 \\
       673 &      189.172745 &       62.180912 &         31 &      16.30 &       0.82 &      11.50 &       0.58 &      10.00 &       0.64 &       7.65 &       0.63 &       59.9 &       12.0 &       83.3 &        6.2 \\
       674 &      189.305527 &       62.181725 &         18 &      16.30 &       0.82 &      12.50 &       0.63 &      12.80 &       0.71 &      14.10 &       0.80 &       77.4 &       14.2 &      119.0 &        6.8 \\
       675 &      189.229019 &       62.182323 &         27 &      11.20 &       0.56 &      12.90 &       0.65 &      16.50 &       0.91 &      14.30 &       0.86 &       39.9 &        7.8 &      224.0 &        6.7 \\
       676 &      189.004562 &       62.182861 &         22 &      52.00 &       2.60 &      37.50 &       1.88 &      40.30 &       2.06 &      35.70 &       1.86 &      166.3 &       10.4 &      178.0 &        5.6 \\
       677 &      189.213730 &       62.181007 &         27 &      30.60 &       1.53 &      28.50 &       1.43 &      21.70 &       1.16 &      24.40 &       1.31 &       92.8 &        8.9 &       71.9 &        5.8 \\
       678 &      189.286118 &       62.180851 &         27 &      41.10 &       2.06 &      39.80 &       1.99 &      33.60 &       1.71 &      82.30 &       4.13 &      189.1 &       11.7 &      250.0 &        7.4 \\
       679 &      189.073639 &       62.180481 &         33 &      12.60 &       0.63 &       9.92 &       0.50 &       6.67 &       0.54 &       7.22 &       0.63 &       68.2 &        5.9 &       51.1 &        5.9 \\
       680 &      189.169800 &       62.180279 &         31 &      15.70 &       0.79 &      12.30 &       0.62 &      10.70 &       0.68 &      11.40 &       0.76 &      114.0 &       11.1 &      128.0 &        5.8 \\
       681 &      189.194214 &       62.180267 &         24 &      34.70 &       1.74 &      26.10 &       1.31 &      25.00 &       1.32 &      21.30 &       1.17 &      300.5 &       14.2 &      349.0 &        6.5 \\
       682 &      189.349152 &       62.179462 &         12 &      76.70 &       3.84 &      51.80 &       2.59 &      47.50 &       2.41 &     215.00 &      10.76 &      157.5 &       10.9 &      205.0 &        6.8 \\
       683 &      189.121307 &       62.179440 &         31 &      97.00 &       4.85 &      86.80 &       4.34 &      76.00 &       3.82 &      72.10 &       3.64 &      463.0 &       18.3 &      730.0 &       12.7 \\
       684 &      189.199509 &       62.179314 &         22 &      45.40 &       2.27 &      37.50 &       1.88 &      26.50 &       1.39 &      24.30 &       1.31 &      130.3 &       13.5 &       99.4 &        5.0 \\
       685 &      189.197678 &       62.179462 &         24 &      21.70 &       1.09 &      21.60 &       1.08 &      15.70 &       0.89 &      16.10 &       0.94 &       62.6 &       13.5 &       56.6 &        5.4 \\
       686 &      189.340561 &       62.178959 &         19 &      29.60 &       1.48 &      21.10 &       1.06 &      18.50 &       1.00 &      16.90 &       0.95 &      198.0 &        9.8 &      230.0 &        6.0 \\
       687 &      189.341080 &       62.176590 &         12 &      71.60 &       3.58 &      52.50 &       2.63 &      43.30 &       2.20 &      42.20 &       2.16 &      156.5 &       11.3 &      255.0 &        5.5 \\
       688 &      189.000687 &       62.179832 &         15 &      12.90 &       0.65 &      14.80 &       0.74 &      26.70 &       1.41 &      59.10 &       3.00 &      461.3 &       23.7 &     1240.0 &       10.2 \\
       689 &      189.019852 &       62.178654 &         38 &      16.90 &       0.85 &      11.90 &       0.60 &       9.85 &       0.66 &       8.82 &       0.68 &       98.1 &        8.1 &      116.0 &        4.5 \\
       690 &      189.113602 &       62.178661 &         33 &      15.10 &       0.76 &      18.00 &       0.90 &      14.90 &       0.85 &      13.90 &       0.87 &       61.4 &       10.4 &      103.0 &       10.9 \\
       691 &      189.134766 &       62.177956 &         19 &      36.80 &       1.84 &      26.20 &       1.31 &      18.00 &       0.99 &      17.70 &       1.03 &      128.5 &       13.1 &      122.0 &        6.1 \\
       692 &      189.033890 &       62.176643 &         22 &      78.00 &       3.90 &      73.60 &       3.68 &     129.00 &       6.47 &     264.00 &      13.21 &      774.1 &       21.5 &     2300.0 &       13.5 \\
       693 &      189.027771 &       62.176201 &         27 &      24.40 &       1.22 &      15.80 &       0.79 &      15.50 &       0.89 &      11.90 &       0.79 &       75.5 &       11.8 &       77.0 &        9.9 \\
       694 &      189.213028 &       62.175240 &         22 &      95.10 &       4.76 &      97.00 &       4.85 &      80.00 &       4.02 &     267.00 &      13.36 &      676.9 &       18.9 &     1000.0 &       11.4 \\
       695 &      189.254227 &       62.174644 &         35 &      12.30 &       0.62 &      10.80 &       0.54 &      10.40 &       0.63 &       9.62 &       0.66 &       55.7 &        8.3 &       50.3 &        7.1 \\
       696 &      189.056808 &       62.174179 &         53 &      28.20 &       1.41 &      25.00 &       1.25 &      21.70 &       1.17 &      43.00 &       2.21 &      113.6 &        8.1 &      143.0 &        5.0 \\
       697 &      189.166580 &       62.174763 &         23 &      48.40 &       2.42 &      35.00 &       1.75 &      27.90 &       1.46 &      21.30 &       1.18 &      116.4 &       10.7 &      143.0 &        6.1 \\
       698 &      189.283218 &       62.174648 &         17 &      22.80 &       1.14 &      23.40 &       1.17 &      18.00 &       0.96 &      22.90 &       1.21 &      272.1 &       14.4 &      157.0 &        8.3 \\
       699 &      189.304138 &       62.174561 &         27 &      18.20 &       0.91 &      12.90 &       0.65 &      14.40 &       0.79 &      10.80 &       0.67 &      143.7 &       11.3 &      182.0 &        6.1 \\
       700 &      189.022552 &       62.175388 &         34 &      36.00 &       1.80 &      24.30 &       1.22 &      26.70 &       1.41 &      20.70 &       1.16 &      146.0 &        9.1 &      166.0 &        6.6 \\
       701 &      189.258133 &       62.173481 &         35 &      47.10 &       2.36 &      41.00 &       2.05 &      30.50 &       1.57 &      67.70 &       3.41 &      194.4 &       12.4 &      224.0 &        7.3 \\
       702 &      189.280701 &       62.174156 &         21 &      13.20 &       0.66 &      13.00 &       0.65 &       9.88 &       0.59 &      13.30 &       0.78 &      128.9 &       10.5 &       65.4 &        7.0 \\
       703 &      189.033325 &       62.173828 &         21 &      43.70 &       2.19 &      27.70 &       1.39 &      29.70 &       1.55 &      20.40 &       1.14 &      173.9 &       13.5 &      167.0 &        5.8 \\
       704 &      189.238937 &       62.173920 &         36 &      16.20 &       0.81 &      10.50 &       0.53 &       8.47 &       0.57 &       5.57 &       0.56 &       33.6 &        6.3 &        6.5 &        6.1 \\
       705 &      188.990097 &       62.173435 &         11 &      11.10 &       0.56 &      15.10 &       0.76 &      21.10 &       1.15 &      36.20 &       1.89 &       73.2 &       11.8 &      110.0 &        5.4 \\
       706 &      189.087189 &       62.172150 &         23 &      31.00 &       1.55 &      22.20 &       1.11 &      19.00 &       1.04 &      13.70 &       0.87 &      131.7 &       11.3 &      162.0 &        6.4 \\
       707 &      189.003464 &       62.175117 &         17 &      28.40 &       1.42 &      18.70 &       0.94 &      19.00 &       1.05 &      13.40 &       0.85 &       82.5 &       11.1 &       87.3 &        6.9 \\
       708 &      189.119812 &       62.173206 &         34 &      24.80 &       1.24 &      17.00 &       0.85 &      14.70 &       0.85 &       9.89 &       0.73 &      103.7 &       11.1 &      111.0 &        5.6 \\
       709 &      189.030807 &       62.172977 &         26 &      20.60 &       1.03 &      14.30 &       0.72 &      18.20 &       1.01 &      13.70 &       0.86 &       79.6 &        8.3 &       81.4 &        6.7 \\
       710 &      189.094482 &       62.174641 &         34 &       7.69 &       0.39 &       9.68 &       0.49 &      13.20 &       0.78 &      25.10 &       1.36 &       60.3 &        9.4 &      105.0 &        5.6 \\
       711 &      189.239410 &       62.172394 &         39 &      27.30 &       1.37 &      21.10 &       1.06 &      17.50 &       0.96 &      13.70 &       0.84 &       59.1 &        6.7 &       68.8 &        6.0 \\
       712 &      189.122498 &       62.171783 &         31 &      20.70 &       1.04 &      16.30 &       0.82 &      13.00 &       0.78 &      14.60 &       0.91 &      155.9 &       10.5 &      173.0 &        5.8 \\
       713 &      189.155609 &       62.170879 &         19 &      15.30 &       0.77 &      16.60 &       0.83 &      11.60 &       0.72 &      11.90 &       0.80 &       88.0 &       12.8 &       43.5 &        5.4 \\
       714 &      189.049042 &       62.170723 &         30 &      21.40 &       1.07 &      26.50 &       1.33 &      25.30 &       1.33 &      19.60 &       1.11 &       61.7 &        6.8 &      155.0 &        3.6 \\
       715 &      189.071182 &       62.169849 &         37 &      54.40 &       2.72 &      37.50 &       1.88 &      31.80 &       1.64 &      25.60 &       1.39 &       44.6 &        8.7 &       80.3 &        5.8 \\
       716 &      189.165512 &       62.169403 &         25 &      27.70 &       1.39 &      22.10 &       1.11 &      18.60 &       1.02 &      27.50 &       1.47 &       94.9 &        9.6 &      103.0 &        5.3 \\
       717 &      189.063309 &       62.169090 &         55 &      68.00 &       3.40 &      52.20 &       2.61 &      38.20 &       1.95 &      46.10 &       2.36 &      311.0 &       12.2 &      325.0 &        6.6 \\
       718 &      189.066483 &       62.168941 &         51 &      39.40 &       1.97 &      41.20 &       2.06 &      30.90 &       1.60 &     120.00 &       6.02 &      272.1 &       12.6 &      316.0 &        5.7 \\
       719 &      189.023911 &       62.167461 &         14 &      56.50 &       2.83 &      47.70 &       2.39 &      47.90 &       2.43 &      50.60 &       2.58 &      296.9 &       14.8 &      528.0 &        6.8 \\
       720 &      189.095062 &       62.168705 &         31 &      42.50 &       2.13 &      26.60 &       1.33 &      24.30 &       1.29 &      17.20 &       1.01 &      111.5 &       13.1 &      129.0 &        7.0 \\
       721 &      189.278656 &       62.168491 &         35 &      10.30 &       0.52 &       7.16 &       0.36 &       6.03 &       0.46 &       4.11 &       0.48 &       44.6 &        8.5 &       35.7 &        7.3 \\
       722 &      189.163025 &       62.168365 &         22 &      41.60 &       2.08 &      35.80 &       1.79 &      39.40 &       2.02 &      29.70 &       1.57 &       59.5 &       10.9 &      225.0 &        6.2 \\
       723 &      189.140320 &       62.168324 &         24 &      74.20 &       3.71 &      56.80 &       2.84 &      44.90 &       2.29 &      49.50 &       2.53 &      528.4 &       14.8 &      581.0 &        9.0 \\
       724 &      189.168884 &       62.167591 &         28 &      24.40 &       1.22 &      16.40 &       0.82 &      17.00 &       0.95 &      13.30 &       0.84 &       93.9 &        9.6 &      107.0 &        5.5 \\
       725 &      189.217911 &       62.166019 &         23 &      16.90 &       0.85 &      11.30 &       0.57 &      12.20 &       0.74 &       9.78 &       0.70 &       97.2 &       11.7 &       91.9 &        8.4 \\
       726 &      189.243134 &       62.166157 &         34 &     300.00 &       0.10 &     209.00 &       0.12 &     155.00 &       0.58 &     614.00 &       0.63 &      470.1 &       16.5 &      540.0 &        9.8 \\
       727 &      189.271149 &       62.166489 &         36 &       8.06 &       0.40 &       7.37 &       0.37 &       4.41 &       0.42 &       2.95 &       0.48 &       43.5 &        8.3 &       20.9 &        8.3 \\
       728 &      189.263611 &       62.164700 &         20 &      15.30 &       0.77 &      11.00 &       0.55 &      10.50 &       0.65 &       7.63 &       0.61 &       74.1 &        9.4 &       98.1 &        7.2 \\
       729 &      189.113434 &       62.167252 &         27 &      14.80 &       0.74 &       9.52 &       0.48 &       9.26 &       0.64 &       6.24 &       0.63 &       76.1 &        8.3 &       63.6 &        5.2 \\
       730 &      189.255081 &       62.166023 &         23 &      19.30 &       0.97 &      12.60 &       0.63 &      12.00 &       0.71 &       8.50 &       0.64 &       65.4 &        7.6 &       81.4 &        7.2 \\
       731 &      189.060165 &       62.164978 &         23 &      51.70 &       2.59 &      36.10 &       1.81 &      30.40 &       1.58 &      23.40 &       1.28 &      187.4 &       13.1 &      258.0 &        5.9 \\
       732 &      189.041260 &       62.164753 &         38 &      14.80 &       0.74 &       9.89 &       0.50 &      10.90 &       0.69 &       7.77 &       0.65 &       58.1 &        5.9 &       53.9 &        5.4 \\
       733 &      189.027374 &       62.164333 &         13 &     127.00 &       6.35 &      88.80 &       4.44 &      98.50 &       4.94 &      90.40 &       4.55 &      339.4 &       15.0 &      499.0 &        8.3 \\
       734 &      189.034607 &       62.164410 &         31 &      16.20 &       0.81 &      10.70 &       0.54 &      10.00 &       0.66 &       5.46 &       0.59 &       66.9 &        8.1 &       65.7 &        4.8 \\
       735 &      189.118896 &       62.164345 &         19 &      12.20 &       0.61 &       8.89 &       0.45 &       6.69 &       0.55 &       7.00 &       0.65 &       54.4 &       10.7 &       41.6 &        5.8 \\
       736 &      189.159943 &       62.164764 &         18 &      36.10 &       1.81 &      25.50 &       1.28 &      18.40 &       1.02 &      18.70 &       1.08 &       56.9 &       11.7 &       38.1 &        6.2 \\
       737 &      189.292999 &       62.163452 &         17 &      11.80 &       0.59 &      11.80 &       0.59 &       7.88 &       0.54 &       8.11 &       0.62 &       52.6 &        8.5 &       35.9 &        7.7 \\
       738 &      189.162750 &       62.162296 &         18 &      29.30 &       1.47 &      27.80 &       1.39 &      21.80 &       1.17 &      21.30 &       1.19 &       72.8 &       10.0 &      124.0 &        5.6 \\
       739 &      189.173203 &       62.163403 &         26 &     135.00 &       6.75 &      98.10 &       4.91 &      89.90 &       4.52 &     110.00 &       5.52 &      254.5 &       16.1 &      422.0 &        8.4 \\
       740 &      189.174164 &       62.161976 &         28 &      58.50 &       2.93 &      38.80 &       1.94 &      31.70 &       1.64 &      25.50 &       1.38 &       91.7 &       12.2 &      123.0 &        6.5 \\
       741 &      189.065094 &       62.162960 &         20 &      68.50 &       3.43 &      59.00 &       2.95 &      42.00 &       2.14 &      34.60 &       1.81 &      123.2 &       14.1 &      107.0 &        5.6 \\
       742 &      189.077591 &       62.159225 &         38 &      19.10 &       0.96 &      12.30 &       0.62 &      12.00 &       0.74 &       8.30 &       0.68 &       60.4 &        8.5 &       60.2 &        5.4 \\
       743 &      189.134171 &       62.160244 &         22 &      20.90 &       1.05 &      19.10 &       0.96 &      13.90 &       0.82 &      14.00 &       0.89 &      112.1 &        9.2 &       69.9 &        4.8 \\
       744 &      189.160904 &       62.160339 &         25 &      39.70 &       1.99 &      27.20 &       1.36 &      25.80 &       1.36 &      19.40 &       1.11 &      180.3 &       10.0 &      210.0 &        5.0 \\
       745 &      189.146667 &       62.160019 &         21 &      12.90 &       0.65 &      10.60 &       0.53 &       7.55 &       0.58 &      10.40 &       0.75 &       82.7 &       10.0 &       71.4 &        5.1 \\
       746 &      189.149139 &       62.160362 &         24 &       5.21 &       0.27 &       5.05 &       0.26 &       5.55 &       0.52 &       9.60 &       0.72 &       55.7 &        9.8 &       35.9 &        5.3 \\
       747 &      189.099396 &       62.159332 &         30 &      13.20 &       0.66 &      17.10 &       0.86 &      15.80 &       0.90 &      14.70 &       0.91 &       61.7 &       10.5 &      161.0 &        7.4 \\
       748 &      189.177399 &       62.159451 &         35 &      66.40 &       3.32 &      54.00 &       2.70 &      50.10 &       2.54 &      81.80 &       4.12 &      323.4 &       10.4 &      481.0 &        7.2 \\
       749 &      189.278656 &       62.158993 &         20 &      20.50 &       1.03 &      24.00 &       1.20 &      18.70 &       1.02 &      20.60 &       1.15 &      125.8 &       10.5 &      180.0 &        7.4 \\
       750 &      189.202652 &       62.158947 &         18 &      30.70 &       1.54 &      25.00 &       1.25 &      21.30 &       1.15 &      31.00 &       1.63 &      114.0 &       10.0 &      127.0 &        7.8 \\
       751 &      189.029770 &       62.160084 &         12 &      26.60 &       1.33 &      17.50 &       0.88 &      17.40 &       0.97 &      12.70 &       0.82 &      108.7 &       15.5 &       74.1 &        6.3 \\
       752 &      189.196716 &       62.158363 &         19 &      19.20 &       0.96 &      15.90 &       0.80 &      10.00 &       0.65 &       9.40 &       0.70 &       77.3 &        9.2 &       51.9 &        7.7 \\
       753 &      189.186142 &       62.157520 &         26 &      19.80 &       0.99 &      15.30 &       0.77 &      12.70 &       0.77 &      17.60 &       1.02 &       64.5 &        9.1 &       58.6 &        6.1 \\
       754 &      189.239105 &       62.156628 &         28 &       8.41 &       0.42 &       6.01 &       0.31 &       4.34 &       0.47 &       3.36 &       0.53 &       42.8 &        8.1 &       40.4 &        7.6 \\
       755 &      189.158325 &       62.156158 &         36 &      53.40 &       2.67 &      33.40 &       1.67 &      33.60 &       1.74 &      27.80 &       1.49 &      192.7 &       10.0 &      214.0 &        6.0 \\
       756 &      189.133392 &       62.154755 &         21 &      23.20 &       1.16 &      16.40 &       0.82 &      13.50 &       0.81 &      10.20 &       0.75 &       76.1 &       10.2 &       71.8 &        6.3 \\
       757 &      189.281281 &       62.155552 &         14 &      21.00 &       1.05 &      15.20 &       0.76 &      14.70 &       0.85 &      12.00 &       0.82 &      123.4 &       12.8 &      133.0 &        8.6 \\
       758 &      189.125229 &       62.156647 &         17 &      27.20 &       1.36 &      39.20 &       1.96 &      59.90 &       3.03 &     120.00 &       6.03 &      199.7 &       12.6 &      223.0 &        7.1 \\
       759 &      189.170349 &       62.154507 &         26 &      10.30 &       0.52 &      10.10 &       0.51 &       8.02 &       0.59 &      10.10 &       0.74 &       91.6 &        8.5 &       80.4 &        6.7 \\
       760 &      189.232437 &       62.154881 &         37 &      74.40 &       3.72 &      72.80 &       3.64 &      67.40 &       3.40 &     152.00 &       7.62 &      399.4 &       10.4 &      854.0 &       11.1 \\
       761 &      189.195862 &       62.151897 &         23 &      12.00 &       0.60 &       8.50 &       0.43 &       7.25 &       0.56 &       6.68 &       0.62 &       75.7 &        9.6 &       96.1 &        6.3 \\
       762 &      189.251083 &       62.152744 &         23 &      17.40 &       0.87 &      25.00 &       1.25 &      31.70 &       1.64 &      24.40 &       1.33 &       88.0 &       10.7 &      267.0 &        7.6 \\
       763 &      189.081650 &       62.149616 &         14 &      14.90 &       0.75 &      11.20 &       0.56 &       7.98 &       0.59 &       7.88 &       0.68 &       76.1 &       12.0 &       80.2 &        6.4 \\
       764 &      189.132339 &       62.151928 &         21 &     283.00 &      14.15 &     182.00 &       9.10 &     144.00 &       7.21 &     134.00 &       6.72 &      171.8 &       20.2 &      247.0 &       12.3 \\
       765 &      189.185684 &       62.148663 &         24 &      28.30 &       1.42 &      22.80 &       1.14 &      18.10 &       1.01 &      16.10 &       0.97 &      108.7 &       10.4 &       99.1 &        5.8 \\
       766 &      189.127060 &       62.147522 &         34 &      70.20 &       3.51 &      51.80 &       2.59 &      50.50 &       2.56 &      43.60 &       2.25 &      298.7 &       11.5 &      393.0 &        5.4 \\
       767 &      189.088806 &       62.148636 &         22 &      29.00 &       1.45 &      22.20 &       1.11 &      14.80 &       0.86 &      15.40 &       0.95 &      152.6 &       11.5 &      151.0 &        6.4 \\
       768 &      189.154282 &       62.147884 &         31 &      11.00 &       0.55 &      13.80 &       0.69 &      19.20 &       1.06 &      13.90 &       0.88 &       54.6 &        8.1 &      371.0 &        7.7 \\
       769 &      189.059708 &       62.147129 &         11 &      14.40 &       0.72 &      16.00 &       0.80 &      13.60 &       0.81 &      11.00 &       0.78 &       66.5 &       11.8 &       35.1 &        7.4 \\
       770 &      189.156769 &       62.144451 &         25 &      38.90 &       1.95 &      23.70 &       1.19 &      21.90 &       1.18 &      14.00 &       0.89 &       95.8 &        8.5 &       89.6 &        7.0 \\
       771 &      189.209213 &       62.145710 &         34 &      91.00 &       4.55 &      76.80 &       3.84 &      71.60 &       3.61 &     128.00 &       6.42 &      337.6 &       15.2 &      596.0 &        8.9 \\
       772 &      189.228424 &       62.146469 &         27 &      67.50 &       3.38 &      47.40 &       2.37 &      44.70 &       2.28 &      47.30 &       2.42 &      169.0 &       10.9 &      255.0 &        6.9 \\
       773 &      189.105423 &       62.146313 &         18 &      29.70 &       1.49 &      21.00 &       1.05 &      19.10 &       1.05 &      14.90 &       0.93 &      189.1 &       11.7 &      212.0 &        7.1 \\
       774 &      189.274063 &       62.146194 &         22 &      42.50 &       2.13 &      37.40 &       1.87 &      27.20 &       1.47 &      22.40 &       1.31 &      124.8 &       12.4 &       90.9 &        7.4 \\
       775 &      189.078888 &       62.145699 &         11 &      56.70 &       2.84 &      39.60 &       1.98 &      27.30 &       1.43 &      20.30 &       1.16 &       46.5 &        9.2 &       54.7 &        5.8 \\
       776 &      189.150558 &       62.145298 &         20 &      54.20 &       2.71 &      38.70 &       1.94 &      39.60 &       2.03 &      39.50 &       2.05 &      206.8 &       11.8 &      217.0 &        8.7 \\
       777 &      189.256226 &       62.145012 &         20 &      29.20 &       1.46 &      20.40 &       1.02 &      21.30 &       1.17 &      16.40 &       1.01 &      114.4 &       10.5 &      179.0 &        7.0 \\
       778 &      189.126694 &       62.145309 &         43 &      20.70 &       1.04 &      13.60 &       0.68 &      14.70 &       0.86 &       8.92 &       0.71 &       87.0 &        9.1 &      104.0 &        4.3 \\
       779 &      189.248627 &       62.146511 &         22 &      11.00 &       0.55 &      13.70 &       0.69 &      11.90 &       0.75 &      10.60 &       0.77 &       56.0 &        9.4 &       85.0 &        5.6 \\
       780 &      189.166931 &       62.144493 &         30 &     128.00 &       6.40 &      82.10 &       4.11 &      82.00 &       4.12 &     420.00 &      21.01 &      288.1 &       11.3 &      326.0 &        5.6 \\
       781 &      189.101746 &       62.143410 &         33 &     112.00 &       5.60 &      79.10 &       3.96 &      67.10 &       3.38 &      54.50 &       2.78 &      471.9 &       22.9 &      624.0 &       11.5 \\
       782 &      189.110626 &       62.143169 &         30 &      24.00 &       1.20 &      27.90 &       1.40 &      23.10 &       1.24 &      22.00 &       1.23 &      125.2 &       15.0 &      139.0 &        6.4 \\
       783 &      189.138443 &       62.142982 &         26 &     106.00 &       5.30 &      93.80 &       4.69 &     101.00 &       5.07 &     118.00 &       5.93 &      516.1 &       27.0 &      779.0 &        7.9 \\
       784 &      189.225449 &       62.143066 &         19 &      35.70 &       1.79 &      34.70 &       1.74 &      40.70 &       2.08 &      53.50 &       2.73 &      132.8 &        8.1 &      263.0 &        5.7 \\
       785 &      189.194443 &       62.142582 &         29 &     113.00 &       5.65 &      82.00 &       4.10 &      69.70 &       3.51 &      64.60 &       3.28 &      653.9 &       18.1 &      991.0 &        8.8 \\
       786 &      189.191360 &       62.142784 &         29 &      28.90 &       1.45 &      21.50 &       1.08 &      16.30 &       0.93 &      16.80 &       1.00 &       47.5 &       10.5 &       49.3 &        6.8 \\
       787 &      189.262512 &       62.142513 &         18 &      12.10 &       0.61 &      13.90 &       0.70 &      17.40 &       1.02 &      12.50 &       0.91 &       44.2 &        7.0 &      232.0 &        7.9 \\
       788 &      189.183517 &       62.143173 &         21 &      54.10 &       2.71 &      37.30 &       1.87 &      31.20 &       1.62 &      24.20 &       1.33 &       63.0 &        6.8 &       76.2 &        7.4 \\
       789 &      189.224213 &       62.141022 &         19 &      30.20 &       1.51 &      21.20 &       1.06 &      20.00 &       1.09 &      19.10 &       1.11 &       79.6 &        9.4 &       72.8 &        3.8 \\
       790 &      189.240921 &       62.140888 &         19 &     131.00 &       6.55 &      89.30 &       4.47 &      77.30 &       3.89 &      54.70 &       2.80 &      155.9 &       11.7 &      167.0 &        6.8 \\
       791 &      189.143600 &       62.141083 &         21 &      14.70 &       0.74 &      12.90 &       0.65 &       8.86 &       0.63 &      10.70 &       0.77 &       93.1 &       13.1 &       78.9 &        5.4 \\
       792 &      189.189743 &       62.140324 &         31 &      55.90 &       2.80 &      49.30 &       2.47 &      42.00 &       2.15 &      78.10 &       3.94 &      220.9 &        7.4 &      236.0 &        8.4 \\
       793 &      189.193741 &       62.141171 &         36 &      20.10 &       1.01 &      13.00 &       0.65 &      12.20 &       0.75 &      11.00 &       0.78 &       44.8 &       10.5 &        0.0 &        0.0 \\
       794 &      189.111267 &       62.141621 &         30 &      25.60 &       1.28 &      18.20 &       0.91 &      16.90 &       0.95 &      16.90 &       1.01 &       79.2 &        8.3 &       51.2 &        4.8 \\
       795 &      189.176712 &       62.139381 &         31 &      12.60 &       0.63 &       8.86 &       0.45 &       8.22 &       0.60 &       7.21 &       0.66 &       46.8 &        8.9 &       78.6 &        5.9 \\
       796 &      189.195740 &       62.139660 &         30 &      44.60 &       2.23 &      27.60 &       1.38 &      24.40 &       1.30 &      16.50 &       0.99 &       49.3 &        8.5 &       66.0 &        5.9 \\
       797 &      189.076172 &       62.138779 &         11 &      44.50 &       2.23 &      32.30 &       1.62 &      23.90 &       1.28 &      17.90 &       1.05 &       82.0 &       19.1 &       92.1 &        7.1 \\
       798 &      189.138016 &       62.138836 &         25 &      30.00 &       1.50 &      20.00 &       1.00 &      16.30 &       0.93 &      11.40 &       0.79 &       79.4 &        8.3 &       96.8 &        6.4 \\
       799 &      189.105072 &       62.137360 &         25 &      66.30 &       3.32 &      63.40 &       3.17 &      46.30 &       2.36 &      41.20 &       2.13 &      256.3 &       11.3 &      191.0 &        7.1 \\
       800 &      189.140625 &       62.135406 &         27 &    3640.00 &    4673.55 &    2460.00 &     123.00 &    1750.00 &      87.50 &     951.00 &      47.55 &      272.1 &       12.0 &      216.0 &       10.0 \\
       801 &      189.233078 &       62.135620 &         20 &     116.00 &       5.80 &      81.80 &       4.09 &      78.90 &       3.98 &      82.10 &       4.15 &      551.4 &       19.2 &      859.0 &       10.8 \\
       802 &      189.179108 &       62.135498 &         41 &      16.20 &       0.81 &      11.00 &       0.55 &       8.82 &       0.63 &       7.93 &       0.68 &       82.2 &        9.1 &       88.2 &        6.6 \\
       803 &      189.227798 &       62.134502 &         23 &      58.60 &       2.93 &      47.00 &       2.35 &      39.30 &       2.03 &      35.40 &       1.88 &      304.0 &       10.9 &      269.0 &        5.7 \\
       804 &      189.135605 &       62.133293 &         19 &      22.80 &       1.14 &      28.00 &       1.40 &      48.60 &       2.47 &     108.00 &       5.43 &      408.3 &       14.4 &      820.0 &        9.6 \\
       805 &      189.209335 &       62.135006 &         26 &      19.40 &       0.97 &      14.10 &       0.71 &      13.00 &       0.79 &      15.60 &       0.97 &       56.0 &        8.0 &       52.9 &        5.9 \\
       806 &      189.215866 &       62.131500 &         27 &      43.30 &       2.17 &      31.90 &       1.60 &      25.50 &       1.36 &      24.70 &       1.39 &      247.4 &       10.4 &      288.0 &        5.5 \\
       807 &      189.142715 &       62.131828 &         28 &      29.40 &       1.47 &      17.40 &       0.87 &      14.90 &       0.87 &      11.10 &       0.79 &       67.9 &        8.0 &       83.5 &        8.2 \\
       808 &      189.202347 &       62.133717 &         20 &      11.90 &       0.60 &       8.52 &       0.43 &      13.50 &       0.82 &       5.20 &       0.63 &       72.0 &        9.1 &       54.0 &        6.9 \\
       809 &      189.242310 &       62.132034 &         16 &      74.50 &       3.73 &      56.60 &       2.83 &      41.90 &       2.17 &      34.10 &       1.87 &      155.3 &       12.6 &      153.0 &        6.7 \\
       810 &      189.208633 &       62.133751 &         22 &      34.60 &       1.73 &      26.60 &       1.33 &      31.80 &       1.66 &      41.00 &       2.13 &      180.3 &        9.8 &      226.0 &        7.0 \\
       811 &      189.190948 &       62.131733 &         19 &      38.20 &       1.91 &      44.00 &       2.20 &      34.80 &       1.80 &      44.80 &       2.31 &      323.4 &       15.2 &      374.0 &        7.9 \\
       812 &      189.087982 &       62.130737 &         12 &      22.30 &       1.12 &      17.10 &       0.86 &      19.90 &       1.09 &      22.10 &       1.24 &      124.0 &       16.3 &      141.0 &        7.6 \\
       813 &      189.125793 &       62.129562 &         23 &      25.40 &       1.27 &      23.80 &       1.19 &      18.40 &       1.02 &      18.60 &       1.08 &      105.3 &       12.8 &       78.9 &        5.7 \\
       814 &      189.226196 &       62.129200 &         24 &      94.20 &       4.71 &      79.70 &       3.99 &      72.20 &       3.65 &     442.00 &      22.11 &      579.7 &       18.3 &      796.0 &        8.5 \\
       815 &      189.090576 &       62.128605 &         12 &      19.20 &       0.96 &      19.00 &       0.95 &      14.10 &       0.84 &      14.60 &       0.92 &       97.4 &       12.6 &       64.6 &        5.8 \\
       816 &      189.153625 &       62.126404 &         31 &      30.60 &       1.53 &      21.80 &       1.09 &      17.50 &       0.98 &      17.10 &       1.02 &      162.2 &        7.4 &      174.0 &        7.5 \\
       817 &      189.206879 &       62.127247 &         20 &      34.80 &       1.74 &      55.40 &       2.77 &      97.50 &       4.90 &     213.00 &      10.67 &      779.4 &       23.3 &     1440.0 &       12.6 \\
       818 &      189.134903 &       62.126148 &         30 &      98.40 &       4.92 &      63.00 &       3.15 &      59.30 &       3.00 &      38.20 &       1.99 &      138.3 &        9.6 &      116.0 &        5.4 \\
       819 &      189.172653 &       62.125008 &         22 &      10.20 &       0.51 &       7.38 &       0.38 &       4.58 &       0.50 &       4.81 &       0.63 &       44.2 &        7.6 &       24.5 &        6.8 \\
       820 &      189.113174 &       62.127228 &         13 &      20.70 &       1.04 &      20.90 &       1.05 &      17.50 &       0.98 &      21.40 &       1.21 &       81.6 &       12.6 &       50.1 &        6.3 \\
       821 &      189.113327 &       62.126118 &         11 &      35.30 &       1.77 &      29.80 &       1.49 &      23.40 &       1.25 &      41.50 &       2.15 &       68.2 &       12.6 &       66.7 &        5.4 \\
       822 &      189.220566 &       62.124168 &         14 &   10900.00 &     545.00 &    9480.00 &     474.00 &   10200.00 &     510.00 &    5490.00 &     274.50 &     1527.0 &       48.7 &      801.0 &       14.5 \\
       823 &      189.102600 &       62.124302 &         10 &      22.90 &       1.15 &      19.40 &       0.97 &      15.40 &       0.89 &      26.20 &       1.42 &       74.9 &       14.4 &       71.0 &        5.0 \\
       824 &      189.164658 &       62.123413 &         34 &      33.40 &       1.67 &      21.90 &       1.10 &      20.20 &       1.10 &      13.80 &       0.90 &      130.3 &        9.2 &      150.0 &        7.0 \\
       825 &      189.103348 &       62.122005 &         10 &      82.10 &       4.11 &      55.60 &       2.78 &      49.90 &       2.54 &     232.00 &      11.61 &      167.4 &       15.7 &      304.0 &        5.8 \\
       826 &      189.157639 &       62.123215 &         32 &      25.40 &       1.27 &      17.30 &       0.87 &      17.80 &       1.00 &      13.70 &       0.89 &      144.0 &        7.4 &      145.0 &        6.9 \\
       827 &      189.107254 &       62.120735 &         13 &      11.50 &       0.58 &       8.99 &       0.45 &       6.96 &       0.57 &       8.34 &       0.70 &       81.2 &       16.5 &       58.7 &        5.6 \\
       828 &      189.143326 &       62.121876 &         22 &      13.20 &       0.66 &       8.41 &       0.43 &       7.62 &       0.58 &       6.03 &       0.64 &       66.7 &       12.0 &       47.2 &        7.2 \\
       829 &      189.116943 &       62.121067 &         12 &      25.40 &       1.27 &      24.80 &       1.24 &      20.30 &       1.11 &      19.40 &       1.12 &      114.4 &       15.2 &      103.0 &        5.6 \\
       830 &      189.145126 &       62.119488 &         18 &      69.90 &       3.50 &      46.60 &       2.33 &      52.00 &       2.64 &      44.20 &       2.28 &      282.8 &       17.4 &      380.0 &       12.2 \\
       831 &      189.149368 &       62.118793 &         19 &     108.00 &       5.40 &      87.60 &       4.38 &      70.60 &       3.56 &     103.00 &       5.18 &      258.0 &       25.5 &       44.8 &       12.2 \\
       832 &      189.151535 &       62.118595 &         23 &      71.70 &       3.59 &      66.10 &       3.31 &      55.00 &       2.79 &     190.00 &       9.52 &      339.4 &       18.3 &      594.0 &       16.2 \\
       833 &      189.195312 &       62.116627 &         12 &      14.40 &       0.72 &      10.30 &       0.52 &       9.77 &       0.72 &       5.91 &       0.81 &       74.2 &       15.4 &       54.4 &        7.0 \\
       834 &      189.163162 &       62.116405 &         24 &      12.30 &       0.62 &       7.75 &       0.39 &       6.91 &       0.58 &       5.22 &       0.66 &       43.0 &        7.6 &       31.7 &        6.9 \\
       835 &      189.108246 &       62.115345 &         16 &      80.70 &       4.04 &      51.90 &       2.60 &      51.80 &       2.63 &      36.70 &       1.92 &      196.2 &       13.9 &      220.0 &        6.8 \\
       836 &      189.122955 &       62.112942 &         12 &      54.50 &       2.73 &      35.60 &       1.78 &      40.20 &       2.06 &      31.20 &       1.66 &      374.7 &       18.9 &      372.0 &        6.2 \\
       837 &      189.184174 &       62.112999 &         19 &      49.90 &       2.50 &      37.70 &       1.89 &      27.10 &       1.45 &      20.40 &       1.27 &       68.2 &       11.5 &       67.9 &        6.6 \\
       838 &      189.132477 &       62.112114 &         13 &      31.80 &       1.59 &      41.50 &       2.08 &      42.10 &       2.15 &      32.90 &       1.74 &       98.8 &       15.5 &      347.0 &        9.8 \\
       839 &      189.143692 &       62.107803 &         17 &      70.60 &       3.53 &      64.70 &       3.24 &      47.00 &       2.40 &      39.80 &       2.08 &      167.0 &       19.8 &      108.0 &        8.8 \\


==> Table3_data.tex <==
         0 &       53.103943 &    -27.663679 &          2 &      29.60 &       1.48 &      20.80 &       1.05 &      23.70 &       1.37 &      17.00 &       1.10 &      120.5 &       23.7 &      120.0 &        5.7 \\
         1 &       53.142094 &    -27.664965 &          2 &      33.70 &       1.69 &      26.00 &       1.30 &      21.40 &       1.19 &      22.30 &       1.24 &      252.7 &       25.3 &      161.0 &        8.8 \\
         2 &       53.144711 &    -27.666069 &          3 &     171.00 &       8.55 &     149.00 &       7.45 &     112.00 &       5.62 &     576.00 &      28.81 &      830.6 &       39.8 &      938.0 &       11.5 \\
         3 &       53.110268 &    -27.667072 &          2 &      26.90 &       1.35 &      22.30 &       1.12 &      16.30 &       1.00 &      16.80 &       1.03 &      208.5 &       19.4 &      143.0 &        5.6 \\
         4 &       53.103607 &    -27.666225 &          4 &      21.10 &       1.06 &      19.70 &       0.99 &      13.80 &       0.92 &      13.00 &       0.90 &       81.8 &       14.6 &       44.2 &        4.9 \\
         5 &       53.102222 &    -27.669676 &          3 &      46.90 &       2.35 &      35.90 &       1.80 &      33.60 &       1.77 &      40.40 &       2.10 &      251.0 &       38.7 &      322.0 &        6.6 \\
         6 &       53.110622 &    -27.669182 &          3 &      31.10 &       1.56 &      26.90 &       1.35 &      20.50 &       1.17 &      17.30 &       1.04 &       99.2 &       17.9 &       74.0 &        5.4 \\
         7 &       53.123016 &    -27.669071 &          3 &     102.00 &       5.10 &      63.70 &       3.19 &      60.70 &       3.08 &      40.60 &       2.10 &      201.5 &       20.2 &      256.0 &        5.3 \\
         8 &       53.126549 &    -27.669138 &          3 &      25.90 &       1.30 &      26.20 &       1.31 &      19.70 &       1.11 &      19.90 &       1.14 &      174.7 &       15.9 &      118.0 &        5.1 \\
         9 &       53.129875 &    -27.671673 &          4 &      61.40 &       3.07 &      43.80 &       2.19 &      45.70 &       2.34 &      39.40 &       2.04 &      199.7 &       24.8 &      203.0 &        4.9 \\
        10 &       53.147671 &    -27.672302 &          4 &      44.70 &       2.24 &      39.10 &       1.96 &      27.80 &       1.47 &      25.60 &       1.38 &      158.2 &       24.8 &      108.0 &        4.9 \\
        11 &       53.102448 &    -27.672508 &          4 &      28.80 &       1.44 &      22.20 &       1.11 &      16.80 &       0.99 &      16.30 &       0.98 &      169.0 &       16.8 &      162.0 &        5.5 \\
        12 &       53.109512 &    -27.674276 &          4 &      28.50 &       1.43 &      22.10 &       1.11 &      19.20 &       1.08 &      22.10 &       1.23 &      180.3 &       17.4 &      175.0 &       11.9 \\
        13 &       53.114948 &    -27.674074 &          4 &      25.50 &       1.28 &      18.20 &       0.91 &      13.90 &       0.85 &      12.10 &       0.80 &      107.8 &       17.0 &       67.8 &        5.4 \\
        14 &       53.127071 &    -27.675257 &          4 &      33.80 &       1.69 &      32.10 &       1.61 &      25.40 &       1.35 &      19.10 &       1.09 &      116.0 &       16.5 &       57.1 &        3.9 \\
        15 &       53.090645 &    -27.675821 &          3 &      42.60 &       2.13 &      41.00 &       2.05 &      33.30 &       1.74 &      84.40 &       4.25 &      215.6 &       19.8 &      272.0 &        4.0 \\
        16 &       53.110355 &    -27.676670 &          5 &     198.00 &       9.90 &     258.00 &      12.90 &     387.00 &      19.36 &     543.00 &      27.16 &     1325.5 &       50.0 &     2160.0 &       19.4 \\
        17 &       53.123756 &    -27.677969 &          9 &      33.10 &       1.66 &      26.90 &       1.35 &      20.00 &       1.10 &      29.40 &       1.56 &      122.3 &       15.9 &      135.0 &        3.8 \\
        18 &       53.084019 &    -27.680033 &          6 &      28.70 &       1.44 &      24.90 &       1.25 &      21.60 &       1.18 &      21.10 &       1.17 &      155.5 &       18.9 &      116.0 &        4.3 \\
        19 &       53.080742 &    -27.681108 &          3 &      95.90 &       4.80 &      77.70 &       3.89 &      95.30 &       4.79 &     107.00 &       5.38 &      394.2 &       31.5 &      740.0 &        8.8 \\
        20 &       53.090210 &    -27.682375 &          3 &      17.80 &       0.89 &      14.70 &       0.74 &      11.40 &       0.73 &      13.50 &       0.84 &      135.9 &       19.6 &      115.0 &        3.8 \\
        21 &       53.129295 &    -27.680716 &          4 &      60.50 &       3.03 &      45.20 &       2.26 &      32.90 &       1.71 &      27.50 &       1.47 &      122.7 &       18.9 &      170.0 &        3.4 \\
        22 &       53.128834 &    -27.683001 &          5 &      13.20 &       0.66 &       8.05 &       0.41 &       7.88 &       0.60 &       5.58 &       0.58 &       98.0 &       17.9 &       46.7 &        3.1 \\
        23 &       53.085453 &    -27.683109 &          6 &      20.20 &       1.01 &      14.70 &       0.74 &      14.20 &       0.84 &       9.06 &       0.67 &      110.7 &       14.4 &      131.0 &        4.3 \\
        24 &       53.104046 &    -27.683870 &          3 &      53.30 &       2.67 &      34.20 &       1.71 &      34.60 &       1.79 &      24.20 &       1.31 &      104.3 &       13.7 &      145.0 &        3.8 \\
        25 &       53.135242 &    -27.682543 &          7 &      32.70 &       1.64 &      27.80 &       1.39 &      24.70 &       1.31 &      27.40 &       1.46 &      149.9 &       12.6 &      205.0 &        5.1 \\
        26 &       53.142612 &    -27.684610 &          4 &      19.20 &       0.96 &      20.20 &       1.01 &      17.30 &       0.97 &      17.70 &       1.02 &      187.4 &       17.6 &       76.5 &        3.5 \\
        27 &       53.112488 &    -27.684843 &          5 &     395.00 &      19.75 &     464.00 &      23.20 &     579.00 &      28.95 &     648.00 &      32.40 &      797.1 &       40.1 &      993.0 &        7.0 \\
        28 &       53.088100 &    -27.685289 &          6 &      79.60 &       3.98 &      65.40 &       3.27 &      45.10 &       2.30 &      39.00 &       2.01 &      167.2 &       17.6 &      191.0 &        4.2 \\
        29 &       53.081654 &    -27.688253 &          5 &      30.60 &       1.53 &      31.30 &       1.57 &      26.40 &       1.39 &      33.50 &       1.75 &      201.5 &       14.6 &       65.5 &        9.3 \\
        30 &       53.158722 &    -27.687243 &          3 &      43.40 &       2.17 &      40.90 &       2.05 &      28.70 &       1.50 &      90.40 &       4.55 &      199.7 &       19.8 &      244.0 &        4.9 \\
        31 &       53.065475 &    -27.687944 &          3 &      15.90 &       0.80 &      12.70 &       0.64 &       9.82 &       0.68 &       9.97 &       0.72 &       96.2 &       17.2 &       94.1 &        4.2 \\
        32 &       53.137383 &    -27.688189 &          5 &     127.00 &       6.35 &      94.90 &       4.75 &      66.10 &       3.34 &      51.10 &       2.61 &       97.2 &       12.0 &      134.0 &        3.3 \\
        33 &       53.131115 &    -27.688498 &          7 &      35.00 &       1.75 &      22.40 &       1.12 &      22.90 &       1.23 &      15.70 &       0.94 &      136.1 &       11.8 &      138.0 &        4.9 \\
        34 &       53.087513 &    -27.687744 &          6 &      16.50 &       0.83 &      18.80 &       0.94 &      17.80 &       0.99 &      18.30 &       1.04 &       85.9 &       14.2 &       98.7 &        3.4 \\
        35 &       53.082500 &    -27.689766 &          3 &     162.00 &       8.10 &     176.00 &       8.80 &     216.00 &      10.81 &     395.00 &      19.76 &     1170.0 &       38.1 &     3310.0 &       21.3 \\
        36 &       53.041489 &    -27.688335 &          2 &     515.00 &      25.75 &     320.00 &      16.00 &     217.00 &      10.86 &     114.00 &       5.73 &       93.1 &       17.4 &        9.6 &        6.6 \\
        37 &       53.137024 &    -27.690088 &          5 &      49.50 &       2.48 &      37.70 &       1.89 &      27.90 &       1.46 &      25.70 &       1.38 &      219.1 &       23.7 &      226.0 &        3.9 \\
        38 &       53.084435 &    -27.692427 &          4 &      90.60 &       4.53 &      64.00 &       3.20 &      45.40 &       2.31 &     173.00 &       8.66 &      155.5 &       18.5 &      184.0 &        6.3 \\
        39 &       53.139149 &    -27.694260 &          5 &      45.50 &       2.28 &      34.20 &       1.71 &      24.50 &       1.30 &      21.50 &       1.19 &      104.6 &       15.0 &      139.0 &        4.2 \\
        40 &       53.074039 &    -27.694685 &          5 &      14.80 &       0.74 &      13.90 &       0.70 &       8.85 &       0.63 &       8.67 &       0.66 &       95.5 &       12.8 &       46.3 &        2.9 \\
        41 &       53.115063 &    -27.695923 &          8 &      53.10 &       2.66 &      53.50 &       2.68 &      72.90 &       3.67 &      95.30 &       4.79 &      210.3 &       16.1 &      412.0 &        6.0 \\
        42 &       53.111485 &    -27.696098 &          3 &      58.90 &       2.95 &      49.50 &       2.48 &      60.50 &       3.06 &      73.20 &       3.69 &      169.6 &       20.7 &      420.0 &        5.5 \\
        43 &       53.038292 &    -27.696741 &          3 &      56.10 &       2.81 &      52.10 &       2.61 &      35.90 &       1.85 &     172.00 &       8.62 &      316.3 &       24.6 &      285.0 &        4.3 \\
        44 &       53.023373 &    -27.695400 &          2 &      56.70 &       2.84 &      54.40 &       2.72 &      43.50 &       2.23 &      39.00 &       2.02 &      314.6 &       24.4 &      179.0 &        5.9 \\
        45 &       53.135078 &    -27.697430 &          4 &      21.70 &       1.09 &      20.90 &       1.05 &      14.80 &       0.86 &      16.10 &       0.95 &      133.6 &       16.3 &       97.4 &        3.6 \\
        46 &       53.127319 &    -27.696169 &          4 &      17.30 &       0.87 &      11.30 &       0.57 &      11.80 &       0.74 &       7.30 &       0.62 &       86.4 &       15.4 &       93.6 &        4.3 \\
        47 &       53.078903 &    -27.697836 &          3 &      24.20 &       1.21 &      17.50 &       0.88 &      15.30 &       0.88 &      12.50 &       0.80 &      101.8 &       15.9 &      133.0 &        3.1 \\
        48 &       53.053337 &    -27.700537 &          4 &      28.80 &       1.44 &      19.90 &       1.00 &      15.50 &       0.90 &      15.50 &       0.93 &      122.3 &       12.4 &      133.0 &        4.0 \\
        49 &       53.129696 &    -27.701571 &          4 &      33.20 &       1.66 &      35.00 &       1.75 &      31.60 &       1.64 &      27.20 &       1.45 &       96.7 &       17.6 &      175.0 &        3.6 \\
        50 &       53.133595 &    -27.702093 &          4 &      55.70 &       2.79 &      38.60 &       1.93 &      29.30 &       1.53 &      26.20 &       1.40 &      205.0 &       20.4 &      181.0 &        3.1 \\
        51 &       53.062340 &    -27.706976 &          8 &     109.00 &       5.45 &     118.00 &       5.90 &     115.00 &       5.77 &      85.60 &       4.31 &      151.8 &       20.5 &      169.0 &        5.5 \\
        52 &       53.104721 &    -27.705404 &          3 &      65.10 &       3.26 &      82.80 &       4.14 &     100.00 &       5.02 &     122.00 &       6.12 &      243.9 &       19.4 &      583.0 &        9.6 \\
        53 &       53.138279 &    -27.706007 &          3 &     501.00 &      25.05 &     302.00 &      15.10 &     212.00 &      10.61 &     118.00 &       5.92 &       79.2 &       14.8 &       17.9 &        3.3 \\
        54 &       53.109268 &    -27.706430 &          4 &      28.00 &       1.40 &      18.90 &       0.95 &      18.80 &       1.03 &      13.50 &       0.84 &       89.8 &       14.2 &       91.7 &        4.1 \\
        55 &       53.090031 &    -27.706718 &          5 &      50.00 &       2.50 &      33.80 &       1.69 &      35.10 &       1.81 &      28.10 &       1.49 &      194.4 &       15.4 &      242.0 &        4.7 \\
        56 &       53.144173 &    -27.706825 &          7 &      68.40 &       3.42 &      59.60 &       2.98 &      53.70 &       2.72 &     107.00 &       5.37 &      243.9 &       22.9 &      294.0 &        3.5 \\
        57 &       53.142731 &    -27.707096 &          7 &      82.00 &       4.10 &      65.80 &       3.29 &      46.80 &       2.38 &      46.60 &       2.38 &      145.5 &       20.4 &       72.8 &        3.0 \\
        58 &       53.167648 &    -27.706707 &          3 &    4090.00 &    4674.48 &    2720.00 &     136.00 &    1820.00 &      91.00 &    1020.00 &      51.00 &      273.9 &       18.7 &      120.0 &        4.5 \\
        59 &       53.089211 &    -27.708727 &          6 &      45.90 &       2.30 &      28.80 &       1.44 &      27.10 &       1.42 &      20.30 &       1.13 &      106.8 &       16.5 &      110.0 &        3.4 \\
        60 &       53.091022 &    -27.708309 &          5 &      16.90 &       0.85 &      12.70 &       0.64 &      10.50 &       0.67 &       8.15 &       0.64 &       95.3 &       13.5 &       70.3 &        4.1 \\
        61 &       53.086037 &    -27.709669 &          3 &      27.90 &       1.40 &      32.50 &       1.63 &      34.00 &       1.75 &      24.10 &       1.30 &       83.6 &       10.2 &      459.0 &        6.2 \\
        62 &       53.141190 &    -27.710651 &          4 &      25.10 &       1.26 &      17.50 &       0.88 &      19.40 &       1.07 &      16.00 &       0.95 &      122.8 &       18.9 &      116.0 &        4.1 \\
        63 &       53.119282 &    -27.709436 &          4 &      14.00 &       0.70 &       9.88 &       0.50 &       7.29 &       0.57 &       6.28 &       0.59 &       75.5 &       13.7 &       46.4 &        3.5 \\
        64 &       53.033234 &    -27.711037 &          4 &      30.60 &       1.53 &      32.30 &       1.62 &      46.30 &       2.36 &      69.70 &       3.52 &      256.3 &       18.5 &      522.0 &        6.9 \\
        65 &       53.112137 &    -27.711151 &          4 &      16.00 &       0.80 &      17.70 &       0.89 &      14.50 &       0.84 &      15.90 &       0.94 &       82.7 &       13.5 &      162.0 &        4.3 \\
        66 &       53.055115 &    -27.711466 &          4 &     136.00 &       6.80 &      99.90 &       5.00 &     109.00 &       5.47 &     102.00 &       5.13 &      440.1 &       19.4 &      774.0 &        9.4 \\
        67 &       53.091717 &    -27.712198 &          6 &      20.80 &       1.04 &      25.90 &       1.30 &      24.90 &       1.32 &      22.80 &       1.24 &      110.7 &       15.4 &      229.0 &        4.0 \\
        68 &       53.089458 &    -27.711670 &          4 &      27.90 &       1.40 &      34.20 &       1.71 &      33.30 &       1.72 &      26.20 &       1.40 &       86.3 &       10.7 &      316.0 &        4.2 \\
        69 &       53.020447 &    -27.711840 &          5 &      40.40 &       2.02 &      25.70 &       1.29 &      25.60 &       1.36 &      18.40 &       1.06 &      108.0 &       23.3 &      142.0 &        5.0 \\
        70 &       53.044804 &    -27.709705 &          5 &     205.00 &      10.25 &     155.00 &       7.75 &     114.00 &       5.72 &      78.20 &       3.94 &      100.9 &       13.3 &      100.0 &        3.3 \\
        71 &       53.059620 &    -27.711975 &          4 &      16.10 &       0.81 &      14.10 &       0.71 &       9.79 &       0.66 &      10.70 &       0.74 &      107.4 &       12.2 &       55.2 &        4.4 \\
        72 &       53.123478 &    -27.711927 &          6 &      62.90 &       3.15 &      56.80 &       2.84 &      70.40 &       3.55 &      79.30 &       4.00 &      334.1 &       21.8 &      561.0 &        7.8 \\
        73 &       53.057720 &    -27.713686 &          4 &      69.60 &       3.48 &      47.50 &       2.38 &      50.50 &       2.56 &      52.30 &       2.66 &      155.2 &       19.4 &      333.0 &        6.5 \\
        74 &       53.038441 &    -27.714302 &          5 &      43.10 &       2.16 &      36.30 &       1.82 &      25.70 &       1.36 &      47.60 &       2.43 &      117.5 &       14.2 &      123.0 &        3.5 \\
        75 &       53.023632 &    -27.714966 &          5 &      21.80 &       1.09 &      19.90 &       1.00 &      14.30 &       0.84 &      14.90 &       0.91 &      123.2 &       16.6 &       85.7 &        5.2 \\
        76 &       53.021313 &    -27.714842 &          3 &      27.80 &       1.39 &      22.60 &       1.13 &      24.70 &       1.32 &      30.50 &       1.61 &      124.8 &       14.4 &      188.0 &        5.7 \\
        77 &       53.097618 &    -27.715397 &          5 &      12.60 &       0.63 &      14.20 &       0.71 &      15.90 &       0.90 &      15.60 &       0.92 &      101.5 &       14.8 &      227.0 &        4.2 \\
        78 &       53.120865 &    -27.715496 &          7 &      57.80 &       2.89 &      43.50 &       2.18 &      31.70 &       1.64 &      26.10 &       1.40 &      198.0 &       13.7 &      220.0 &        4.1 \\
        79 &       53.150784 &    -27.716204 &          6 &      30.60 &       1.53 &      21.70 &       1.09 &      19.00 &       1.05 &      18.50 &       1.05 &      169.2 &       16.1 &      205.0 &        4.1 \\
        80 &       53.071396 &    -27.717684 &          5 &      72.20 &       3.61 &      62.10 &       3.11 &      66.50 &       3.35 &      87.50 &       4.40 &      394.2 &       18.1 &     1580.0 &       12.7 \\
        81 &       53.082180 &    -27.718332 &          3 &      26.10 &       1.31 &      20.00 &       1.00 &      15.70 &       0.88 &      13.10 &       0.81 &       88.6 &       15.9 &      119.0 &        4.1 \\
        82 &       53.124748 &    -27.717226 &          7 &      33.40 &       1.67 &      35.20 &       1.76 &      27.90 &       1.46 &      31.50 &       1.65 &      300.5 &       15.0 &      173.0 &        3.3 \\
        83 &       53.106983 &    -27.718338 &          4 &      17.10 &       0.86 &      29.90 &       1.50 &      69.30 &       3.49 &     155.00 &       7.77 &      420.6 &       26.3 &      544.0 &        5.7 \\
        84 &       53.171787 &    -27.719475 &          4 &      17.60 &       0.88 &      16.90 &       0.85 &      12.60 &       0.77 &      12.70 &       0.81 &      146.0 &       16.8 &       66.8 &        4.5 \\
        85 &       53.043800 &    -27.719297 &          7 &      80.10 &       4.01 &      74.50 &       3.73 &      82.60 &       4.15 &      89.40 &       4.50 &      279.3 &       18.7 &      513.0 &        3.7 \\
        86 &       53.162876 &    -27.718601 &          4 &      76.00 &       3.80 &      47.50 &       2.38 &      45.90 &       2.34 &      32.90 &       1.72 &      182.1 &       21.1 &      226.0 &        5.4 \\
        87 &       53.169273 &    -27.719110 &          5 &      24.10 &       1.21 &      21.60 &       1.08 &      14.20 &       0.84 &      17.80 &       1.02 &      162.4 &       16.3 &      141.0 &        4.0 \\
        88 &       53.016754 &    -27.719076 &          5 &      51.60 &       2.58 &      33.10 &       1.66 &      31.90 &       1.67 &      22.00 &       1.23 &      104.6 &       17.0 &       87.5 &        4.7 \\
        89 &       53.048035 &    -27.720003 &          4 &      58.00 &       2.90 &      48.90 &       2.45 &      36.30 &       1.87 &      32.30 &       1.69 &      159.2 &       24.4 &      188.0 &        2.9 \\
        90 &       53.139381 &    -27.720325 &          3 &     496.00 &      24.80 &     321.00 &      16.05 &     220.00 &      11.01 &     273.00 &      13.66 &      242.2 &       25.2 &      193.0 &        4.3 \\
        91 &       53.097481 &    -27.721367 &          6 &      69.30 &       3.47 &      46.30 &       2.32 &      48.20 &       2.45 &      37.50 &       1.94 &      196.2 &       15.4 &      248.0 &        4.3 \\
        92 &       53.128075 &    -27.721592 &          8 &      19.50 &       0.98 &      14.40 &       0.72 &      11.90 &       0.74 &      10.80 &       0.73 &       80.8 &       10.7 &       93.0 &        3.3 \\
        93 &       53.042938 &    -27.721493 &          4 &      67.60 &       3.38 &      45.50 &       2.28 &      36.30 &       1.87 &     132.00 &       6.62 &      103.9 &       18.7 &       91.7 &        3.8 \\
        94 &       53.125237 &    -27.722040 &          7 &      62.80 &       3.14 &      51.00 &       2.55 &      35.70 &       1.84 &      36.90 &       1.91 &      309.3 &       15.0 &      332.0 &        4.0 \\
        95 &       53.169445 &    -27.721010 &          4 &      43.10 &       2.16 &      31.40 &       1.57 &      28.70 &       1.50 &      23.90 &       1.29 &       76.9 &       14.6 &      135.0 &        5.7 \\
        96 &       53.001457 &    -27.722212 &          3 &      27.20 &       1.36 &      28.60 &       1.43 &      32.60 &       1.76 &      38.70 &       2.08 &       99.7 &       17.2 &      110.0 &        4.6 \\
        97 &       53.051125 &    -27.723465 &          6 &      14.80 &       0.74 &      14.60 &       0.73 &      10.40 &       0.68 &      11.80 &       0.78 &       97.6 &       16.5 &       34.6 &        3.9 \\
        98 &       53.130848 &    -27.723438 &          2 &      32.80 &       1.64 &      25.10 &       1.26 &      17.40 &       0.97 &      15.90 &       0.94 &      153.2 &       14.4 &      114.0 &        2.6 \\
        99 &       53.173748 &    -27.724571 &          4 &      47.30 &       2.37 &      37.00 &       1.85 &      31.20 &       1.62 &      29.60 &       1.56 &      163.7 &       17.2 &      180.0 &        4.6 \\
       100 &       53.045628 &    -27.725025 &          6 &      24.90 &       1.25 &      21.10 &       1.06 &      13.90 &       0.82 &      14.70 &       0.89 &      126.2 &       14.2 &       95.1 &        3.1 \\
       101 &       53.004604 &    -27.725391 &          4 &      48.20 &       2.41 &      35.80 &       1.79 &      29.80 &       1.61 &      24.90 &       1.43 &      213.8 &       19.8 &      208.0 &        4.8 \\
       102 &       53.058815 &    -27.726452 &          4 &      17.40 &       0.87 &      21.10 &       1.06 &      21.00 &       1.14 &      23.20 &       1.27 &      104.5 &       17.2 &      156.0 &        3.9 \\
       103 &       53.016579 &    -27.727161 &          4 &      67.40 &       3.37 &      49.70 &       2.49 &      41.90 &       2.15 &      34.00 &       1.79 &      321.6 &       20.4 &      317.0 &        6.8 \\
       104 &       53.151691 &    -27.727455 &          4 &      11.70 &       0.59 &      10.90 &       0.55 &       9.49 &       0.64 &       8.65 &       0.65 &       69.3 &       13.7 &       28.4 &        4.1 \\
       105 &       53.006943 &    -27.730476 &          4 &      10.10 &       0.51 &      10.30 &       0.52 &      10.10 &       0.79 &       8.97 &       0.82 &      107.0 &       17.6 &       38.8 &        4.8 \\
       106 &       53.045422 &    -27.728710 &          5 &      67.90 &       3.40 &      48.10 &       2.41 &      37.10 &       1.91 &      29.40 &       1.56 &      115.0 &       21.1 &      120.0 &        3.2 \\
       107 &       53.125065 &    -27.729931 &          4 &      96.60 &       4.83 &      59.70 &       2.99 &      58.50 &       2.96 &      39.00 &       2.01 &      210.3 &       18.3 &      204.0 &        3.3 \\
       108 &       53.051559 &    -27.731646 &          6 &      43.30 &       2.17 &      42.60 &       2.13 &      34.60 &       1.79 &      98.20 &       4.94 &      249.2 &       15.2 &      298.0 &        5.3 \\
       109 &       53.029819 &    -27.732307 &          7 &      32.30 &       1.62 &      26.60 &       1.33 &      18.60 &       1.03 &      16.70 &       0.98 &      110.5 &       17.0 &       83.8 &        4.8 \\
       110 &       53.132580 &    -27.732405 &          7 &      19.40 &       0.97 &      21.50 &       1.08 &      15.90 &       0.90 &      15.60 &       0.92 &       70.8 &       11.8 &      135.0 &        3.0 \\
       111 &       53.124901 &    -27.734797 &          2 &     611.00 &       0.12 &     416.00 &       0.12 &     571.00 &       0.61 &    3670.00 &       0.65 &     2944.3 &      128.2 &     4660.0 &      466.0 \\
       112 &       53.123913 &    -27.733496 &          4 &      28.10 &       1.41 &      20.90 &       1.05 &      31.40 &       1.63 &     175.00 &       8.76 &      163.1 &       31.8 &        0.0 &        0.0 \\
       113 &       53.186588 &    -27.735188 &          3 &     143.00 &       7.15 &      96.20 &       4.81 &      67.30 &       3.39 &     158.00 &       7.92 &      176.6 &       21.5 &      217.0 &        4.2 \\
       114 &       53.155796 &    -27.735376 &          5 &      28.50 &       1.43 &      21.20 &       1.06 &      14.80 &       0.85 &      14.60 &       0.87 &      162.1 &       14.4 &      144.0 &        3.5 \\
       115 &       52.999462 &    -27.735390 &          2 &      26.80 &       1.34 &      19.50 &       0.99 &      14.70 &       1.18 &      13.00 &       1.17 &      149.9 &       17.0 &       87.2 &        5.8 \\
       116 &       53.112556 &    -27.735334 &          5 &      40.70 &       2.04 &      33.80 &       1.69 &      25.20 &       1.33 &      24.00 &       1.29 &      173.4 &       18.7 &      204.0 &        5.2 \\
       117 &       53.049400 &    -27.737133 &          4 &      21.60 &       1.08 &      20.00 &       1.00 &      14.20 &       0.84 &      15.40 &       0.92 &      148.8 &       21.8 &      103.0 &        5.0 \\
       118 &       53.045444 &    -27.737576 &          4 &      42.10 &       2.11 &      55.80 &       2.79 &      74.30 &       3.74 &      90.70 &       4.56 &      185.6 &       19.6 &      293.0 &        4.9 \\
       119 &       53.175194 &    -27.739344 &          6 &      14.30 &       0.72 &      12.00 &       0.60 &       8.51 &       0.60 &       7.33 &       0.60 &       91.7 &       15.7 &       56.3 &        4.4 \\
       120 &       53.140648 &    -27.738277 &          5 &      13.30 &       0.67 &      12.70 &       0.64 &       9.64 &       0.64 &       9.57 &       0.68 &      102.3 &       15.7 &       50.6 &        3.0 \\
       121 &       53.014751 &    -27.738739 &          4 &      33.90 &       1.70 &      26.80 &       1.34 &      24.00 &       1.31 &      33.00 &       1.76 &      148.5 &       20.9 &      161.0 &        7.2 \\
       122 &       53.094082 &    -27.740602 &          6 &     105.00 &       5.25 &      67.80 &       3.39 &      69.40 &       3.50 &      56.60 &       2.87 &      365.8 &       17.4 &      583.0 &        5.5 \\
       123 &       53.096447 &    -27.739799 &          6 &      20.10 &       1.01 &      13.10 &       0.66 &      14.10 &       0.82 &      12.20 &       0.77 &      113.5 &       13.1 &      111.0 &        3.3 \\
       124 &       53.150078 &    -27.740025 &          3 &      17.50 &       0.88 &      12.60 &       0.63 &       9.24 &       0.62 &       9.65 &       0.68 &       84.7 &       14.4 &      121.0 &        3.9 \\
       125 &       53.113667 &    -27.741388 &          3 &      31.70 &       1.59 &      25.60 &       1.28 &      18.50 &       1.01 &      85.50 &       4.30 &      121.4 &       25.7 &       93.5 &        3.3 \\
       126 &       53.124393 &    -27.740175 &          4 &     706.00 &       0.16 &     481.00 &       0.16 &     783.00 &       0.80 &    5790.00 &       0.87 &     5290.6 &      308.4 &     7590.0 &      759.0 \\
       127 &       53.166771 &    -27.738613 &          7 &      35.10 &       1.76 &      24.80 &       1.24 &      20.70 &       1.12 &      18.50 &       1.04 &      136.5 &       16.1 &      160.0 &        4.6 \\
       128 &       53.213657 &    -27.741524 &          2 &     122.00 &       6.10 &      85.40 &       4.27 &      69.30 &       3.55 &      42.80 &       2.39 &      108.0 &       18.3 &       58.9 &        4.9 \\
       129 &       53.083759 &    -27.739658 &          7 &      35.10 &       1.76 &      31.10 &       1.56 &      20.20 &       1.10 &      21.80 &       1.20 &      220.9 &       14.8 &      137.0 &        3.7 \\
       130 &       53.107304 &    -27.742008 &          4 &      34.40 &       1.72 &      25.00 &       1.25 &      23.60 &       1.25 &      18.60 &       1.04 &      224.4 &       14.6 &      318.0 &        4.6 \\
       131 &       53.075012 &    -27.742168 &          4 &      16.20 &       0.06 &      16.30 &       0.10 &      13.30 &       0.50 &      14.90 &       0.50 &      205.2 &       15.2 &       62.3 &        4.3 \\
       132 &       53.061562 &    -27.742613 &          7 &      18.70 &       0.94 &      12.20 &       0.61 &      12.50 &       0.76 &       9.98 &       0.70 &      107.6 &       14.2 &      190.0 &        4.5 \\
       133 &       53.079353 &    -27.741722 &          3 &       8.26 &       0.42 &      13.40 &       0.67 &      26.80 &       1.41 &      44.30 &       2.27 &      146.9 &       14.1 &      286.0 &        4.5 \\
       134 &       53.204960 &    -27.743465 &          3 &      37.70 &       1.89 &      30.70 &       1.54 &      20.70 &       1.17 &      70.80 &       3.60 &      121.9 &       28.7 &       91.0 &        2.6 \\
       135 &       53.215889 &    -27.743637 &          2 &     108.00 &       5.40 &     103.00 &       5.16 &     134.00 &       6.76 &     225.00 &      11.31 &      549.7 &       35.5 &     1330.0 &       12.3 \\
       136 &       53.063454 &    -27.743944 &          4 &      18.60 &       0.93 &      17.00 &       0.85 &      13.40 &       0.80 &      14.80 &       0.89 &      148.7 &       13.7 &       96.5 &        4.3 \\
       137 &       53.115009 &    -27.742058 &          3 &      43.10 &       2.16 &      34.50 &       1.73 &      23.60 &       1.25 &     109.00 &       5.47 &      128.1 &       15.7 &       87.8 &        3.2 \\
       138 &       53.110123 &    -27.745552 &          5 &      23.40 &       1.17 &      19.80 &       0.99 &      16.50 &       0.92 &      15.20 &       0.89 &      170.8 &       18.9 &      124.0 &        3.3 \\
       139 &       53.146339 &    -27.744404 &          5 &      14.40 &       0.72 &      10.60 &       0.53 &       8.08 &       0.58 &       8.56 &       0.64 &       85.1 &       13.1 &       21.2 &        4.5 \\
       140 &       53.040691 &    -27.745205 &          2 &     168.00 &       8.40 &     111.00 &       5.55 &     138.00 &       6.91 &     889.00 &      44.45 &      758.2 &       36.3 &     1210.0 &       10.6 \\
       141 &       53.172802 &    -27.744581 &         12 &      43.00 &       2.15 &      41.10 &       2.06 &      29.80 &       1.55 &      26.80 &       1.42 &      140.1 &        9.6 &       86.6 &        3.7 \\
       142 &       53.086308 &    -27.748367 &          6 &      65.50 &       3.28 &      46.80 &       2.34 &      37.00 &       1.90 &      29.90 &       1.57 &      265.1 &       19.8 &      317.0 &        3.6 \\
       143 &       53.083515 &    -27.746515 &          5 &      13.70 &       0.69 &      15.80 &       0.79 &      19.10 &       1.04 &      30.10 &       1.58 &      125.2 &       13.5 &      334.0 &        6.8 \\
       144 &       53.161552 &    -27.747025 &         14 &      55.20 &       2.76 &      36.70 &       1.84 &      33.30 &       1.72 &      29.00 &       1.53 &      144.8 &       10.7 &      283.0 &        5.1 \\
       145 &       53.068676 &    -27.747057 &          4 &      31.30 &       1.57 &      23.30 &       1.17 &      22.00 &       1.18 &      17.80 &       1.01 &      172.5 &       17.0 &      230.0 &        4.2 \\
       146 &       53.172462 &    -27.749447 &         19 &      21.30 &       1.07 &      20.40 &       1.02 &      14.90 &       0.85 &      16.50 &       0.96 &      180.3 &        8.5 &      107.0 &        4.0 \\
       147 &       53.175358 &    -27.749641 &         25 &       9.14 &       0.46 &       6.89 &       0.35 &       4.67 &       0.47 &       4.36 &       0.54 &       38.0 &        6.7 &       27.8 &        3.8 \\
       148 &       53.179985 &    -27.749268 &          9 &      66.90 &       3.35 &      47.10 &       2.36 &      40.90 &       2.09 &      32.20 &       1.68 &      126.2 &       11.5 &      115.0 &        4.0 \\
       149 &       53.036186 &    -27.752308 &          8 &      48.60 &       2.43 &      48.20 &       2.41 &      34.70 &       1.79 &      34.30 &       1.79 &      302.2 &       17.2 &      198.0 &        5.3 \\
       150 &       53.125851 &    -27.751381 &          5 &      25.00 &       1.25 &      21.30 &       1.07 &      25.80 &       1.35 &      30.20 &       1.58 &       85.7 &       20.7 &      165.0 &        4.0 \\
       151 &       53.157196 &    -27.751619 &         12 &      13.90 &       0.70 &      13.80 &       0.69 &      10.90 &       0.68 &      11.20 &       0.74 &      105.3 &        9.6 &       53.6 &        4.2 \\
       152 &       53.024879 &    -27.752111 &          3 &      51.90 &       2.60 &      41.90 &       2.10 &      31.90 &       1.67 &      36.20 &       1.89 &      362.3 &       27.6 &      349.0 &        6.5 \\
       153 &       53.085888 &    -27.752079 &          5 &      24.00 &       1.20 &      21.40 &       1.07 &      14.40 &       0.83 &      39.60 &       2.04 &       86.4 &       17.4 &      103.0 &        4.1 \\
       154 &       53.195179 &    -27.753881 &          3 &      36.40 &       1.82 &      25.00 &       1.25 &      23.60 &       1.24 &      17.60 &       1.01 &      167.7 &       20.2 &      169.0 &        4.2 \\
       155 &       53.217888 &    -27.754059 &          3 &      20.30 &       1.02 &      14.20 &       0.73 &      11.60 &       0.94 &       8.69 &       1.01 &       92.3 &       18.1 &       84.3 &        4.0 \\
       156 &       53.051228 &    -27.753719 &          4 &      24.90 &       1.25 &      16.20 &       0.81 &      16.60 &       0.93 &      12.30 &       0.78 &      100.2 &       15.4 &       88.1 &        3.9 \\
       157 &       53.127357 &    -27.755161 &          5 &      56.80 &       2.84 &      37.70 &       1.89 &      41.20 &       2.10 &      30.00 &       1.57 &      190.9 &       22.0 &      236.0 &        3.4 \\
       158 &       53.125191 &    -27.756657 &          4 &      59.40 &       2.97 &      51.30 &       2.57 &      51.40 &       2.60 &      56.10 &       2.84 &      266.9 &       15.5 &      425.0 &        4.8 \\
       159 &       53.124332 &    -27.755812 &          5 &      64.30 &       3.22 &      45.10 &       2.26 &      37.80 &       1.93 &      29.80 &       1.56 &      147.9 &       15.0 &      188.0 &        5.2 \\
       160 &       53.072842 &    -27.757936 &          4 &      20.60 &       1.03 &      16.40 &       0.82 &      12.20 &       0.74 &      13.50 &       0.83 &      160.4 &       19.8 &      135.0 &        3.2 \\
       161 &       53.204578 &    -27.756859 &          3 &      27.40 &       1.37 &      20.90 &       1.05 &      15.50 &       0.88 &      14.90 &       0.91 &      112.6 &       20.2 &      105.0 &        4.2 \\
       162 &       53.022850 &    -27.757078 &          4 &      31.20 &       1.56 &      29.00 &       1.45 &      20.10 &       1.12 &      24.00 &       1.32 &      238.6 &       19.6 &      194.0 &        5.1 \\
       163 &       53.111885 &    -27.757915 &          3 &      47.40 &       2.37 &      33.10 &       1.66 &      32.80 &       1.69 &      23.70 &       1.27 &      231.6 &       19.4 &      241.0 &        5.0 \\
       164 &       53.163536 &    -27.759041 &         28 &      56.60 &       2.83 &      44.90 &       2.25 &      30.40 &       1.57 &      27.30 &       1.44 &      142.8 &       10.4 &      150.0 &        5.1 \\
       165 &       53.013363 &    -27.758095 &          2 &      43.20 &       2.16 &      32.90 &       1.65 &      31.80 &       1.70 &      36.90 &       1.97 &      165.5 &       31.8 &      190.0 &        4.9 \\
       166 &       53.124870 &    -27.758396 &          4 &      77.80 &       3.89 &      91.10 &       4.56 &     109.00 &       5.47 &     142.00 &       7.12 &      335.8 &       21.8 &      481.0 &        5.1 \\
       167 &       53.183647 &    -27.761621 &         38 &      97.70 &       4.89 &      68.70 &       3.44 &      54.20 &       2.73 &      32.70 &       1.69 &       43.5 &        8.5 &       29.4 &        4.2 \\
       168 &       53.134037 &    -27.759790 &          5 &      71.50 &       3.58 &      51.00 &       2.55 &      43.40 &       2.21 &      33.60 &       1.75 &       79.2 &       12.9 &       68.5 &        4.0 \\
       169 &       53.172905 &    -27.759134 &         45 &      23.70 &       1.19 &      16.70 &       0.84 &      12.60 &       0.73 &      58.70 &       2.97 &       49.3 &        6.5 &       68.5 &        3.9 \\
       170 &       53.060078 &    -27.761385 &          3 &      54.40 &       2.72 &      53.20 &       2.66 &      38.90 &       1.99 &     152.00 &       7.62 &      291.6 &       20.9 &      243.0 &        4.2 \\
       171 &       53.172203 &    -27.760731 &         37 &      15.70 &       0.79 &      17.30 &       0.87 &      13.00 &       0.75 &      15.10 &       0.88 &       80.4 &        7.0 &      122.0 &        4.5 \\
       172 &       53.151489 &    -27.762114 &         26 &      32.90 &       1.65 &      32.50 &       1.63 &      27.80 &       1.44 &      81.60 &       4.11 &      185.6 &        9.1 &      196.0 &        4.4 \\
       173 &       53.137459 &    -27.763092 &         12 &     151.00 &       0.08 &     114.00 &       0.12 &      94.50 &       0.54 &      78.50 &       0.57 &      459.6 &       35.5 &      476.0 &        5.2 \\
       174 &       53.136208 &    -27.763281 &         12 &      90.20 &       4.51 &      64.40 &       3.22 &      52.10 &       2.63 &      37.90 &       1.95 &       61.7 &       13.7 &       40.4 &        4.4 \\
       175 &       53.137230 &    -27.761591 &         10 &      51.10 &       2.56 &      44.30 &       2.22 &      42.70 &       2.17 &      35.40 &       1.83 &       82.9 &       12.0 &        0.0 &        0.0 \\
       176 &       53.028519 &    -27.764011 &          5 &      21.00 &       1.05 &      14.50 &       0.73 &      14.10 &       0.84 &      10.60 &       0.74 &       96.8 &       19.2 &      115.0 &        4.9 \\
       177 &       53.181141 &    -27.765791 &         35 &      23.30 &       1.17 &      19.80 &       0.99 &      13.30 &       0.75 &      13.70 &       0.80 &      116.6 &        7.4 &       98.7 &        3.8 \\
       178 &       53.190071 &    -27.765327 &          8 &      24.90 &       1.25 &      20.70 &       1.04 &      14.30 &       0.79 &      28.20 &       1.47 &       66.3 &       12.2 &       59.7 &        4.2 \\
       179 &       53.050846 &    -27.765192 &          3 &      19.70 &       0.99 &      14.20 &       0.71 &      10.80 &       0.68 &      10.30 &       0.70 &      103.9 &       18.3 &       89.2 &        3.3 \\
       180 &       53.026676 &    -27.765291 &          3 &      34.50 &       1.73 &      36.20 &       1.81 &      27.50 &       1.45 &      26.00 &       1.41 &      199.7 &       25.7 &      128.0 &        4.6 \\
       181 &       53.096436 &    -27.765253 &          3 &      27.30 &       1.37 &      25.20 &       1.26 &      17.40 &       0.96 &      18.60 &       1.05 &      132.6 &       20.5 &      112.0 &        4.2 \\
       182 &       53.076836 &    -27.765600 &          4 &      72.90 &       3.65 &      44.90 &       2.25 &      42.00 &       2.14 &      44.40 &       2.27 &      103.7 &       19.6 &      252.0 &        5.4 \\
       183 &       53.155361 &    -27.766169 &         42 &       9.63 &       0.48 &       7.39 &       0.37 &       4.64 &       0.42 &       4.05 &       0.48 &       33.1 &        6.3 &       40.2 &        5.6 \\
       184 &       53.093060 &    -27.766651 &          3 &      21.00 &       1.05 &      14.00 &       0.70 &      16.10 &       0.90 &      12.80 &       0.80 &       75.9 &       14.6 &       49.7 &        3.5 \\
       185 &       53.142372 &    -27.765114 &         25 &      21.10 &       1.06 &      18.70 &       0.94 &      13.20 &       0.76 &      30.90 &       1.61 &       54.4 &        6.7 &       76.2 &        3.2 \\
       186 &       53.098343 &    -27.767038 &          5 &      34.90 &       1.75 &      30.60 &       1.53 &      23.20 &       1.23 &      22.70 &       1.23 &      198.0 &       18.7 &      157.0 &        3.6 \\
       187 &       53.162804 &    -27.767260 &         49 &      72.20 &       3.61 &      79.90 &       4.00 &      86.80 &       4.35 &     106.00 &       5.32 &      156.7 &        6.5 &      281.0 &        5.0 \\
       188 &       53.151318 &    -27.766775 &         36 &      11.90 &       0.60 &       8.12 &       0.41 &       7.32 &       0.51 &       6.94 &       0.56 &       76.9 &        6.8 &      116.0 &        3.9 \\
       189 &       53.114887 &    -27.767645 &          5 &     100.00 &       5.00 &      64.90 &       3.25 &      64.30 &       3.24 &      45.10 &       2.30 &      224.4 &       20.9 &      269.0 &        4.7 \\
       190 &       53.136700 &    -27.768909 &         28 &      90.10 &       4.51 &      90.60 &       4.53 &      71.60 &       3.60 &     235.00 &      11.76 &      470.1 &       23.5 &      611.0 &        9.6 \\
       191 &       53.116951 &    -27.768438 &          9 &      18.30 &       0.92 &      15.50 &       0.78 &      11.40 &       0.68 &      12.60 &       0.77 &      125.8 &       11.3 &      102.0 &        4.3 \\
       192 &       53.166275 &    -27.768673 &         54 &      13.80 &       0.69 &      12.80 &       0.64 &       9.19 &       0.57 &      11.50 &       0.71 &       56.0 &        6.1 &       26.0 &        3.7 \\
       193 &       53.178326 &    -27.768333 &         44 &      72.50 &       3.63 &      47.00 &       2.35 &      49.70 &       2.51 &      36.20 &       1.85 &      212.1 &        8.3 &      250.0 &        3.8 \\
       194 &       53.093895 &    -27.767820 &          4 &      15.50 &       0.78 &      24.30 &       1.22 &      37.30 &       1.91 &      55.20 &       2.80 &      116.4 &       16.6 &      147.0 &        4.5 \\
       195 &       53.158695 &    -27.770624 &         46 &       9.31 &       0.47 &       6.24 &       0.32 &       4.62 &       0.41 &       3.63 &       0.45 &       36.6 &        5.4 &       30.1 &        3.7 \\
       196 &       53.082428 &    -27.769508 &          4 &      15.10 &       0.76 &      13.70 &       0.69 &      10.00 &       0.65 &      10.50 &       0.72 &       79.4 &       12.2 &       68.8 &        2.8 \\
       197 &       53.165520 &    -27.769909 &         52 &      35.60 &       1.78 &      44.90 &       2.25 &      45.50 &       2.30 &      47.70 &       2.42 &      142.0 &        4.8 &      225.0 &        3.8 \\
       198 &       53.169876 &    -27.771137 &         39 &      57.60 &       2.88 &      37.20 &       1.86 &      36.80 &       1.87 &      27.60 &       1.44 &      136.6 &        6.5 &      148.0 &        4.2 \\
       199 &       53.105888 &    -27.771500 &          6 &      35.30 &       1.77 &      24.80 &       1.24 &      26.70 &       1.39 &      20.90 &       1.14 &      270.4 &       20.2 &      366.0 &        5.0 \\
       200 &       53.127937 &    -27.771509 &         23 &      25.20 &       1.26 &      22.20 &       1.11 &      16.10 &       0.88 &      15.70 &       0.89 &       99.4 &        8.3 &       60.3 &        3.2 \\
       201 &       53.102493 &    -27.772394 &          8 &      35.00 &       1.75 &      31.00 &       1.55 &      22.20 &       1.17 &      19.50 &       1.08 &      121.9 &       13.3 &       90.3 &        3.7 \\
       202 &       53.173946 &    -27.772160 &         50 &      29.90 &       1.50 &      28.30 &       1.42 &      20.80 &       1.09 &      67.70 &       3.41 &      149.2 &        4.4 &      245.0 &        3.8 \\
       203 &       53.050900 &    -27.772482 &          5 &      55.60 &       2.78 &      42.60 &       2.13 &      32.10 &       1.66 &      30.10 &       1.58 &      164.7 &       17.2 &      224.0 &        3.7 \\
       204 &       53.128487 &    -27.772785 &         26 &      36.60 &       1.83 &      26.20 &       1.31 &      19.10 &       1.01 &      13.80 &       0.81 &       51.6 &        8.9 &       65.4 &        3.4 \\
       205 &       53.027309 &    -27.773104 &          3 &      44.40 &       2.22 &      39.10 &       1.96 &      28.50 &       1.50 &      25.30 &       1.37 &      130.9 &       13.5 &       90.1 &        4.6 \\
       206 &       53.048187 &    -27.773113 &          8 &      14.90 &       0.75 &      12.80 &       0.64 &       8.98 &       0.61 &       9.46 &       0.68 &       77.1 &        9.6 &       73.3 &        4.4 \\
       207 &       53.064373 &    -27.775431 &          3 &      29.30 &       1.47 &      27.80 &       1.39 &      32.60 &       1.68 &      32.70 &       1.71 &      109.9 &       22.8 &      197.0 &        5.4 \\
       208 &       53.147900 &    -27.774004 &         41 &      46.50 &       2.33 &      38.00 &       1.90 &      27.60 &       1.42 &      26.20 &       1.37 &      165.5 &        8.0 &      157.0 &        3.7 \\
       209 &       53.176003 &    -27.773808 &         35 &      11.80 &       0.59 &      10.10 &       0.51 &       6.71 &       0.46 &       6.91 &       0.51 &       44.8 &        5.9 &       23.6 &        3.0 \\
       210 &       53.084446 &    -27.772432 &          4 &       8.61 &       0.43 &      10.40 &       0.53 &       8.25 &       0.58 &       7.13 &       0.60 &       71.0 &       14.1 &       69.5 &        3.4 \\
       211 &       53.120720 &    -27.773298 &         17 &      47.90 &       2.40 &      31.10 &       1.56 &      29.10 &       1.49 &      22.70 &       1.21 &      110.8 &       10.9 &      184.0 &        4.6 \\
       212 &       53.218124 &    -27.774078 &          2 &    1750.00 &      87.50 &    1080.00 &      54.00 &     736.00 &      36.80 &     403.00 &      20.16 &      125.4 &       19.8 &       47.8 &        5.8 \\
       213 &       53.149048 &    -27.774414 &         42 &      33.20 &       1.66 &      26.60 &       1.33 &      19.00 &       1.01 &      19.10 &       1.04 &      100.4 &        7.4 &       86.9 &        2.6 \\
       214 &       53.058464 &    -27.776264 &          3 &      20.50 &       1.03 &      15.50 &       0.78 &      17.20 &       0.95 &      13.60 &       0.84 &      113.5 &       22.0 &      250.0 &        3.3 \\
       215 &       53.152702 &    -27.775349 &         46 &      25.20 &       1.26 &      18.70 &       0.94 &      16.20 &       0.88 &      15.80 &       0.88 &      117.4 &        5.7 &       18.1 &        3.7 \\
       216 &       53.151848 &    -27.775513 &         47 &      31.90 &       1.60 &      24.90 &       1.25 &      21.20 &       1.11 &      21.70 &       1.15 &      132.4 &        4.8 &      256.0 &        4.4 \\
       217 &       53.152042 &    -27.774845 &         45 &      20.00 &       1.00 &      13.50 &       0.68 &      13.40 &       0.74 &      11.50 &       0.69 &       50.9 &        6.3 &        6.1 &        4.5 \\
       218 &       53.158394 &    -27.774069 &         45 &       7.86 &       0.39 &       9.55 &       0.48 &      15.50 &       0.84 &      28.50 &       1.48 &       79.2 &        7.4 &       79.2 &        3.3 \\
       219 &       53.162296 &    -27.775162 &         46 &      24.40 &       1.22 &      21.00 &       1.05 &      15.80 &       0.85 &      33.10 &       1.70 &       84.5 &        5.6 &       99.6 &        3.0 \\
       220 &       53.131069 &    -27.773191 &         27 &      29.60 &       1.48 &      35.90 &       1.80 &      52.30 &       2.64 &      71.60 &       3.60 &      154.7 &        7.0 &      350.0 &        5.0 \\
       221 &       53.160511 &    -27.776344 &         41 &       9.17 &       0.46 &       9.33 &       0.47 &      12.20 &       0.69 &      12.90 &       0.75 &       37.6 &        6.5 &      200.0 &        3.3 \\
       222 &       53.160347 &    -27.775570 &         40 &      40.50 &       2.03 &      26.40 &       1.32 &      24.90 &       1.29 &      18.80 &       1.02 &       36.4 &        7.0 &       10.6 &        3.2 \\
       223 &       53.185852 &    -27.775709 &         47 &       8.11 &       0.41 &       7.92 &       0.40 &       5.23 &       0.41 &       5.02 &       0.45 &       42.1 &        6.8 &       34.3 &        3.5 \\
       224 &       53.193047 &    -27.775669 &         24 &       8.13 &       0.41 &       7.55 &       0.38 &       6.57 &       0.46 &      11.70 &       0.69 &       57.7 &        7.2 &       52.6 &        3.7 \\
       225 &       53.180996 &    -27.776278 &         49 &      16.90 &       0.85 &      11.60 &       0.58 &      12.20 &       0.69 &      10.70 &       0.65 &       70.2 &        5.2 &       91.4 &        2.8 \\
       226 &       53.116589 &    -27.777643 &         26 &     145.00 &       7.25 &     136.00 &       6.80 &     101.00 &       5.06 &     435.00 &      21.75 &      726.4 &       14.1 &      882.0 &        6.5 \\
       227 &       53.025253 &    -27.779348 &          3 &      12.20 &       0.61 &       8.98 &       0.46 &       9.87 &       0.71 &       7.49 &       0.69 &      101.8 &       20.0 &       47.8 &        3.5 \\
       228 &       53.133423 &    -27.775909 &         33 &     466.00 &      23.30 &     288.00 &      14.40 &     204.00 &      10.21 &     109.00 &       5.47 &       33.2 &        5.6 &        9.5 &        5.5 \\
       229 &       53.183346 &    -27.776531 &         46 &       8.65 &       0.43 &      11.00 &       0.55 &      15.70 &       0.85 &      21.20 &       1.12 &       42.8 &        5.4 &      126.0 &        4.0 \\
       230 &       53.145191 &    -27.777998 &         46 &      23.90 &       1.20 &      18.90 &       0.95 &      13.70 &       0.76 &      15.50 &       0.87 &      151.4 &        5.2 &      133.0 &        3.0 \\
       231 &       53.110767 &    -27.780296 &          7 &      53.50 &       2.68 &      45.90 &       2.30 &      30.80 &       1.57 &      60.30 &       3.04 &      143.8 &        9.1 &      108.0 &        4.4 \\
       232 &       53.049717 &    -27.779148 &          7 &      28.80 &       1.44 &      26.30 &       1.32 &      19.10 &       1.04 &      18.00 &       1.02 &      146.7 &       12.2 &      102.0 &        2.4 \\
       233 &       53.035538 &    -27.780142 &          4 &     293.00 &      14.65 &     266.00 &      13.30 &     194.00 &       9.71 &     476.00 &      23.81 &      984.4 &       42.0 &     1060.0 &        8.3 \\
       234 &       53.196327 &    -27.779100 &         20 &      17.00 &       0.85 &      15.00 &       0.75 &       8.82 &       0.54 &       7.44 &       0.52 &       48.6 &       10.5 &       22.6 &        4.9 \\
       235 &       53.040581 &    -27.780399 &          4 &      12.50 &       0.63 &       8.77 &       0.44 &       6.97 &       0.54 &       6.44 &       0.59 &       72.3 &       11.1 &       88.5 &        4.9 \\
       236 &       53.128719 &    -27.780466 &         40 &      23.50 &       1.18 &      19.80 &       0.99 &      14.80 &       0.81 &      14.20 &       0.80 &      125.4 &        6.7 &      101.0 &        4.1 \\
       237 &       53.165836 &    -27.781631 &         40 &      11.80 &       0.59 &       9.04 &       0.46 &       6.12 &       0.44 &       5.42 &       0.45 &       46.3 &        5.9 &       35.1 &        3.4 \\
       238 &       53.135193 &    -27.781836 &         37 &       9.02 &       0.45 &       9.41 &       0.47 &       7.59 &       0.49 &       8.04 &       0.55 &       35.2 &        6.8 &       39.8 &        4.2 \\
       239 &       53.172558 &    -27.781063 &         52 &      20.40 &       1.02 &      13.70 &       0.69 &      14.10 &       0.77 &      12.20 &       0.71 &       67.1 &        7.2 &       78.1 &        3.0 \\
       240 &       53.048237 &    -27.783169 &          3 &      20.20 &       1.01 &      13.00 &       0.65 &      13.80 &       0.79 &       7.79 &       0.62 &      108.7 &       19.6 &      104.0 &        3.5 \\
       241 &       53.179054 &    -27.780626 &         34 &      33.70 &       1.69 &      26.90 &       1.35 &      20.40 &       1.07 &      21.20 &       1.12 &      226.2 &        7.2 &      223.0 &        3.6 \\
       242 &       53.087132 &    -27.784933 &          4 &     120.00 &       6.00 &      78.50 &       3.93 &      89.70 &       4.50 &      69.70 &       3.51 &      468.3 &       24.4 &      618.0 &        5.9 \\
       243 &       53.118671 &    -27.782982 &         36 &      16.30 &       0.82 &      19.60 &       0.98 &      26.10 &       1.34 &      23.60 &       1.24 &       39.3 &        8.0 &      221.0 &        5.1 \\
       244 &       53.176521 &    -27.785551 &         49 &      33.40 &       1.67 &      31.60 &       1.58 &      21.40 &       1.12 &      17.70 &       0.96 &       58.5 &        6.5 &       52.1 &        3.3 \\
       245 &       53.160313 &    -27.784096 &         39 &      68.40 &       3.42 &      47.10 &       2.36 &      35.30 &       1.79 &      23.50 &       1.23 &       60.8 &        5.9 &       81.9 &        3.3 \\
       246 &       53.143429 &    -27.783289 &         53 &      23.80 &       1.19 &      28.90 &       1.45 &      25.70 &       1.32 &      25.00 &       1.30 &      201.5 &        6.3 &      119.0 &        4.4 \\
       247 &       53.044037 &    -27.785143 &          3 &      19.20 &       0.96 &      13.60 &       0.68 &      10.60 &       0.66 &      10.60 &       0.72 &      112.4 &       13.7 &      150.0 &        3.9 \\
       248 &       53.157185 &    -27.785349 &         34 &      15.40 &       0.77 &      10.70 &       0.54 &      11.10 &       0.64 &       8.88 &       0.57 &       49.9 &        6.8 &       61.3 &        3.3 \\
       249 &       53.209831 &    -27.785336 &          6 &      38.60 &       1.93 &      31.50 &       1.58 &      29.90 &       1.54 &      42.90 &       2.18 &      142.2 &       20.7 &      198.0 &        6.9 \\
       250 &       53.181660 &    -27.783100 &         49 &      10.10 &       0.51 &      11.40 &       0.57 &       8.91 &       0.54 &       7.96 &       0.54 &       43.0 &        5.7 &       70.5 &        2.6 \\
       251 &       53.070946 &    -27.785965 &          6 &      20.00 &       1.00 &      13.30 &       0.67 &      15.20 &       0.84 &      11.20 &       0.71 &      116.0 &       15.7 &      117.0 &        4.5 \\
       252 &       53.075932 &    -27.785885 &          4 &      24.10 &       1.21 &      26.70 &       1.34 &      21.10 &       1.11 &      23.80 &       1.26 &      196.2 &       18.1 &      114.0 &        3.7 \\
       253 &       53.166119 &    -27.787609 &         36 &      36.10 &       1.81 &      27.40 &       1.37 &      19.50 &       1.02 &      20.90 &       1.11 &      187.4 &        6.8 &      175.0 &        3.6 \\
       254 &       53.139355 &    -27.786860 &         31 &       5.63 &       0.28 &       5.19 &       0.26 &       3.70 &       0.36 &       4.06 &       0.41 &       42.4 &        6.5 &       16.5 &        5.2 \\
       255 &       53.103561 &    -27.785177 &          6 &      38.40 &       1.92 &      36.80 &       1.84 &      26.80 &       1.38 &      81.50 &       4.09 &      235.1 &       14.2 &      225.0 &        4.7 \\
       256 &       53.142067 &    -27.786785 &         36 &      20.20 &       1.01 &      16.70 &       0.84 &      11.60 &       0.66 &      52.70 &       2.66 &       79.2 &        5.7 &       76.7 &        3.8 \\
       257 &       53.047939 &    -27.787022 &          4 &      83.20 &       4.16 &      63.40 &       3.17 &      80.20 &       4.03 &      94.60 &       4.75 &      447.2 &       20.2 &      736.0 &        6.3 \\
       258 &       53.059608 &    -27.787052 &          7 &      42.60 &       2.13 &      29.10 &       1.46 &      29.00 &       1.49 &      22.80 &       1.22 &       98.0 &       14.6 &       97.4 &        4.2 \\
       259 &       53.099628 &    -27.786299 &          7 &      17.30 &       0.87 &      12.50 &       0.63 &      12.70 &       0.71 &      10.10 &       0.64 &       65.9 &       10.2 &       59.5 &        4.8 \\
       260 &       53.086002 &    -27.788111 &          8 &      33.60 &       1.68 &      22.80 &       1.14 &      24.10 &       1.25 &      17.50 &       0.96 &      139.5 &        9.6 &      139.0 &        4.8 \\
       261 &       53.197529 &    -27.786510 &         44 &      15.60 &       0.78 &      13.80 &       0.69 &      10.60 &       0.62 &      11.80 &       0.69 &      142.1 &        6.3 &      102.0 &        4.1 \\
       262 &       53.059288 &    -27.789248 &          9 &      39.80 &       1.99 &      35.90 &       1.80 &      34.50 &       1.76 &      29.70 &       1.54 &       83.8 &       13.3 &      366.0 &        5.5 \\
       263 &       53.045483 &    -27.789579 &          4 &      86.50 &       4.33 &      77.70 &       3.89 &      55.90 &       2.82 &     115.00 &       5.77 &      259.8 &       35.2 &      309.0 &        5.6 \\
       264 &       53.184109 &    -27.791632 &         43 &      15.70 &       0.79 &      15.70 &       0.79 &      13.00 &       0.72 &      15.40 &       0.85 &       33.9 &        5.7 &       73.0 &        6.2 \\
       265 &       53.184738 &    -27.790051 &         49 &       7.02 &       0.35 &       5.12 &       0.26 &       4.36 &       0.38 &       7.14 &       0.50 &       30.7 &        4.8 &       40.5 &        4.2 \\
       266 &       53.187912 &    -27.790083 &         43 &      59.10 &       2.96 &      53.20 &       2.66 &      45.50 &       2.30 &     147.00 &       7.36 &      304.0 &       12.4 &      353.0 &        8.9 \\
       267 &       53.090637 &    -27.790257 &          6 &      13.80 &       0.69 &       9.89 &       0.50 &       7.23 &       0.49 &       8.21 &       0.56 &       93.7 &       15.5 &      104.0 &        3.7 \\
       268 &       53.130589 &    -27.790337 &         32 &      27.60 &       1.38 &      18.80 &       0.94 &      21.70 &       1.13 &      16.90 &       0.92 &      120.1 &        8.9 &      140.0 &        5.7 \\
       269 &       53.153881 &    -27.790852 &         40 &      19.70 &       0.99 &      20.00 &       1.00 &      20.50 &       1.07 &      15.10 &       0.84 &       35.7 &        7.8 &      162.0 &        3.8 \\
       270 &       53.186897 &    -27.791096 &         44 &     184.00 &       9.20 &     151.00 &       7.55 &     112.00 &       5.61 &     587.00 &      29.35 &      758.2 &       14.4 &      941.0 &       12.2 \\
       271 &       53.137608 &    -27.792046 &         35 &      11.90 &       0.60 &       8.04 &       0.41 &       6.85 &       0.46 &       5.65 &       0.45 &       39.4 &        6.3 &       35.3 &        5.1 \\
       272 &       53.178040 &    -27.792839 &         66 &      10.40 &       0.52 &      11.10 &       0.56 &       8.63 &       0.53 &       7.83 &       0.53 &       59.4 &        4.4 &       51.9 &        3.3 \\
       273 &       53.184105 &    -27.792755 &         36 &      22.20 &       1.11 &      15.50 &       0.78 &      17.30 &       0.92 &      20.90 &       1.10 &      105.7 &        6.3 &      245.0 &        7.7 \\
       274 &       53.036068 &    -27.792946 &          3 &     464.00 &      23.20 &     522.00 &      26.10 &     693.00 &      34.65 &     924.00 &      46.20 &     2244.6 &       98.6 &     3570.0 &       20.4 \\
       275 &       53.161518 &    -27.792370 &         41 &      34.20 &       1.71 &      34.70 &       1.74 &      32.60 &       1.66 &      75.20 &       3.78 &      346.4 &        7.6 &      835.0 &        6.6 \\
       276 &       53.187805 &    -27.794128 &         47 &      24.00 &       1.20 &      20.60 &       1.03 &      17.50 &       0.93 &      32.30 &       1.65 &       94.5 &        6.5 &      255.0 &        8.9 \\
       277 &       53.176147 &    -27.796232 &         62 &      39.90 &       2.00 &      28.30 &       1.42 &      22.30 &       1.16 &      22.50 &       1.18 &      233.3 &        5.2 &      269.0 &        2.9 \\
       278 &       53.034115 &    -27.797855 &          3 &      41.00 &       2.05 &      28.00 &       1.40 &      29.60 &       1.53 &      20.60 &       1.13 &      256.3 &       42.2 &      314.0 &        4.9 \\
       279 &       53.119923 &    -27.798849 &          4 &      27.60 &       1.38 &      28.10 &       1.41 &      24.30 &       1.25 &      21.90 &       1.15 &       88.0 &       12.0 &      136.0 &        4.8 \\
       280 &       53.156666 &    -27.795652 &         43 &      24.00 &       1.20 &      20.70 &       1.04 &      16.00 &       0.86 &      15.30 &       0.84 &       65.2 &        6.7 &       85.9 &        3.8 \\
       281 &       53.166859 &    -27.798841 &         49 &      22.60 &       1.13 &      24.40 &       1.22 &      27.00 &       1.39 &      19.50 &       1.04 &       75.7 &        6.5 &      410.0 &        5.3 \\
       282 &       53.124714 &    -27.799286 &         14 &      27.30 &       1.37 &      17.80 &       0.89 &      17.90 &       0.94 &      14.00 &       0.78 &       71.6 &        8.5 &       88.6 &        3.9 \\
       283 &       53.214584 &    -27.799561 &          5 &      50.20 &       2.51 &      32.30 &       1.62 &      29.70 &       1.53 &      26.00 &       1.37 &       82.9 &       11.3 &      102.0 &        3.7 \\
       284 &       53.180180 &    -27.799028 &         82 &      59.00 &       2.95 &      36.90 &       1.85 &      35.90 &       1.82 &      27.10 &       1.40 &      123.2 &        4.4 &      173.0 &        3.1 \\
       285 &       53.039337 &    -27.801939 &          4 &      60.70 &       3.04 &      72.50 &       3.63 &     107.00 &       5.36 &     234.00 &      11.71 &      620.3 &       68.3 &      927.0 &       10.0 \\
       286 &       53.093887 &    -27.804977 &          4 &       5.62 &       0.28 &       4.39 &       0.23 &       4.70 &       0.39 &       5.04 &       0.44 &       86.4 &       15.5 &       71.3 &        9.6 \\
       287 &       53.044655 &    -27.802036 &          6 &      60.60 &       3.03 &      42.80 &       2.14 &      51.30 &       2.59 &      51.70 &       2.62 &      304.0 &       25.0 &      503.0 &        6.5 \\
       288 &       53.073433 &    -27.803352 &          5 &      33.10 &       1.66 &      22.00 &       1.10 &      22.20 &       1.15 &      18.00 &       0.97 &      146.1 &       16.1 &      131.0 &        4.1 \\
       289 &       53.185089 &    -27.805378 &         55 &      53.60 &       2.68 &      46.40 &       2.32 &      35.30 &       1.79 &      71.10 &       3.57 &      176.2 &        5.2 &      229.0 &        3.3 \\
       290 &       53.209576 &    -27.806749 &         11 &      34.00 &       1.70 &      26.30 &       1.32 &      17.60 &       0.94 &      16.70 &       0.93 &       96.0 &        8.3 &       68.1 &        3.8 \\
       291 &       53.130283 &    -27.805696 &         34 &       8.39 &       0.42 &       6.90 &       0.35 &       5.21 &       0.39 &       4.67 &       0.41 &       41.0 &        7.2 &       31.8 &        4.8 \\
       292 &       53.118618 &    -27.807449 &          2 &      23.40 &       1.17 &      16.00 &       0.80 &      18.20 &       0.96 &      15.60 &       0.85 &      113.6 &       22.6 &      180.0 &        5.3 \\
       293 &       53.205730 &    -27.807951 &         16 &     160.00 &       8.00 &     145.00 &       7.25 &     103.00 &       5.16 &     275.00 &      13.76 &      535.6 &       19.1 &      654.0 &        7.4 \\
       294 &       53.206757 &    -27.807564 &         15 &      37.10 &       1.86 &      30.70 &       1.54 &      22.60 &       1.18 &      50.00 &       2.53 &       83.6 &       14.4 &        0.0 &        0.0 \\
       295 &       53.085281 &    -27.808159 &          5 &      28.10 &       1.41 &      21.50 &       1.08 &      14.20 &       0.78 &      14.80 &       0.82 &      133.6 &       14.8 &      128.0 &        3.8 \\
       296 &       53.120045 &    -27.808332 &          4 &      21.00 &       1.05 &      26.00 &       1.30 &      28.60 &       1.46 &      21.50 &       1.13 &      129.2 &       22.0 &      430.0 &        6.1 \\
       297 &       53.210129 &    -27.809290 &         13 &    3480.00 &     174.00 &    1980.00 &      99.00 &    1340.00 &      67.00 &     734.00 &      36.70 &      199.7 &       10.2 &       83.1 &        4.1 \\
       298 &       53.154842 &    -27.809492 &         33 &      11.70 &       0.59 &      13.00 &       0.65 &      13.70 &       0.75 &       9.98 &       0.62 &       33.6 &        5.9 &      194.0 &        4.1 \\
       299 &       53.145042 &    -27.809927 &         47 &      11.20 &       0.56 &      10.30 &       0.52 &       6.82 &       0.46 &       8.05 &       0.53 &       62.8 &        5.6 &       47.3 &        4.0 \\
       300 &       53.164265 &    -27.810898 &         39 &       8.38 &       0.42 &       5.85 &       0.30 &       5.78 &       0.43 &       4.47 &       0.43 &       43.5 &        6.3 &       35.4 &        4.0 \\
       301 &       53.156376 &    -27.810873 &         41 &      25.90 &       1.30 &      17.20 &       0.86 &      18.40 &       0.97 &      14.30 &       0.80 &       98.8 &        6.3 &      118.0 &        4.2 \\
       302 &       53.163105 &    -27.812487 &         50 &     133.00 &       6.65 &      99.30 &       4.97 &      74.50 &       3.74 &      65.10 &       3.28 &      131.5 &        7.4 &      123.0 &        3.5 \\
       303 &       53.134251 &    -27.812704 &         38 &      25.10 &       1.26 &      19.10 &       0.96 &      15.40 &       0.83 &      19.20 &       1.02 &       72.8 &        8.0 &       59.8 &        4.1 \\
       304 &       53.143780 &    -27.813555 &         32 &     125.00 &       6.25 &      97.10 &       4.86 &      64.10 &       3.22 &     222.00 &      11.11 &      289.9 &       14.8 &      275.0 &        4.0 \\
       305 &       53.197456 &    -27.813900 &         18 &       1.99 &       0.11 &       2.68 &       0.15 &       2.56 &       0.36 &       6.73 &       0.52 &       48.3 &       11.8 &       95.5 &        3.3 \\
       306 &       53.102505 &    -27.814396 &          2 &      47.50 &       2.38 &      35.20 &       1.76 &      38.90 &       1.97 &      37.10 &       1.89 &      182.1 &       27.0 &      227.0 &        3.8 \\
       307 &       53.181919 &    -27.814211 &         31 &       2.17 &       0.11 &       2.83 &       0.15 &       4.79 &       0.40 &      15.90 &       0.88 &      145.8 &        6.8 &      280.0 &        4.7 \\
       308 &       53.066730 &    -27.816639 &          3 &      26.70 &       1.34 &      31.00 &       1.55 &      26.10 &       1.34 &      26.10 &       1.35 &      242.2 &       30.0 &      165.0 &        4.1 \\
       309 &       53.165203 &    -27.814177 &         47 &      17.30 &       0.87 &      18.40 &       0.92 &      21.20 &       1.11 &      27.70 &       1.43 &       87.0 &        5.7 &      159.0 &        3.6 \\
       310 &       53.136284 &    -27.816626 &         26 &      18.60 &       0.93 &      12.30 &       0.62 &      13.20 &       0.72 &       9.60 &       0.59 &       46.1 &        9.2 &       53.0 &        3.7 \\
       311 &       53.137142 &    -27.815674 &         35 &      26.00 &       1.30 &      17.70 &       0.89 &      16.90 &       0.90 &      11.40 &       0.67 &       90.5 &        8.9 &       69.4 &        3.5 \\
       312 &       53.191143 &    -27.815504 &         22 &       6.24 &       0.31 &       7.23 &       0.37 &       7.10 &       0.49 &       5.94 &       0.50 &       49.9 &        9.8 &       27.3 &        3.7 \\
       313 &       53.149837 &    -27.814081 &         46 &      24.90 &       1.25 &      23.30 &       1.17 &      16.40 &       0.88 &      16.90 &       0.92 &       65.9 &        5.6 &       88.7 &        4.4 \\
       314 &       53.171120 &    -27.814795 &         36 &      51.10 &       2.56 &      44.80 &       2.24 &      31.50 &       1.61 &      70.70 &       3.56 &      146.5 &       10.4 &      148.0 &        4.8 \\
       315 &       53.044701 &    -27.816536 &          2 &      20.30 &       1.02 &      21.00 &       1.05 &      16.30 &       0.88 &      16.80 &       0.92 &      116.3 &       20.7 &       74.8 &        4.8 \\
       316 &       53.199871 &    -27.815573 &          6 &      21.20 &       1.06 &      18.80 &       0.94 &      12.30 &       0.70 &      66.20 &       3.34 &      104.6 &       13.5 &      172.0 &        3.2 \\
       317 &       53.180988 &    -27.817242 &         22 &      15.10 &       0.76 &      17.80 &       0.89 &      18.10 &       0.96 &      15.00 &       0.85 &       55.3 &        9.2 &      284.0 &        4.6 \\
       318 &       53.161682 &    -27.819332 &         39 &      10.60 &       0.53 &       7.58 &       0.38 &       7.63 &       0.50 &       5.83 &       0.49 &       33.9 &        7.4 &       31.1 &        3.8 \\
       319 &       53.184769 &    -27.819843 &         14 &      13.30 &       0.67 &      15.80 &       0.79 &      18.50 &       0.99 &      14.10 &       0.82 &       60.4 &       10.0 &      238.0 &        3.8 \\
       320 &       53.120728 &    -27.819048 &          6 &      95.60 &       4.78 &      73.40 &       3.67 &      50.60 &       2.55 &      45.10 &       2.28 &      286.4 &       16.3 &      278.0 &        4.0 \\
       321 &       53.180092 &    -27.820694 &         14 &      21.20 &       1.06 &      25.60 &       1.28 &      31.60 &       1.62 &      32.10 &       1.66 &       70.8 &        9.1 &      149.0 &        3.5 \\
       322 &       53.148785 &    -27.821192 &         42 &      17.00 &       0.85 &      21.30 &       1.07 &      31.30 &       1.60 &      45.90 &       2.33 &      196.2 &        6.5 &      581.0 &        7.1 \\
       323 &       53.077850 &    -27.822239 &          2 &      41.70 &       2.09 &      34.90 &       1.75 &      26.30 &       1.35 &      27.50 &       1.42 &      259.8 &       31.8 &      248.0 &        4.0 \\
       324 &       53.071045 &    -27.822750 &          2 &     124.00 &       6.20 &      99.90 &       5.00 &      70.90 &       3.56 &      92.20 &       4.62 &      164.9 &       22.6 &      197.0 &        3.8 \\
       325 &       53.216476 &    -27.821722 &          5 &      17.40 &       0.87 &      19.10 &       0.96 &      15.80 &       0.89 &      13.30 &       0.82 &       98.0 &       17.9 &       46.9 &        4.5 \\
       326 &       53.160213 &    -27.825615 &         25 &      10.40 &       0.52 &       6.77 &       0.34 &       6.48 &       0.47 &       5.04 &       0.48 &       38.2 &        6.3 &        8.6 &        4.1 \\
       327 &       53.202129 &    -27.826385 &          6 &      40.50 &       2.03 &      36.90 &       1.85 &      29.10 &       1.51 &      28.50 &       1.50 &      201.5 &       15.9 &      152.0 &        4.5 \\
       328 &       53.150738 &    -27.825613 &         27 &     107.00 &       5.35 &      85.50 &       4.28 &      89.50 &       4.49 &     120.00 &       6.01 &      532.0 &       13.5 &      744.0 &        6.9 \\
       329 &       53.093620 &    -27.826433 &          6 &      91.90 &       4.60 &      64.20 &       3.21 &      66.30 &       3.33 &      57.70 &       2.91 &      362.3 &       37.7 &      504.0 &        6.3 \\
       330 &       53.189808 &    -27.826805 &          3 &      38.30 &       1.92 &      30.20 &       1.51 &      38.50 &       1.96 &      53.20 &       2.70 &      240.4 &       19.1 &      544.0 &        5.7 \\
       331 &       53.098522 &    -27.827232 &          7 &      44.60 &       2.23 &      34.40 &       1.72 &      42.70 &       2.16 &      46.20 &       2.34 &      251.0 &       15.4 &      323.0 &        4.8 \\
       332 &       53.067318 &    -27.828306 &          2 &     128.00 &       6.40 &      81.70 &       4.09 &      81.20 &       4.07 &      67.40 &       3.39 &      123.2 &       22.0 &      315.0 &        4.6 \\
       333 &       53.148319 &    -27.828928 &         24 &      23.30 &       1.17 &      18.40 &       0.92 &      17.40 &       0.93 &      19.30 &       1.05 &       88.6 &        5.9 &      109.0 &        4.2 \\
       334 &       53.131023 &    -27.829384 &          4 &     104.00 &       5.20 &      88.10 &       4.41 &      68.90 &       3.46 &     282.00 &      14.11 &      387.1 &       37.4 &      466.0 &        5.8 \\
       335 &       53.202827 &    -27.829626 &          7 &      12.00 &       0.60 &      10.50 &       0.53 &       6.96 &       0.53 &       6.09 &       0.56 &       70.0 &       15.0 &       41.4 &        3.7 \\
       336 &       53.161697 &    -27.832382 &         11 &     106.00 &       5.30 &     104.00 &       5.20 &      76.70 &       3.85 &     403.00 &      20.16 &      623.9 &       17.4 &      543.0 &        4.6 \\
       337 &       53.176289 &    -27.830729 &          3 &      43.00 &       2.15 &      35.30 &       1.77 &      28.40 &       1.47 &      47.80 &       2.43 &      135.0 &       19.8 &      215.0 &        4.5 \\
       338 &       53.215469 &    -27.830948 &          4 &      35.10 &       1.76 &      24.00 &       1.20 &      29.60 &       1.54 &      23.10 &       1.26 &      233.3 &       19.6 &      303.0 &        5.2 \\
       339 &       53.075096 &    -27.831469 &          2 &     135.00 &       6.75 &      84.50 &       4.23 &      82.90 &       4.16 &      58.20 &       2.93 &      268.6 &       23.5 &      394.0 &        4.8 \\
       340 &       53.093922 &    -27.830564 &          5 &      45.90 &       2.30 &      29.40 &       1.47 &      27.40 &       1.41 &      19.60 &       1.05 &       83.6 &       14.8 &       94.4 &        4.0 \\
       341 &       53.109295 &    -27.834942 &          5 &      18.90 &       0.95 &      16.10 &       0.81 &      12.80 &       0.72 &      12.70 &       0.75 &       81.3 &       10.7 &       68.1 &        3.6 \\
       342 &       53.157188 &    -27.833555 &         11 &      34.10 &       1.71 &      39.90 &       2.00 &      36.70 &       1.87 &      31.40 &       1.63 &      115.8 &       11.1 &      251.0 &        5.2 \\
       343 &       53.218075 &    -27.833805 &          4 &      25.20 &       1.26 &      17.60 &       0.88 &      18.80 &       1.03 &      13.50 &       0.84 &      203.2 &       15.0 &      220.0 &        5.1 \\
       344 &       53.072670 &    -27.834238 &          3 &      33.40 &       1.67 &      39.60 &       1.98 &      34.30 &       1.74 &      29.50 &       1.52 &      151.8 &       20.4 &      341.0 &        4.2 \\
       345 &       53.152092 &    -27.835184 &         12 &      21.60 &       1.08 &      15.20 &       0.76 &      14.40 &       0.81 &      11.30 &       0.72 &       66.9 &       11.1 &       76.4 &        3.3 \\
       346 &       53.132477 &    -27.832985 &          4 &      30.80 &       1.54 &      22.40 &       1.12 &      18.50 &       0.98 &      18.20 &       0.99 &      194.4 &       17.2 &      250.0 &        4.3 \\
       347 &       53.062359 &    -27.834875 &          3 &      43.80 &       2.19 &      29.00 &       1.45 &      31.70 &       1.62 &      24.40 &       1.28 &      174.1 &       32.7 &      212.0 &        3.5 \\
       348 &       53.155346 &    -27.835890 &          6 &      13.10 &       0.66 &      11.30 &       0.57 &       8.75 &       0.57 &       9.16 &       0.64 &       88.8 &       13.9 &       61.7 &        4.5 \\
       349 &       53.214886 &    -27.838348 &          4 &      27.70 &       1.39 &      19.30 &       0.97 &      21.20 &       1.14 &      16.10 &       0.94 &      201.5 &       24.8 &      242.0 &        3.7 \\
       350 &       53.107727 &    -27.838873 &          6 &      30.10 &       1.51 &      22.90 &       1.15 &      16.10 &       0.88 &      19.10 &       1.04 &      212.1 &       18.3 &      171.0 &        3.7 \\
       351 &       53.081974 &    -27.839922 &          6 &      47.00 &       2.35 &      34.10 &       1.71 &      34.70 &       1.77 &      34.70 &       1.78 &      153.2 &       20.2 &      159.0 &        3.7 \\
       352 &       53.176758 &    -27.840427 &          5 &      76.20 &       3.81 &      53.10 &       2.66 &      54.50 &       2.76 &      46.10 &       2.35 &      208.5 &       17.4 &      254.0 &        6.5 \\
       353 &       53.131374 &    -27.841379 &          8 &      41.40 &       2.07 &      50.00 &       2.50 &      43.90 &       2.22 &      32.50 &       1.68 &       87.3 &       14.8 &      184.0 &        3.7 \\
       354 &       53.141762 &    -27.841419 &          4 &      23.90 &       1.20 &      26.60 &       1.33 &      20.40 &       1.08 &      22.10 &       1.19 &      187.4 &       22.4 &      120.0 &        4.2 \\
       355 &       53.137447 &    -27.841770 &          3 &      84.50 &       4.23 &      56.70 &       2.84 &      61.40 &       3.09 &      49.70 &       2.52 &      323.4 &       22.8 &      392.0 &        4.7 \\
       356 &       53.198788 &    -27.843992 &          4 &      41.30 &       2.07 &      49.80 &       2.49 &      44.20 &       2.25 &      35.60 &       1.84 &      144.6 &       20.2 &      289.0 &        4.3 \\
       357 &       53.115459 &    -27.844723 &          3 &      68.90 &       3.45 &      57.00 &       2.85 &      44.90 &       2.28 &      57.30 &       2.90 &      395.9 &       36.6 &      636.0 &        4.2 \\
       358 &       53.161846 &    -27.845901 &          4 &      59.30 &       2.97 &      43.50 &       2.18 &      31.30 &       1.62 &      25.70 &       1.37 &      145.1 &       16.3 &      149.0 &        5.0 \\
       359 &       53.104961 &    -27.850084 &          6 &       8.89 &       0.45 &       5.86 &       0.30 &       4.82 &       0.46 &       3.72 &       0.51 &       73.5 &       14.4 &       60.5 &        4.1 \\
       360 &       53.239647 &    -27.851028 &          2 &     184.00 &       9.20 &     127.00 &       6.35 &      84.40 &       4.26 &     112.00 &       5.64 &      117.5 &       21.3 &       93.5 &        3.8 \\
       361 &       53.074421 &    -27.849838 &          3 &     324.00 &       0.10 &     242.00 &       0.11 &     231.00 &       0.54 &    1370.00 &       0.58 &     1182.0 &       69.4 &     1270.0 &      127.0 \\
       362 &       53.217972 &    -27.847853 &          4 &      32.90 &       1.65 &      25.30 &       1.27 &      22.30 &       1.19 &      29.40 &       1.55 &      118.4 &       18.7 &      120.0 &        3.8 \\
       363 &       53.070736 &    -27.850708 &          4 &      11.70 &       0.59 &       9.39 &       0.47 &       8.78 &       0.57 &      13.40 &       0.80 &       91.2 &       22.4 &      161.0 &        3.4 \\
       364 &       53.196507 &    -27.851795 &          4 &      61.40 &       3.07 &      54.70 &       2.74 &      37.10 &       1.90 &      35.20 &       1.82 &      219.1 &       17.4 &      172.0 &        4.4 \\
       365 &       53.231213 &    -27.851894 &          3 &    1460.00 &      73.00 &     934.00 &      46.70 &     644.00 &      32.20 &     352.00 &      17.61 &      101.5 &       15.7 &       40.5 &        4.2 \\
       366 &       53.122517 &    -27.852787 &          4 &      40.70 &       2.04 &      26.60 &       1.33 &      24.40 &       1.28 &      17.40 &       0.99 &      121.4 &       21.5 &      107.0 &        5.0 \\
       367 &       53.071991 &    -27.853678 &          5 &      30.50 &       1.53 &      27.30 &       1.37 &      17.90 &       0.97 &      16.30 &       0.94 &      129.1 &       14.2 &       81.4 &        3.2 \\
       368 &       53.220211 &    -27.854191 &          4 &      74.50 &       3.73 &      53.90 &       2.70 &      42.70 &       2.18 &      37.50 &       1.94 &      335.8 &       21.3 &      346.0 &        4.3 \\
       369 &       53.109127 &    -27.852970 &          4 &      62.90 &       3.15 &      42.70 &       2.14 &      46.40 &       2.36 &      34.40 &       1.78 &      226.2 &       15.7 &      282.0 &        5.1 \\
       370 &       53.149815 &    -27.855150 &          2 &      41.00 &       2.05 &      39.00 &       1.95 &      28.70 &       1.49 &      77.60 &       3.91 &      129.9 &       21.8 &      209.0 &        5.0 \\
       371 &       53.220284 &    -27.855621 &          4 &      47.30 &       2.37 &      43.90 &       2.20 &      41.80 &       2.14 &      46.90 &       2.40 &      116.6 &       28.9 &      140.0 &        3.7 \\
       372 &       53.163994 &    -27.854404 &          7 &      13.90 &       0.70 &      12.90 &       0.65 &       9.24 &       0.62 &      10.10 &       0.69 &       68.9 &       13.1 &       63.9 &        3.7 \\
       373 &       53.137791 &    -27.856701 &          5 &      43.70 &       2.19 &      26.90 &       1.35 &      24.10 &       1.27 &      14.60 &       0.86 &       79.6 &       17.8 &       64.0 &        5.0 \\
       374 &       53.095139 &    -27.856842 &          3 &      17.10 &       0.86 &      11.70 &       0.59 &       9.08 &       0.61 &       7.41 &       0.60 &       82.5 &       16.5 &       72.2 &        4.1 \\
       375 &       53.155075 &    -27.857798 &          4 &     102.00 &       5.10 &      83.00 &       4.15 &      71.70 &       3.61 &      88.20 &       4.43 &      399.4 &       25.3 &      467.0 &        4.8 \\
       376 &       53.077911 &    -27.858221 &          4 &      55.10 &       2.76 &      36.40 &       1.82 &      36.80 &       1.88 &      27.70 &       1.47 &      108.2 &       19.4 &      143.0 &        3.8 \\
       377 &       53.221855 &    -27.859503 &          4 &      35.50 &       1.78 &      21.80 &       1.09 &      22.20 &       1.20 &      14.40 &       0.88 &      139.8 &       16.3 &      104.0 &        4.8 \\
       378 &       53.245789 &    -27.861210 &          2 &      25.50 &       1.28 &      29.60 &       1.48 &      27.60 &       1.55 &      26.70 &       1.55 &      132.2 &       19.4 &      152.0 &        5.4 \\
       379 &       53.184414 &    -27.861475 &          4 &     186.00 &       9.30 &     215.00 &      10.75 &     262.00 &      13.11 &     698.00 &      34.90 &     2421.4 &       83.4 &     7260.0 &      726.0 \\
       380 &       53.183468 &    -27.862181 &          5 &     282.00 &      14.10 &     260.00 &      13.00 &     187.00 &       9.36 &     624.00 &      31.20 &      650.4 &       59.9 &        0.0 &        0.0 \\
       381 &       53.086327 &    -27.861851 &          5 &      60.90 &       3.05 &      41.90 &       2.10 &      47.80 &       2.43 &      36.00 &       1.86 &      275.7 &       18.5 &      358.0 &        4.0 \\
       382 &       53.121750 &    -27.862642 &          4 &       8.48 &       0.43 &       5.77 &       0.30 &       4.81 &       0.47 &       4.07 &       0.50 &       70.7 &       13.5 &       46.8 &        4.0 \\
       383 &       53.106041 &    -27.865231 &          5 &      44.80 &       2.24 &      29.80 &       1.49 &      32.00 &       1.65 &      22.10 &       1.20 &      129.5 &       17.0 &      171.0 &        4.4 \\
       384 &       53.165432 &    -27.865261 &          5 &      19.90 &       1.00 &      17.70 &       0.89 &      12.60 &       0.76 &      29.70 &       1.56 &      109.4 &       17.4 &      127.0 &        5.5 \\
       385 &       53.152489 &    -27.864750 &          5 &      30.10 &       1.51 &      28.80 &       1.44 &      20.40 &       1.10 &      58.20 &       2.95 &      132.2 &       14.1 &      132.0 &        3.6 \\
       386 &       53.088879 &    -27.868126 &          5 &      24.40 &       1.22 &      19.10 &       0.96 &      14.40 &       0.83 &      13.50 &       0.82 &      108.5 &       17.2 &       94.5 &        3.5 \\
       387 &       53.177967 &    -27.866537 &          5 &      19.30 &       0.97 &      15.70 &       0.79 &      11.10 &       0.70 &      12.10 &       0.78 &      104.3 &       12.6 &       84.4 &        2.8 \\
       388 &       53.221874 &    -27.868305 &          5 &      13.90 &       0.70 &      12.40 &       0.62 &       9.17 &       0.64 &       9.07 &       0.68 &       82.2 &       14.8 &        2.6 &        3.5 \\
       389 &       53.187519 &    -27.868914 &          3 &      25.00 &       1.25 &      15.90 &       0.80 &      14.60 &       0.85 &       9.71 &       0.69 &       95.1 &       14.6 &       85.6 &        2.8 \\
       390 &       53.150826 &    -27.868389 &          4 &      71.70 &       3.59 &      44.90 &       2.25 &      38.60 &       1.97 &      25.00 &       1.33 &      125.4 &       19.1 &       88.7 &        3.6 \\
       391 &       53.206512 &    -27.867624 &          4 &      32.10 &       1.61 &      28.80 &       1.44 &      22.40 &       1.20 &      53.90 &       2.74 &      166.1 &       14.4 &      156.0 &        3.9 \\
       392 &       53.171238 &    -27.871046 &          8 &      25.70 &       1.29 &      18.90 &       0.95 &      15.90 &       0.90 &      18.10 &       1.03 &       69.5 &       12.6 &       54.5 &        2.6 \\
       393 &       53.157288 &    -27.870144 &          5 &      56.90 &       2.85 &      87.70 &       4.39 &     145.00 &       7.26 &     263.00 &      13.16 &      646.9 &       17.2 &     1080.0 &        6.6 \\
       394 &       53.191238 &    -27.872198 &          4 &      23.10 &       1.16 &      18.10 &       0.91 &      18.40 &       1.02 &      18.00 &       1.03 &      199.7 &       16.5 &      224.0 &        3.2 \\
       395 &       53.071529 &    -27.872450 &          3 &      65.30 &       3.27 &      59.20 &       2.96 &      50.90 &       2.58 &      64.90 &       3.28 &      321.6 &       21.6 &      288.0 &        5.9 \\
       396 &       53.107288 &    -27.872313 &          5 &      21.50 &       1.08 &      16.80 &       0.84 &      11.50 &       0.71 &      10.30 &       0.70 &       96.8 &       19.8 &       94.2 &        3.7 \\
       397 &       53.084389 &    -27.872812 &          4 &      84.50 &       4.23 &      93.20 &       4.66 &      68.60 &       3.46 &     301.00 &      15.06 &      692.9 &       34.4 &      819.0 &        6.4 \\
       398 &       53.163067 &    -27.873096 &          4 &      56.70 &       2.84 &      38.30 &       1.92 &      39.50 &       2.02 &      30.00 &       1.57 &      236.9 &       21.5 &      288.0 &        5.3 \\
       399 &       53.076103 &    -27.873589 &          5 &      21.20 &       1.06 &      17.20 &       0.86 &      22.60 &       1.21 &      22.60 &       1.22 &      164.3 &       17.8 &      199.0 &        4.2 \\
       400 &       53.139290 &    -27.874521 &          4 &       3.90 &       0.20 &       5.87 &       0.30 &       6.35 &       0.52 &      12.60 &       0.78 &       97.6 &       18.3 &      351.0 &        6.1 \\
       401 &       53.094097 &    -27.875595 &          6 &      26.10 &       1.31 &      16.70 &       0.84 &      16.90 &       0.94 &      12.30 &       0.78 &      131.7 &       15.9 &      121.0 &        3.4 \\
       402 &       53.073364 &    -27.874601 &          4 &      86.80 &       4.34 &      69.00 &       3.45 &      45.10 &       2.29 &      40.30 &       2.07 &      266.9 &       20.2 &      251.0 &        4.3 \\
       403 &       53.117245 &    -27.876287 &          4 &      23.40 &       1.17 &      20.90 &       1.05 &      15.70 &       0.89 &      23.80 &       1.28 &      173.5 &       20.2 &      114.0 &        2.7 \\
       404 &       53.155022 &    -27.876791 &          5 &      44.60 &       2.23 &      40.50 &       2.03 &      28.30 &       1.48 &      80.70 &       4.06 &      174.1 &       17.0 &      197.0 &        3.7 \\
       405 &       53.126308 &    -27.877171 &          3 &      61.20 &       3.06 &      38.70 &       1.94 &      36.20 &       1.86 &      22.90 &       1.24 &      105.3 &       23.1 &       92.1 &        3.2 \\
       406 &       53.069233 &    -27.878778 &          2 &      23.40 &       1.17 &      18.60 &       0.93 &      15.80 &       0.90 &      16.20 &       0.94 &      115.0 &       21.6 &       62.9 &        3.9 \\
       407 &       53.096519 &    -27.879478 &          6 &      29.50 &       1.48 &      23.80 &       1.19 &      17.10 &       0.95 &      15.10 &       0.89 &      125.6 &       20.5 &      108.0 &        3.8 \\
       408 &       53.173176 &    -27.880173 &          7 &      39.30 &       1.97 &      37.50 &       1.88 &      28.70 &       1.50 &      90.10 &       4.53 &      208.5 &       18.9 &      152.0 &        4.2 \\
       409 &       53.100224 &    -27.882589 &          8 &      22.40 &       1.12 &      18.50 &       0.93 &      14.80 &       0.86 &      12.80 &       0.80 &      124.8 &       17.8 &       95.2 &        3.4 \\
       410 &       53.136570 &    -27.878857 &          4 &      24.50 &       1.23 &      18.30 &       0.92 &      17.60 &       0.98 &      16.90 &       0.97 &       83.8 &       14.8 &       97.4 &        3.2 \\
       411 &       53.139751 &    -27.880682 &          4 &      47.00 &       2.35 &      36.50 &       1.83 &      25.40 &       1.34 &      24.50 &       1.31 &      127.9 &       25.3 &      168.0 &        3.5 \\
       412 &       53.208973 &    -27.881218 &          4 &      16.80 &       0.84 &      13.80 &       0.69 &      15.90 &       0.91 &      30.40 &       1.60 &       91.7 &       21.1 &      191.0 &        3.5 \\
       413 &       53.127441 &    -27.881704 &          4 &      15.10 &       0.76 &      11.00 &       0.55 &       8.59 &       0.61 &       7.19 &       0.60 &       96.3 &       18.7 &       70.2 &        3.4 \\
       414 &       53.200699 &    -27.882498 &          6 &     143.00 &       7.15 &      86.60 &       4.33 &      77.20 &       3.89 &      49.20 &       2.51 &      101.1 &       21.3 &      162.0 &        3.7 \\
       415 &       53.126743 &    -27.884489 &          7 &      30.90 &       1.55 &      23.20 &       1.16 &      30.70 &       1.60 &      31.90 &       1.67 &      187.4 &       12.8 &      142.0 &        6.4 \\
       416 &       53.125599 &    -27.885077 &         10 &      23.50 &       1.18 &      17.40 &       0.87 &      25.40 &       1.34 &      52.90 &       2.69 &      122.8 &       11.3 &      469.0 &        8.2 \\
       417 &       53.076038 &    -27.886080 &          4 &      11.20 &       0.56 &       8.48 &       0.43 &       4.96 &       0.50 &       6.00 &       0.57 &       98.2 &       24.4 &       39.0 &        4.0 \\
       418 &       53.128780 &    -27.886560 &          4 &      28.00 &       1.40 &      18.90 &       0.95 &      20.80 &       1.13 &      18.70 &       1.06 &      131.3 &       19.4 &      220.0 &        3.5 \\
       419 &       53.127033 &    -27.886770 &          9 &      14.00 &       0.70 &      10.10 &       0.51 &       7.85 &       0.59 &       6.92 &       0.60 &       90.6 &       14.2 &       69.9 &        4.3 \\
       420 &       53.213139 &    -27.885794 &          3 &      22.40 &       1.12 &      16.00 &       0.80 &      12.70 &       0.77 &      11.20 &       0.75 &      105.5 &       16.3 &      138.0 &        4.8 \\
       421 &       53.236019 &    -27.888025 &          3 &      34.10 &       1.71 &      33.40 &       1.67 &      28.20 &       1.49 &      63.30 &       3.21 &      249.2 &       14.8 &      700.0 &        9.4 \\
       422 &       53.144138 &    -27.890188 &          4 &      27.20 &       1.36 &      21.90 &       1.10 &      17.40 &       0.97 &      21.70 &       1.18 &      228.0 &       18.9 &      206.0 &        4.2 \\
       423 &       53.110386 &    -27.888296 &          4 &      24.10 &       1.21 &      17.70 &       0.89 &      12.50 &       0.76 &      13.10 &       0.82 &      123.2 &       20.0 &      116.0 &        3.8 \\
       424 &       53.098644 &    -27.890095 &          6 &      70.00 &       3.50 &      56.60 &       2.83 &      63.30 &       3.20 &      79.60 &       4.01 &      178.6 &       17.4 &      449.0 &        8.3 \\
       425 &       53.163452 &    -27.890537 &          4 &      13.50 &       0.68 &      16.80 &       0.84 &      27.20 &       1.42 &      51.20 &       2.61 &      213.8 &       15.5 &      503.0 &        4.9 \\
       426 &       53.192913 &    -27.890911 &          3 &      32.90 &       1.65 &      39.70 &       1.99 &      36.10 &       1.86 &      37.60 &       1.95 &      365.8 &       22.4 &      187.0 &        3.8 \\
       427 &       53.232746 &    -27.891195 &          3 &      38.00 &       1.90 &      27.00 &       1.35 &      22.60 &       1.22 &      18.60 &       1.06 &      183.8 &       20.7 &      197.0 &        3.7 \\
       428 &       53.104950 &    -27.893105 &          7 &      95.90 &       4.80 &      68.70 &       3.44 &      50.90 &       2.58 &      38.00 &       1.96 &      183.8 &       13.7 &      195.0 &        3.0 \\
       429 &       53.103489 &    -27.893457 &          8 &      21.60 &       1.08 &      14.70 &       0.74 &      16.70 &       0.94 &      13.60 &       0.84 &       86.8 &       12.9 &       80.4 &        3.6 \\
       430 &       53.135033 &    -27.895205 &          3 &      24.00 &       1.20 &      18.70 &       0.94 &      14.20 &       0.83 &      13.20 &       0.82 &      141.0 &       19.4 &       86.4 &        3.3 \\
       431 &       53.106632 &    -27.895332 &          7 &      27.30 &       1.37 &      22.40 &       1.12 &      13.60 &       0.81 &      13.10 &       0.82 &       94.9 &       15.4 &       71.5 &        3.7 \\
       432 &       53.169968 &    -27.895487 &          5 &      19.10 &       0.96 &      13.30 &       0.67 &      11.40 &       0.71 &      11.40 &       0.75 &      114.4 &       13.1 &      152.0 &        3.7 \\
       433 &       53.205559 &    -27.896173 &          6 &      25.50 &       1.28 &      21.70 &       1.09 &      15.50 &       0.89 &      34.70 &       1.81 &      120.0 &       15.7 &      103.0 &        4.2 \\
       434 &       53.163212 &    -27.899431 &          6 &      33.30 &       1.67 &      23.10 &       1.16 &      23.40 &       1.24 &      31.30 &       1.64 &       81.5 &       10.4 &      263.0 &        3.9 \\
       435 &       53.224487 &    -27.898415 &          3 &      98.20 &       4.91 &      68.70 &       3.44 &      51.40 &       2.61 &     220.00 &      11.01 &      190.9 &       17.2 &      205.0 &        3.9 \\
       436 &       53.080219 &    -27.900522 &          2 &      74.60 &       3.73 &      55.60 &       2.78 &      44.70 &       2.28 &      41.70 &       2.14 &      198.0 &       39.4 &      266.0 &        4.3 \\
       437 &       53.102844 &    -27.900087 &          3 &    3870.00 &    4674.01 &    2560.00 &     128.00 &    1720.00 &      86.00 &     954.00 &      47.70 &      272.1 &       23.1 &      114.0 &        4.4 \\
       438 &       53.141792 &    -27.901947 &          3 &      21.10 &       1.06 &      14.00 &       0.70 &      14.10 &       0.82 &       9.73 &       0.69 &      109.9 &       16.6 &       79.2 &        3.2 \\
       439 &       53.233002 &    -27.899256 &          3 &      38.00 &       1.90 &      26.40 &       1.32 &      32.20 &       1.67 &      26.40 &       1.42 &      153.6 &       16.3 &      228.0 &        5.5 \\
       440 &       53.227802 &    -27.900484 &          3 &    2220.00 &     111.00 &    1450.00 &      72.50 &    1040.00 &      52.00 &     547.00 &      27.36 &      180.3 &       18.9 &       65.2 &        3.6 \\
       441 &       53.165161 &    -27.901825 &          4 &      16.10 &       0.81 &      14.60 &       0.73 &      10.90 &       0.69 &      10.60 &       0.72 &       90.3 &       16.1 &       43.2 &        3.5 \\
       442 &       53.143387 &    -27.901604 &          4 &      35.40 &       1.77 &      28.30 &       1.42 &      20.40 &       1.10 &      22.60 &       1.23 &      224.4 &       19.4 &      192.0 &        3.9 \\
       443 &       53.123165 &    -27.901396 &          4 &      13.40 &       0.67 &       9.89 &       0.50 &      10.90 &       0.70 &       8.02 &       0.64 &      104.6 &       12.9 &       77.9 &        4.0 \\
       444 &       53.164112 &    -27.903320 &          8 &      69.70 &       3.49 &      65.40 &       3.27 &      48.40 &       2.46 &      37.40 &       1.93 &      140.1 &       11.5 &       91.8 &        4.1 \\
       445 &       53.145412 &    -27.903904 &          5 &      43.30 &       2.17 &      39.80 &       1.99 &      26.20 &       1.38 &      93.90 &       4.72 &      194.4 &       17.9 &      191.0 &        3.9 \\
       446 &       53.201904 &    -27.904524 &          3 &      47.30 &       2.37 &      31.30 &       1.57 &      30.20 &       1.57 &      20.50 &       1.14 &      170.4 &       25.7 &      209.0 &        4.0 \\
       447 &       53.193310 &    -27.903959 &          6 &     225.00 &      11.25 &     139.00 &       6.95 &     130.00 &       6.52 &      81.10 &       4.09 &      231.6 &       14.4 &      311.0 &        4.4 \\
       448 &       53.136436 &    -27.906446 &          4 &     122.00 &       6.10 &      92.50 &       4.63 &      73.70 &       3.71 &     291.00 &      14.56 &      459.5 &       20.2 &      530.0 &        5.1 \\
       449 &       53.094318 &    -27.906549 &          5 &      46.20 &       2.31 &      36.00 &       1.80 &      25.90 &       1.37 &     122.00 &       6.12 &      147.7 &       15.2 &      214.0 &        3.9 \\
       450 &       53.096375 &    -27.907228 &          5 &      33.70 &       1.69 &      32.60 &       1.63 &      22.90 &       1.23 &      63.20 &       3.20 &      167.6 &       14.2 &      171.0 &        4.3 \\
       451 &       53.113930 &    -27.905968 &          6 &      18.90 &       0.95 &      13.50 &       0.68 &      15.00 &       0.87 &      12.50 &       0.80 &       93.7 &       19.6 &      109.0 &        3.7 \\
       452 &       53.210274 &    -27.905891 &          6 &      77.60 &       3.88 &      53.80 &       2.69 &      45.10 &       2.30 &     192.00 &       9.61 &      146.3 &       21.5 &      287.0 &        6.1 \\
       453 &       53.205532 &    -27.907665 &          4 &      63.10 &       3.16 &      43.70 &       2.19 &      42.00 &       2.15 &      32.60 &       1.71 &      114.7 &       12.8 &       97.6 &        3.3 \\
       454 &       53.091736 &    -27.907915 &          5 &      92.30 &       4.62 &      76.90 &       3.85 &      69.10 &       3.48 &     424.00 &      21.21 &      682.3 &       31.3 &     1050.0 &        7.7 \\
       455 &       53.102146 &    -27.911934 &          3 &     127.00 &       6.35 &      90.40 &       4.52 &      93.10 &       4.68 &     648.00 &      32.40 &      516.1 &       25.7 &      747.0 &        7.6 \\
       456 &       53.187485 &    -27.911047 &          5 &     152.00 &       0.08 &     139.00 &       0.10 &     116.00 &       0.52 &     270.00 &       0.51 &      772.5 &       72.2 &      969.0 &        6.9 \\
       457 &       53.095863 &    -27.914566 &          4 &      42.00 &       2.10 &      29.50 &       1.48 &      35.10 &       1.81 &      28.10 &       1.49 &      168.8 &       16.8 &      248.0 &        4.2 \\
       458 &       53.136982 &    -27.914436 &          6 &      48.10 &       2.41 &      42.30 &       2.12 &      43.50 &       2.22 &      79.20 &       3.99 &      160.6 &       19.8 &      253.0 &        5.5 \\
       459 &       53.145592 &    -27.919817 &          5 &      31.80 &       1.59 &      26.40 &       1.32 &      29.50 &       1.54 &      39.00 &       2.01 &      138.3 &       20.9 &      196.0 &        3.3 \\
       460 &       53.169785 &    -27.918215 &          5 &      76.20 &       3.81 &      57.70 &       2.89 &      48.50 &       2.46 &      45.90 &       2.35 &      406.5 &       19.4 &      532.0 &        5.7 \\
       461 &       53.105915 &    -27.919176 &          4 &      27.00 &       1.35 &      20.40 &       1.02 &      15.60 &       0.90 &      17.60 &       1.01 &      146.0 &       16.1 &      179.0 &        3.6 \\
       462 &       53.164043 &    -27.918699 &          6 &      47.70 &       2.39 &      33.40 &       1.67 &      27.20 &       1.42 &     123.00 &       6.17 &       99.8 &       22.6 &      103.0 &        4.4 \\
       463 &       53.165382 &    -27.918707 &          7 &      16.60 &       0.83 &      14.70 &       0.74 &      10.90 &       0.69 &      34.40 &       1.79 &       80.2 &       14.4 &       36.6 &        4.4 \\
       464 &       53.151646 &    -27.918936 &          5 &      15.80 &       0.79 &      12.80 &       0.64 &      10.10 &       0.66 &      10.10 &       0.70 &       71.6 &       11.8 &       76.6 &        3.3 \\
       465 &       53.114258 &    -27.922361 &          5 &      77.20 &       3.86 &      52.90 &       2.65 &      43.70 &       2.23 &     216.00 &      10.81 &      185.6 &       15.7 &      229.0 &        3.5 \\
       466 &       53.179279 &    -27.923651 &          2 &      55.60 &       2.78 &      36.10 &       1.81 &      35.60 &       1.84 &      25.60 &       1.38 &      180.3 &       19.2 &      216.0 &        3.8 \\
       467 &       53.158791 &    -27.925291 &          4 &      13.00 &       0.65 &       9.67 &       0.49 &       7.56 &       0.58 &       6.33 &       0.58 &      105.7 &       21.6 &       55.2 &        3.3 \\
       468 &       53.146065 &    -27.925846 &          5 &    1310.00 &       0.22 &     844.00 &       0.20 &    1220.00 &       1.04 &    3890.00 &       1.03 &     5909.9 &      281.0 &     7090.0 &      709.0 \\
       469 &       53.096340 &    -27.926001 &          5 &      28.90 &       1.45 &      24.40 &       1.22 &      16.80 &       0.95 &      16.50 &       0.97 &      165.1 &       32.6 &      121.0 &        3.3 \\
       470 &       53.122612 &    -27.927292 &          4 &      81.50 &       4.08 &      57.40 &       2.87 &      69.60 &       3.51 &      57.80 &       2.93 &      461.3 &       26.1 &      562.0 &        6.7 \\
       471 &       53.121021 &    -27.928543 &          3 &      48.40 &       2.42 &      49.40 &       2.47 &      38.20 &       1.96 &      31.80 &       1.67 &      117.0 &       19.6 &      180.0 &        3.9 \\
       472 &       53.115948 &    -27.930311 &          4 &      24.90 &       1.25 &      18.80 &       0.94 &      19.50 &       1.07 &      16.00 &       0.95 &       91.0 &       12.9 &      120.0 &        3.2 \\
       473 &       53.125263 &    -27.929554 &          5 &      74.40 &       3.72 &      50.90 &       2.55 &      53.40 &       2.71 &      39.50 &       2.04 &      180.3 &       16.1 &      255.0 &        5.8 \\
       474 &       53.170074 &    -27.929686 &          2 &      14.20 &       0.71 &      21.70 &       1.09 &      36.80 &       1.90 &      97.80 &       4.92 &      417.1 &       39.8 &      717.0 &        8.3 \\
       475 &       53.113453 &    -27.933357 &          2 &     102.00 &       5.10 &      84.40 &       4.22 &      57.80 &       2.93 &      52.80 &       2.69 &      258.0 &       20.9 &      284.0 &        4.4 \\


==> Table4_data.tex <==
    0.6658 &    42 &     0 &      0.000 &      0.000 &     0 &       2.53 &          1 &          1 &         17 &          0 &      25.32 &      23.39 &      22.42 &      22.09 &       0.01 &       0.02 &       0.02 &       0.01 &          1 \\
    1.1120 &    30 &     0 &      0.000 &      0.000 &     0 &       3.31 &          2 &          1 &         27 &          0 &      23.07 &      22.54 &      21.96 &      21.52 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2140 &    42 &     0 &      0.000 &      0.000 &     0 &       2.72 &          1 &          1 &          1 &          0 &      20.50 &      19.34 &      18.79 &      18.57 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    0.6243 &     1 &     0 &      0.000 &      0.000 &     0 &       2.49 &          1 &          1 &         17 &          0 &      26.43 &      24.76 &      23.77 &      23.06 &       0.01 &       0.05 &       0.04 &       0.02 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.70 &          1 &          1 &          1 &          0 &      26.82 &      23.40 &      25.00 &      24.27 &       0.01 &       0.02 &       0.13 &       0.08 &          1 \\
  -99.0000 &    -1 &     1 &      0.000 &      1.300 &     0 &       2.58 &          2 &          1 &          3 &          0 &      24.53 &      23.66 &      22.55 &      21.91 &       0.04 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.21 &          1 &          2 &          3 &          0 &    -999.00 &      27.25 &      27.28 &      25.01 &    -999.00 &       0.43 &       0.76 &       0.10 &          2 \\
    0.7343 &    42 &     0 &      0.000 &      0.000 &     0 &       2.30 &          1 &          1 &          1 &          0 &      23.46 &      22.25 &      21.08 &      20.64 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3570 &    30 &     0 &      0.000 &      0.000 &     0 &       1.96 &          1 &          1 &          1 &          0 &      24.55 &      24.08 &      23.30 &      22.60 &       0.05 &       0.03 &       0.03 &       0.02 &          1 \\
    0.5659 &    42 &     0 &      0.000 &      0.000 &     0 &       2.53 &          1 &          1 &          1 &          0 &      22.93 &      21.69 &      20.86 &      20.52 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1240 &    30 &     0 &      0.000 &      0.000 &     0 &       2.15 &          1 &          1 &          1 &          0 &      26.64 &      25.34 &      24.11 &      23.01 &       0.28 &       0.07 &       0.04 &       0.02 &          1 \\
    1.0368 &    42 &     0 &      0.000 &      0.000 &     0 &       2.88 &          1 &          1 &          1 &          0 &      25.21 &      24.09 &      23.14 &      22.48 &       0.09 &       0.02 &       0.02 &       0.01 &          1 \\
    1.0387 &    42 &     0 &      0.000 &      0.000 &     0 &       4.53 &          1 &          1 &          5 &          0 &      23.33 &      22.93 &      22.34 &      22.03 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.15 &          1 &          1 &          1 &          0 &      23.68 &      23.23 &      22.46 &      21.92 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.43 &          1 &          1 &          1 &          0 &      24.69 &      24.16 &      23.37 &      22.64 &       0.08 &       0.05 &       0.04 &       0.02 &          1 \\
    0.4260 &    72 &     0 &      0.000 &      0.000 &     0 &       2.85 &          1 &          1 &          1 &          0 &      22.06 &      20.98 &      20.47 &      20.20 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0310 &     2 &     1 &     22.000 &     15.000 &     0 &       2.68 &          1 &          1 &          1 &          0 &      20.09 &      19.87 &      19.79 &      19.62 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.22 &          1 &          1 &          1 &          0 &      25.24 &      24.33 &      23.48 &      22.80 &       0.10 &       0.04 &       0.03 &       0.02 &          0 \\
    1.0390 &    72 &     0 &      0.000 &      0.000 &     0 &       3.89 &          2 &          3 &          3 &          0 &      27.42 &      25.27 &      24.55 &      23.94 &       0.75 &       0.12 &       0.10 &       0.07 &          1 \\
    0.6815 &     1 &     0 &      0.000 &      0.000 &     0 &       2.36 &          1 &          1 &          1 &          0 &      23.55 &      22.20 &      21.09 &      20.70 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0450 &    30 &     0 &      0.000 &      0.000 &     0 &       2.02 &          1 &          1 &          1 &          0 &      25.21 &      24.32 &      23.36 &      22.77 &       0.11 &       0.05 &       0.03 &       0.02 &          2 \\
    1.0370 &    30 &     0 &      0.000 &      0.000 &     0 &       3.61 &          2 &          2 &         19 &          0 &      24.68 &      23.57 &      22.55 &      21.75 &       0.07 &       0.02 &       0.01 &       0.01 &          1 \\
    0.7424 &    42 &     0 &      0.000 &      0.000 &     0 &       3.58 &          1 &          1 &          1 &          0 &      22.88 &      22.47 &      21.90 &      21.78 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8949 &    42 &     0 &      0.000 &      0.000 &     0 &       1.77 &          1 &          1 &          1 &          0 &      23.99 &      23.25 &      22.35 &      22.00 &       0.04 &       0.02 &       0.01 &       0.01 &          1 \\
    0.7330 &     2 &     1 &      0.220 &      2.600 &     0 &       1.53 &          1 &          1 &          1 &          0 &      23.47 &      22.50 &      21.45 &      21.08 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.89 &          1 &          1 &          1 &          0 &      23.93 &      23.58 &      23.05 &      22.41 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.78 &          1 &          1 &          1 &          0 &      26.91 &      25.91 &      24.61 &      24.37 &       0.45 &       0.23 &       0.10 &       0.08 &          1 \\
    0.7340 &     2 &     1 &     60.000 &     66.000 &     0 &       2.85 &          1 &          1 &          1 &          0 &      19.39 &      19.27 &      19.14 &      19.03 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1100 &    30 &     0 &      0.000 &      0.000 &     0 &       2.52 &          1 &          1 &          1 &          0 &      24.06 &      23.23 &      22.36 &      21.51 &       0.05 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       5.69 &          1 &          1 &          5 &          0 &      24.54 &      24.06 &      23.50 &      22.82 &       0.04 &       0.02 &       0.02 &       0.02 &          1 \\
    0.3471 &    42 &     0 &      0.000 &      0.000 &     0 &       2.49 &          1 &          1 &          1 &          0 &      22.50 &      21.27 &      20.59 &      20.27 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    1.0440 &    72 &     0 &      0.000 &      0.000 &     0 &       3.17 &          1 &          1 &          1 &          0 &      25.09 &      24.36 &      23.55 &      23.06 &       0.09 &       0.04 &       0.03 &       0.03 &          2 \\
    1.0420 &    62 &     1 &      0.085 &      0.710 &     0 &       3.06 &          1 &          1 &          1 &          0 &      24.32 &      23.15 &      21.78 &      20.90 &       0.07 &       0.02 &       0.01 &       0.01 &          1 \\
    0.8379 &    42 &     0 &      0.000 &      0.000 &     0 &       3.00 &          2 &          2 &          3 &          0 &      23.05 &      22.37 &      21.48 &      21.23 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.15 &          2 &          1 &          3 &          0 &      25.45 &      25.21 &      24.39 &      23.90 &       0.13 &       0.08 &       0.06 &       0.05 &          1 \\
    0.2290 &     2 &     1 &      0.210 &      0.000 &     0 &       2.85 &          1 &          1 &          1 &          0 &      21.06 &      19.59 &      18.99 &      18.75 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     1 &       3.28 &          1 &          1 &          1 &          0 &      17.55 &      17.20 &      16.75 &      16.06 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9773 &    42 &     0 &      0.000 &      0.000 &     0 &       2.76 &          1 &          1 &          1 &          0 &      25.00 &      23.86 &      22.74 &      22.01 &       0.08 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       4.87 &          1 &          1 &          5 &          0 &      20.21 &      19.20 &      18.76 &      18.57 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0450 &    30 &     0 &      0.000 &      0.000 &     0 &       2.55 &          2 &          1 &          3 &          0 &      24.60 &      23.64 &      22.47 &      21.70 &       0.05 &       0.02 &       0.01 &       0.01 &          1 \\
    1.3260 &    30 &     0 &      0.000 &      0.000 &     0 &       2.28 &          1 &          1 &          1 &          0 &      25.23 &      24.81 &      23.91 &      23.13 &       0.10 &       0.06 &       0.05 &       0.03 &          1 \\
    0.6680 &     2 &     1 &      1.200 &     11.000 &     0 &       2.65 &          1 &          1 &          1 &          0 &      24.07 &      22.79 &      21.62 &      21.32 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7340 &     2 &     1 &      0.650 &      2.700 &     0 &       2.87 &          1 &          1 &          1 &          0 &      24.44 &      23.08 &      21.91 &      21.46 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2473 &    42 &     0 &      0.000 &      0.000 &     0 &       2.42 &          1 &          1 &          1 &          0 &      21.43 &      20.35 &      19.88 &      19.70 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8194 &    41 &     0 &      0.000 &      0.000 &     0 &       2.33 &          2 &          1 &          3 &          0 &      23.29 &      23.72 &      22.90 &      22.02 &       0.03 &       0.03 &       0.03 &       0.01 &          1 \\
    1.2966 &    42 &     0 &      0.000 &      0.000 &     0 &       2.75 &          1 &          1 &          1 &          0 &      23.86 &      23.54 &      23.02 &      22.41 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    0.8400 &    42 &     0 &      0.000 &      0.000 &     0 &       1.40 &          2 &          1 &          3 &          0 &      24.51 &      23.65 &      22.73 &      22.42 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.33 &          2 &          1 &          3 &          0 &      23.35 &      22.71 &      21.97 &      21.64 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0175 &     1 &     0 &      0.000 &      0.000 &     0 &       3.24 &          1 &          2 &          3 &          0 &      23.35 &      22.73 &      21.94 &      21.48 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.32 &          2 &          1 &          3 &          0 &      25.91 &      25.45 &      24.65 &      24.01 &       0.18 &       0.11 &       0.09 &       0.05 &          2 \\
    1.0422 &    42 &     0 &      0.000 &      0.000 &     0 &       3.23 &          1 &          1 &         17 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    2.6087 &    41 &     1 &      0.790 &      1.700 &     0 &       2.12 &          1 &          1 &          1 &          0 &      24.74 &      23.63 &      22.94 &      22.15 &       0.05 &       0.02 &       0.02 &       0.01 &          1 \\
    1.6170 &     2 &     1 &      3.100 &      2.900 &     0 &       2.74 &          1 &          1 &          1 &          0 &      27.06 &      26.10 &      24.71 &      23.66 &       0.38 &       0.14 &       0.06 &       0.03 &          2 \\
    0.0000 &    42 &     0 &      0.000 &      0.000 &     1 &       3.83 &          1 &          1 &          1 &          0 &      19.27 &      18.21 &      17.30 &      16.89 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.01 &          1 &          1 &          1 &          0 &      22.99 &      22.18 &      21.41 &      21.19 &       0.02 &       0.01 &       0.01 &       0.01 &          2 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.76 &          1 &          1 &          1 &          0 &      22.92 &      22.11 &      21.33 &      21.07 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4698 &    42 &     0 &      0.000 &      0.000 &     0 &       3.39 &          1 &          2 &         19 &          0 &      23.63 &      22.21 &      21.38 &      20.95 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0880 &    30 &     0 &      0.000 &      0.000 &     0 &       4.65 &          1 &          2 &          7 &          0 &      23.73 &      22.97 &      21.99 &      21.18 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.0000 &    42 &     0 &      0.000 &      0.000 &     1 &       2.19 &          1 &          1 &          1 &          0 &      16.59 &      15.87 &      15.41 &      14.81 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7360 &     2 &     1 &      0.000 &      1.200 &     0 &       3.38 &          1 &          1 &          1 &          0 &      23.45 &      22.59 &      21.58 &      21.22 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.57 &          1 &          1 &          1 &          0 &      27.03 &      25.70 &      24.38 &      23.61 &       0.30 &       0.08 &       0.04 &       0.02 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.53 &          1 &          1 &          1 &          0 &      27.21 &      27.09 &      26.16 &      25.35 &       0.43 &       0.25 &       0.18 &       0.09 &          0 \\
    0.6194 &    42 &     0 &      0.000 &      0.000 &     0 &       1.67 &          1 &          1 &         17 &          0 &      22.47 &      21.81 &      21.25 &      21.11 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.43 &          1 &          1 &          1 &          0 &      23.23 &      22.93 &      22.29 &      21.89 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5450 &     2 &     1 &      0.200 &      1.200 &     0 &       2.53 &          2 &          1 &          3 &          0 &      23.93 &      22.79 &      21.78 &      21.57 &       0.05 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.59 &          1 &          1 &          1 &          0 &      24.10 &      23.88 &      23.33 &      22.95 &       0.03 &       0.02 &       0.02 &       0.02 &          1 \\
    0.6050 &     2 &     1 &      2.300 &     14.000 &     0 &       2.60 &          1 &          1 &          1 &          0 &      21.66 &      20.64 &      19.83 &      19.59 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.96 &          1 &          1 &          1 &          0 &      25.93 &      25.14 &      24.72 &      24.07 &       0.18 &       0.08 &       0.08 &       0.05 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.35 &          2 &          1 &          3 &          0 &    -999.00 &      27.27 &      25.96 &      25.26 &    -999.00 &       0.36 &       0.18 &       0.10 &          1 \\
    0.6776 &     1 &     0 &      0.000 &      0.000 &     0 &       2.51 &          1 &          1 &          9 &          0 &      23.71 &      22.63 &      21.67 &      21.33 &       0.03 &       0.01 &       0.01 &       0.01 &          2 \\
    0.4179 &    41 &     1 &      0.110 &      0.000 &     0 &       2.12 &          1 &          1 &          1 &          0 &      21.85 &      19.97 &      19.08 &      18.72 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1820 &    30 &     0 &      0.000 &      0.000 &     0 &       2.56 &          1 &          1 &          1 &          0 &      24.95 &      24.47 &      23.69 &      23.02 &       0.08 &       0.05 &       0.04 &       0.03 &          1 \\
  -99.0000 &    -1 &     1 &      0.230 &      0.590 &     0 &       2.47 &          1 &          2 &          3 &          0 &      22.52 &      21.69 &      20.96 &      20.74 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7350 &     2 &     1 &      0.000 &      1.800 &     0 &       3.04 &          1 &          1 &          1 &          0 &      23.33 &      22.26 &      21.23 &      20.83 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3459 &    42 &     0 &      0.000 &      0.000 &     0 &       2.90 &          1 &          1 &          1 &          0 &      23.11 &      21.57 &      20.80 &      20.46 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2960 &    30 &     0 &      0.000 &      0.000 &     0 &       2.55 &          1 &          1 &          1 &          0 &      23.98 &      23.73 &      23.09 &      22.39 &       0.05 &       0.02 &       0.02 &       0.01 &          2 \\
    0.5477 &    42 &     0 &      0.000 &      0.000 &     0 &       2.10 &          1 &          1 &          1 &          0 &      23.98 &      22.78 &      22.00 &      21.68 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    2.1447 &    41 &     0 &      0.000 &      0.000 &     0 &       2.70 &          2 &          1 &          3 &          0 &      25.80 &      25.18 &      24.80 &      24.49 &       0.07 &       0.04 &       0.04 &       0.04 &          1 \\
    0.9250 &    42 &     0 &      0.000 &      0.000 &     0 &       2.24 &          1 &          1 &          1 &          0 &      24.65 &      23.64 &      22.48 &      21.70 &       0.06 &       0.02 &       0.01 &       0.01 &          1 \\
    0.9667 &    42 &     0 &      0.000 &      0.000 &     0 &       3.06 &          1 &          1 &          1 &          0 &      22.35 &      22.11 &      21.53 &      21.29 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5690 &     2 &     1 &      4.000 &      4.800 &     0 &       2.49 &          1 &          2 &          3 &          0 &      23.12 &      21.73 &      20.85 &      20.58 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0207 &    42 &     0 &      0.000 &      0.000 &     0 &       3.30 &          3 &          1 &          3 &          0 &      24.29 &      23.41 &      22.41 &      21.97 &       0.07 &       0.03 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.060 &      0.000 &     0 &       2.78 &          2 &          1 &          3 &          0 &      24.36 &      24.08 &      23.46 &      22.72 &       0.04 &       0.03 &       0.03 &       0.02 &          1 \\
    2.2910 &     2 &     1 &      1.300 &      4.700 &     0 &       2.40 &          1 &          1 &          1 &          0 &      27.41 &      25.77 &      25.26 &      24.90 &       0.46 &       0.09 &       0.09 &       0.08 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.33 &          1 &          1 &          1 &          0 &      27.35 &      26.24 &      25.41 &      24.41 &       0.54 &       0.18 &       0.14 &       0.06 &          0 \\
  -99.0000 &    -1 &     1 &      5.100 &      8.000 &     0 &       2.73 &          1 &          1 &          1 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    0.6715 &    42 &     0 &      0.000 &      0.000 &     0 &       2.07 &          1 &          1 &          1 &          0 &      22.68 &      21.63 &      20.69 &      20.38 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2246 &    42 &     0 &      0.000 &      0.000 &     0 &       2.63 &          1 &          1 &         17 &          0 &      23.75 &      23.40 &      22.82 &      22.29 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    0.6083 &    42 &     0 &      0.000 &      0.000 &     0 &       2.50 &          1 &          1 &          1 &          0 &      23.38 &      22.07 &      21.11 &      20.77 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0179 &    42 &     0 &      0.000 &      0.000 &     0 &       2.24 &          1 &          1 &          1 &          0 &      24.68 &      24.10 &      23.18 &      22.70 &       0.06 &       0.03 &       0.02 &       0.02 &          1 \\
    0.1030 &     2 &     1 &      0.190 &      0.320 &     0 &       3.24 &          1 &          1 &          1 &          0 &      19.04 &      17.68 &      17.12 &      16.85 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6150 &    30 &     0 &      0.000 &      0.000 &     0 &       2.65 &          2 &          1 &          3 &          0 &      22.82 &      21.70 &      20.82 &      20.49 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0360 &    30 &     0 &      0.000 &      0.000 &     0 &       3.38 &          2 &          2 &          3 &          0 &      24.18 &      23.60 &      22.75 &      22.23 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    0.1183 &    42 &     0 &      0.000 &      0.000 &     0 &       2.92 &          1 &          1 &          1 &          0 &      21.08 &      20.10 &      19.59 &      19.37 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0980 &    30 &     0 &      0.000 &      0.000 &     0 &       3.09 &          3 &          2 &          3 &          0 &      24.00 &      23.14 &      22.23 &      21.58 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.43 &          2 &          2 &          3 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    1.0370 &     2 &     1 &      5.300 &      6.200 &     0 &       0.49 &          1 &          1 &          5 &          0 &      22.72 &      22.35 &      22.29 &      22.13 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.20 &          2 &          1 &          3 &          0 &      29.26 &      26.64 &      25.31 &      24.51 &       2.73 &       0.22 &       0.11 &       0.06 &          1 \\
    1.0250 &    30 &     0 &      0.000 &      0.000 &     0 &       2.43 &          1 &          1 &          1 &          0 &      26.62 &      25.22 &      23.81 &      22.98 &       0.27 &       0.07 &       0.03 &       0.02 &          1 \\
    0.7979 &    42 &     1 &      0.000 &      1.700 &     0 &       2.51 &          2 &          1 &          3 &          0 &      25.32 &      24.51 &      23.32 &      22.67 &       0.10 &       0.04 &       0.02 &       0.01 &          1 \\
    1.2150 &    30 &     0 &      0.000 &      0.000 &     0 &       2.32 &          1 &          1 &          1 &          0 &      24.16 &      23.62 &      22.99 &      22.32 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
    0.9998 &    42 &     0 &      0.000 &      0.000 &     0 &       1.78 &          1 &          1 &          1 &          0 &      24.01 &      23.27 &      22.28 &      21.70 &       0.04 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.84 &          2 &          1 &          3 &          0 &      27.95 &      28.81 &      27.59 &      26.52 &       0.31 &       0.71 &       0.39 &       0.18 &          0 \\
    0.9601 &    42 &     0 &      0.000 &      0.000 &     0 &       2.57 &          1 &          1 &          1 &          0 &      25.82 &      24.01 &      22.57 &      21.86 &       0.17 &       0.03 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.28 &          1 &          1 &          1 &          0 &      24.92 &      24.73 &      24.19 &      23.52 &       0.06 &       0.04 &       0.04 &       0.03 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       0.99 &          1 &          1 &          5 &          0 &      25.79 &      25.12 &      24.63 &      23.87 &       0.13 &       0.07 &       0.07 &       0.04 &          1 \\
    0.9980 &    30 &     1 &      0.130 &      0.360 &     0 &       4.01 &          1 &          2 &          7 &          0 &      23.18 &      22.61 &      21.64 &      21.01 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6678 &    42 &     0 &      0.000 &      0.000 &     0 &       3.19 &          1 &          1 &          1 &          0 &      21.79 &      20.94 &      20.06 &      19.79 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4220 &    42 &     0 &      0.000 &      0.000 &     0 &       2.51 &          1 &          1 &          1 &          0 &      23.19 &      21.94 &      21.26 &      20.90 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2158 &    42 &     0 &      0.000 &      0.000 &     0 &       2.71 &          1 &          1 &          1 &          0 &      23.93 &      23.49 &      22.82 &      21.91 &       0.06 &       0.03 &       0.02 &       0.01 &          1 \\
    1.5500 &    30 &     0 &      0.000 &      0.000 &     0 &       2.64 &          1 &          1 &          1 &          0 &      25.72 &      24.99 &      24.03 &      23.51 &       0.10 &       0.04 &       0.03 &       0.02 &          2 \\
    0.0760 &     2 &     1 &      0.610 &      0.900 &     0 &       3.14 &          1 &          1 &          1 &          1 &      18.24 &      17.44 &      17.02 &      16.85 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &      10.07 &          1 &          1 &          5 &          0 &      25.18 &      24.65 &      24.00 &      23.62 &       0.10 &       0.05 &       0.05 &       0.04 &          1 \\
    0.1029 &    42 &     0 &      0.000 &      0.000 &     0 &       3.12 &          1 &          1 &          1 &          0 &      20.26 &      19.03 &      18.50 &      18.27 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    1.0170 &     9 &     0 &      0.000 &      0.000 &     0 &       2.64 &          1 &          1 &          1 &          0 &      25.12 &      24.02 &      23.02 &      22.43 &       0.08 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.58 &          1 &          1 &          1 &          0 &      23.83 &      23.31 &      22.57 &      22.00 &       0.03 &       0.01 &       0.01 &       0.01 &          2 \\
    1.1270 &     9 &     0 &      0.000 &      0.000 &     0 &       1.80 &          2 &          1 &          3 &          0 &      24.43 &      23.73 &      22.95 &      22.15 &       0.06 &       0.03 &       0.02 &       0.01 &          1 \\
    1.3250 &     9 &     0 &      0.000 &      0.000 &     0 &       2.57 &          1 &          1 &          1 &          0 &      23.84 &      23.50 &      22.98 &      22.34 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    1.6150 &     2 &     1 &      5.600 &      7.200 &     0 &       2.26 &          1 &          1 &          1 &          0 &      23.70 &      22.93 &      22.37 &      22.34 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1520 &    30 &     0 &      0.000 &      0.000 &     0 &       1.75 &          1 &          1 &          1 &          0 &      24.75 &      24.09 &      23.40 &      22.71 &       0.05 &       0.02 &       0.02 &       0.01 &          1 \\
    1.2994 &    42 &     0 &      0.000 &      0.000 &     0 &       3.05 &          2 &          1 &          3 &          0 &      25.00 &      24.60 &      23.91 &      23.30 &       0.08 &       0.05 &       0.04 &       0.03 &          1 \\
    0.5241 &    42 &     0 &      0.000 &      0.000 &     0 &       2.51 &          1 &          1 &          1 &          0 &      23.19 &      21.98 &      21.24 &      20.92 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7380 &     2 &     0 &      0.000 &      0.000 &     0 &       2.72 &          1 &          1 &          1 &          0 &      22.48 &      21.55 &      20.62 &      20.29 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7380 &     9 &     0 &      0.000 &      0.000 &     0 &       3.32 &          1 &          1 &          1 &          0 &      23.92 &      23.11 &      22.29 &      22.03 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0380 &     9 &     0 &      0.000 &      0.000 &     0 &       2.53 &          1 &          1 &          1 &          0 &      23.24 &      22.90 &      22.30 &      21.97 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2150 &     9 &     0 &      0.000 &      0.000 &     0 &       4.65 &          1 &          2 &         15 &          0 &      21.38 &      20.48 &      20.08 &      19.95 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.0760 &     2 &     1 &      0.670 &      0.000 &     0 &       3.63 &          1 &          1 &          1 &          1 &      17.70 &      16.99 &      16.60 &      16.46 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5218 &     1 &     0 &      0.000 &      0.000 &     0 &       2.18 &          1 &          1 &          1 &          0 &      23.37 &      21.76 &      20.91 &      20.62 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5340 &     2 &     0 &      0.000 &      0.000 &     0 &       3.71 &          2 &          1 &          3 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    1.2170 &     9 &     0 &      0.000 &      0.000 &     0 &       2.15 &          1 &          1 &          1 &          0 &      24.42 &      23.76 &      23.03 &      22.18 &       0.05 &       0.03 &       0.02 &       0.01 &          1 \\
    0.8910 &     9 &     0 &      0.000 &      0.000 &     0 &       2.20 &          2 &          1 &          3 &          0 &      26.94 &      24.72 &      23.25 &      22.62 &       0.34 &       0.04 &       0.02 &       0.01 &          0 \\
    1.2230 &    30 &     0 &      0.000 &      0.000 &     0 &       3.06 &          3 &          2 &          3 &          1 &      24.06 &      23.78 &      23.36 &      22.83 &       0.04 &       0.03 &       0.03 &       0.02 &          1 \\
    0.7360 &     9 &     0 &      0.000 &      0.000 &     0 &       2.26 &          1 &          1 &          1 &          0 &      26.68 &      24.61 &      23.14 &      22.68 &       0.24 &       0.03 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.79 &          1 &          1 &          1 &          0 &    -999.00 &      27.44 &      26.84 &      26.38 &    -999.00 &       0.23 &       0.21 &       0.16 &          1 \\
    0.2170 &     2 &     0 &      0.000 &      0.000 &     0 &       1.12 &          1 &          1 &         13 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    0.5220 &     2 &     0 &      0.000 &      0.000 &     0 &       3.00 &          2 &          1 &          3 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          2 \\
    1.1090 &    30 &     0 &      0.000 &      0.000 &     0 &       2.64 &          1 &          1 &          1 &          0 &      25.64 &      24.93 &      24.07 &      23.48 &       0.16 &       0.07 &       0.05 &       0.04 &          1 \\
    0.2150 &     9 &     1 &      0.043 &      0.000 &     0 &       4.64 &          1 &          2 &          7 &          0 &      21.50 &      20.36 &      19.88 &      19.71 &       0.01 &       0.01 &       0.01 &       0.01 &          3 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.36 &          1 &          1 &          1 &          0 &      28.23 &      26.10 &      24.95 &      23.99 &       1.46 &       0.18 &       0.10 &       0.05 &          1 \\
    1.0380 &     9 &     0 &      0.000 &      0.000 &     0 &       3.11 &          2 &          1 &          3 &          0 &      24.26 &      23.56 &      22.93 &      22.48 &       0.04 &       0.02 &       0.02 &       0.02 &          1 \\
    0.0860 &     9 &     0 &      0.000 &      0.000 &     0 &       2.54 &          1 &          1 &          1 &          0 &      19.69 &      18.89 &      18.44 &      18.29 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2960 &    30 &     0 &      0.000 &      0.000 &     0 &       2.65 &          1 &          1 &          1 &          0 &      25.20 &      24.55 &      23.78 &      22.98 &       0.12 &       0.06 &       0.05 &       0.03 &          1 \\
    0.9690 &     9 &     0 &      0.000 &      0.000 &     0 &       2.78 &          1 &          1 &          1 &          0 &      23.25 &      22.42 &      21.44 &      20.96 &       0.03 &       0.01 &       0.01 &       0.01 &          0 \\
    1.8930 &    41 &     1 &      0.073 &      3.600 &     0 &       3.00 &          2 &          1 &          3 &          0 &      25.95 &      25.25 &      24.67 &      24.28 &       0.09 &       0.04 &       0.04 &       0.03 &          1 \\
    0.7351 &    42 &     0 &      0.000 &      0.000 &     0 &       2.30 &          2 &          1 &          3 &          0 &      25.36 &      23.40 &      22.02 &      21.56 &       0.08 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9760 &     9 &     0 &      0.000 &      0.000 &     0 &       2.65 &          2 &          1 &          3 &          0 &      23.85 &      23.26 &      22.54 &      22.18 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2020 &    30 &     0 &      0.000 &      0.000 &     0 &       2.81 &          1 &          1 &          1 &          0 &      25.48 &      24.82 &      23.82 &      23.12 &       0.12 &       0.05 &       0.04 &       0.02 &          0 \\
    1.0980 &    30 &     0 &      0.000 &      0.000 &     0 &       4.44 &          1 &          1 &          5 &          0 &      23.96 &      23.71 &      23.10 &      22.65 &       0.03 &       0.02 &       0.02 &       0.02 &          1 \\
    0.5487 &     1 &     0 &      0.000 &      0.000 &     0 &       2.39 &          1 &          1 &          1 &          0 &      22.05 &      21.05 &      20.30 &      20.03 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2940 &     9 &     0 &      0.000 &      0.000 &     0 &       2.68 &          1 &          1 &          1 &          0 &      25.56 &      24.66 &      23.64 &      22.71 &       0.12 &       0.05 &       0.03 &       0.02 &          0 \\
    0.7380 &     9 &     1 &      6.600 &      7.100 &     0 &       2.98 &          2 &          1 &         11 &          0 &      22.61 &      22.08 &      21.72 &      21.51 &       0.01 &       0.01 &       0.01 &       0.01 &          0 \\
    1.6070 &    30 &     0 &      0.000 &      0.000 &     0 &       2.85 &          2 &          1 &          3 &          0 &      27.36 &      26.71 &      25.67 &      24.43 &       0.53 &       0.27 &       0.17 &       0.06 &          1 \\
  -99.0000 &    -1 &     1 &      0.063 &      0.000 &     0 &       2.53 &          1 &          1 &         17 &          0 &      24.52 &      23.67 &      22.72 &      22.11 &       0.04 &       0.02 &       0.01 &       0.01 &          1 \\
    0.3240 &     9 &     0 &      0.000 &      0.000 &     0 &       3.83 &          1 &          1 &          9 &          0 &      21.65 &      20.72 &      20.39 &      20.18 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8400 &    72 &     0 &      0.000 &      0.000 &     0 &       2.53 &          1 &          1 &          1 &          0 &      23.97 &      23.24 &      22.27 &      21.85 &       0.03 &       0.02 &       0.01 &       0.01 &          0 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       0.76 &          1 &          1 &          5 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    0.6440 &     9 &     0 &      0.000 &      0.000 &     0 &       1.62 &          1 &          1 &          1 &          0 &      23.15 &      22.36 &      21.61 &      21.39 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6810 &     9 &     0 &      0.000 &      0.000 &     0 &       3.71 &          1 &          1 &          1 &          0 &      21.94 &      21.21 &      20.47 &      20.28 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9600 &     2 &     1 &      1.600 &      1.600 &     0 &       4.54 &          2 &          3 &          7 &          0 &      23.66 &      23.00 &      22.31 &      21.82 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9540 &     9 &     1 &      0.000 &      0.270 &     0 &       5.14 &          1 &          2 &         23 &          0 &      23.28 &      22.56 &      21.57 &      21.02 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0390 &     9 &     0 &      0.000 &      0.000 &     0 &       2.75 &          1 &          1 &          1 &          0 &      24.38 &      23.74 &      22.93 &      22.40 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
    1.0940 &    30 &     0 &      0.000 &      0.000 &     0 &       3.29 &          1 &          1 &          1 &          0 &      23.81 &      23.20 &      22.42 &      21.86 &       0.05 &       0.03 &       0.02 &       0.01 &          1 \\
    1.1890 &    30 &     0 &      0.000 &      0.000 &     0 &       2.47 &          1 &          1 &          1 &          0 &      26.37 &      25.08 &      23.93 &      23.09 &       0.22 &       0.06 &       0.04 &       0.02 &          2 \\
    0.8310 &     9 &     0 &      0.000 &      0.000 &     0 &       2.48 &          1 &          1 &          1 &          0 &      24.58 &      23.44 &      22.32 &      21.86 &       0.06 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.61 &          1 &          1 &          1 &          0 &      24.39 &      23.67 &      22.64 &      21.83 &       0.07 &       0.03 &       0.02 &       0.01 &          1 \\
    0.5344 &    42 &     0 &      0.000 &      0.000 &     0 &       2.40 &          1 &          1 &          1 &          0 &      22.56 &      21.60 &      20.95 &      20.69 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2150 &     9 &     1 &      6.500 &      9.600 &     0 &       3.43 &          1 &          1 &          1 &          0 &      21.15 &      21.16 &      21.14 &      21.11 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4970 &    72 &     0 &      0.000 &      0.000 &     0 &       2.75 &          1 &          1 &          1 &          0 &      22.86 &      20.93 &      19.94 &      19.59 &       0.02 &       0.01 &       0.01 &       0.01 &          2 \\
    0.5230 &    30 &     0 &      0.000 &      0.000 &     0 &       2.21 &          1 &          1 &          1 &          0 &      23.04 &      21.62 &      20.71 &      20.32 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.060 &      0.000 &     0 &       3.32 &          2 &          1 &          3 &          0 &      21.56 &      20.78 &      20.41 &      20.30 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2890 &     9 &     0 &      0.000 &      0.000 &     0 &       2.79 &          1 &          1 &         17 &          0 &      23.29 &      21.63 &      20.81 &      20.43 &       0.03 &       0.01 &       0.01 &       0.01 &          0 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.75 &          1 &          1 &         17 &          0 &      24.45 &      24.08 &      23.48 &      23.07 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    0.4260 &     9 &     0 &      0.000 &      0.000 &     0 &       2.44 &          2 &          1 &          3 &          0 &      23.84 &      22.60 &      21.96 &      21.58 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9530 &    30 &     1 &      0.930 &      2.200 &     0 &       3.66 &          2 &          2 &          3 &          1 &      24.23 &      22.93 &      21.78 &      21.14 &       0.06 &       0.02 &       0.01 &       0.01 &          1 \\
    0.9550 &     9 &     0 &      0.000 &      0.000 &     0 &       7.83 &          2 &          2 &         15 &          0 &      23.56 &      22.66 &      21.61 &      20.93 &       0.04 &       0.02 &       0.01 &       0.01 &          1 \\
    0.5230 &     9 &     0 &      0.000 &      0.000 &     0 &       6.01 &          1 &          1 &         21 &          0 &      24.98 &      23.23 &      22.12 &      21.68 &       0.07 &       0.01 &       0.01 &       0.01 &          0 \\
    0.8467 &    42 &     0 &      0.000 &      0.000 &     0 &       4.05 &          2 &          1 &          7 &          0 &      23.14 &      22.58 &      21.87 &      21.64 &       0.01 &       0.01 &       0.01 &       0.01 &          0 \\
    1.2200 &    30 &     0 &      0.000 &      0.000 &     0 &       2.48 &          1 &          1 &          1 &          0 &      23.71 &      23.25 &      22.69 &      22.05 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3370 &     3 &     0 &      0.000 &      0.000 &     0 &       3.13 &          1 &          1 &          1 &          0 &      22.05 &      20.97 &      20.55 &      20.33 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0380 &     9 &     0 &      0.000 &      0.000 &     0 &       1.38 &          1 &          1 &         17 &          0 &      23.26 &      22.82 &      22.18 &      21.78 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3290 &    30 &     0 &      0.000 &      0.000 &     0 &       3.41 &          1 &          1 &          1 &          0 &      27.21 &      25.95 &      24.90 &      23.69 &       0.47 &       0.14 &       0.09 &       0.03 &          1 \\
    1.2230 &     9 &     1 &      0.056 &      0.000 &     0 &       3.28 &          2 &          1 &          3 &          0 &      24.53 &      23.96 &      23.15 &      22.36 &       0.05 &       0.03 &       0.02 &       0.01 &          1 \\
    0.7380 &     9 &     1 &      0.000 &      0.320 &     0 &       3.23 &          1 &          1 &          1 &          0 &      25.06 &      22.74 &      21.27 &      20.77 &       0.08 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0960 &     9 &     0 &      0.000 &      0.000 &     0 &       2.14 &          1 &          1 &          1 &          0 &      25.66 &      24.95 &      24.02 &      23.29 &       0.09 &       0.04 &       0.03 &       0.02 &          1 \\
    0.7270 &     2 &     0 &      0.000 &      0.000 &     0 &       5.19 &          1 &          2 &          7 &          0 &      24.07 &      23.24 &      22.34 &      22.05 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3650 &     9 &     0 &      0.000 &      0.000 &     0 &       2.81 &          1 &          1 &          1 &          0 &      21.84 &      20.98 &      20.67 &      20.47 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0300 &     9 &     0 &      0.000 &      0.000 &     0 &       2.64 &          1 &          1 &          1 &          0 &      25.45 &      24.72 &      23.33 &      22.54 &       0.18 &       0.09 &       0.04 &       0.02 &          1 \\
    1.2160 &     2 &     1 &      1.900 &      5.400 &     0 &       2.46 &          1 &          1 &          1 &          0 &      21.24 &      20.98 &      20.98 &      21.02 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8950 &     9 &     0 &      0.000 &      0.000 &     0 &       2.43 &          1 &          1 &          1 &          0 &      25.41 &      24.56 &      23.63 &      23.23 &       0.06 &       0.02 &       0.02 &       0.01 &          1 \\
    0.6700 &     9 &     0 &      0.000 &      0.000 &     0 &       2.88 &          2 &          1 &          3 &          0 &      23.42 &      21.94 &      20.84 &      20.46 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3660 &     9 &     0 &      0.000 &      0.000 &     0 &       3.17 &          2 &          2 &          3 &          0 &      22.54 &      21.11 &      20.44 &      20.09 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1090 &     9 &     0 &      0.000 &      0.000 &     0 &       2.93 &          1 &          1 &          1 &          0 &      25.70 &      25.14 &      24.19 &      23.56 &       0.13 &       0.07 &       0.05 &       0.03 &          1 \\
    1.2950 &    30 &     0 &      0.000 &      0.000 &     0 &       5.54 &          1 &          2 &         23 &          0 &      24.08 &      23.82 &      23.38 &      22.68 &       0.04 &       0.03 &       0.03 &       0.02 &          1 \\
    0.6690 &    72 &     0 &      0.000 &      0.000 &     0 &       2.34 &          2 &          1 &          3 &          0 &      22.39 &      21.53 &      20.69 &      20.41 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.7300 &    41 &     1 &      0.340 &      4.300 &     0 &       3.99 &          1 &          2 &          3 &          0 &      25.30 &      25.17 &      24.64 &      24.37 &       0.04 &       0.03 &       0.03 &       0.03 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.48 &          1 &          1 &          1 &          0 &      23.98 &      23.58 &      22.87 &      22.51 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    1.2200 &    30 &     0 &      0.000 &      0.000 &     0 &       1.90 &          1 &          1 &          1 &          0 &      26.71 &      25.73 &      24.95 &      24.09 &       0.23 &       0.09 &       0.07 &       0.04 &          1 \\
  -99.0000 &    -1 &     1 &      0.890 &      2.800 &     0 &       3.01 &          1 &          2 &          3 &          0 &      25.41 &      25.06 &      24.22 &      23.77 &       0.14 &       0.09 &       0.08 &       0.06 &          1 \\
    0.6218 &    42 &     0 &      0.000 &      0.000 &     0 &       3.04 &          1 &          1 &          1 &          0 &      22.02 &      21.17 &      20.39 &      20.15 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8960 &     9 &     1 &      0.051 &      0.000 &     0 &       2.76 &          1 &          1 &          1 &          0 &      24.03 &      23.03 &      22.09 &      21.73 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3070 &     9 &     0 &      0.000 &      0.000 &     0 &       3.35 &          1 &          2 &          3 &          0 &      23.89 &      23.45 &      22.91 &      22.29 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.09 &          2 &          1 &          3 &          0 &      25.84 &      24.75 &      23.72 &      22.92 &       0.14 &       0.05 &       0.03 &       0.02 &          1 \\
    0.3330 &     3 &     0 &      0.000 &      0.000 &     0 &       2.33 &          1 &          1 &          1 &          0 &      23.65 &      22.05 &      21.27 &      20.94 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0330 &     9 &     1 &      0.110 &      0.730 &     0 &       2.64 &          3 &          1 &          3 &          0 &      24.61 &      23.60 &      22.53 &      21.84 &       0.07 &       0.02 &       0.01 &       0.01 &          1 \\
    1.0160 &     9 &     0 &      0.000 &      0.000 &     0 &       5.83 &          1 &          2 &          7 &          0 &      24.92 &      23.83 &      22.35 &      21.61 &       0.06 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.81 &          1 &          1 &         17 &          0 &      25.25 &      24.74 &      23.74 &      22.92 &       0.13 &       0.07 &       0.05 &       0.03 &          1 \\
    1.2210 &     9 &     0 &      0.000 &      0.000 &     0 &       4.18 &          2 &          1 &          7 &          0 &      23.07 &      22.86 &      22.50 &      22.03 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7350 &     9 &     1 &      0.050 &      0.000 &     0 &       4.11 &          2 &          2 &         15 &          0 &      25.08 &      23.83 &      22.94 &      22.59 &       0.11 &       0.03 &       0.02 &       0.02 &          0 \\
    1.0870 &     9 &     0 &      0.000 &      0.000 &     0 &       3.53 &          2 &          2 &          3 &          0 &      22.42 &      22.12 &      21.58 &      21.12 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2880 &    30 &     0 &      0.000 &      0.000 &     0 &       2.17 &          1 &          1 &          1 &          0 &      23.81 &      23.56 &      23.17 &      22.53 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.10 &          1 &          1 &          1 &          0 &      29.02 &      28.04 &      26.21 &      25.72 &       1.49 &       0.57 &       0.17 &       0.13 &          1 \\
    0.7370 &     9 &     0 &      0.000 &      0.000 &     0 &       2.46 &          1 &          1 &          1 &          0 &      25.26 &      23.86 &      22.46 &      21.91 &       0.10 &       0.02 &       0.01 &       0.01 &          1 \\
    0.0000 &    72 &     0 &      0.000 &      0.000 &     1 &       3.01 &          1 &          1 &          1 &          0 &      23.54 &      16.75 &      16.21 &      15.39 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0940 &     9 &     0 &      0.000 &      0.000 &     0 &       4.90 &          2 &          2 &          7 &          0 &      26.01 &      24.81 &      23.62 &      22.76 &       0.15 &       0.05 &       0.03 &       0.01 &          1 \\
    0.8370 &     9 &     0 &      0.000 &      0.000 &     0 &       1.59 &          2 &          1 &          3 &          0 &      25.36 &      24.42 &      23.24 &      22.83 &       0.09 &       0.03 &       0.02 &       0.01 &          1 \\
    0.9990 &     9 &     1 &      0.050 &      0.000 &     0 &       4.03 &          3 &          3 &          7 &          0 &      25.10 &      23.95 &      22.91 &      22.30 &       0.10 &       0.03 &       0.02 &       0.01 &          1 \\
    1.0470 &     9 &     0 &      0.000 &      0.000 &     0 &       3.61 &          3 &          3 &          3 &          0 &      23.98 &      23.48 &      22.68 &      22.30 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
    0.7640 &     2 &     0 &      0.000 &      0.000 &     0 &       4.57 &          3 &          3 &          7 &          0 &      23.05 &      22.50 &      21.66 &      21.45 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.870 &      1.300 &     0 &       2.82 &          1 &          1 &          1 &          0 &      28.61 &      27.97 &      27.08 &      25.87 &       0.82 &       0.40 &       0.31 &       0.11 &          2 \\
    0.4190 &    72 &     0 &      0.000 &      0.000 &     0 &       2.92 &          1 &          1 &          1 &          0 &      22.52 &      21.53 &      21.03 &      20.75 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    2.2230 &     9 &     1 &      0.049 &      0.320 &     0 &       2.56 &          1 &          1 &          1 &          0 &      24.40 &      23.65 &      23.21 &      22.89 &       0.03 &       0.01 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.027 &      0.000 &     0 &       4.76 &          2 &          2 &          7 &          0 &      25.41 &      24.86 &      24.69 &      24.47 &       0.07 &       0.04 &       0.06 &       0.05 &          1 \\
    0.6250 &     2 &     0 &      0.000 &      0.000 &     0 &       5.27 &          3 &          2 &          7 &          0 &      25.46 &      23.54 &      22.25 &      21.81 &       0.08 &       0.01 &       0.01 &       0.01 &          1 \\
    1.4260 &    30 &     0 &      0.000 &      0.000 &     0 &       1.48 &          1 &          1 &          1 &          0 &      24.43 &      24.20 &      23.70 &      23.23 &       0.04 &       0.03 &       0.03 &       0.02 &          1 \\
    1.2200 &    30 &     1 &      0.150 &      7.100 &     0 &       2.33 &          1 &          1 &          1 &          0 &      26.41 &      25.44 &      24.87 &      23.97 &       0.25 &       0.09 &       0.09 &       0.04 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.60 &          1 &          1 &          1 &          0 &      25.19 &      23.89 &      22.81 &      22.40 &       0.11 &       0.03 &       0.02 &       0.01 &          1 \\
    0.2470 &     9 &     0 &      0.000 &      0.000 &     0 &       2.45 &          1 &          1 &         17 &          0 &      22.22 &      20.53 &      19.73 &      19.38 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6259 &    42 &     0 &      0.000 &      0.000 &     0 &       3.77 &          2 &          1 &          3 &          0 &      22.94 &      22.28 &      21.74 &      21.71 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.0000 &     9 &     0 &      0.000 &      0.000 &     1 &       2.80 &          1 &          1 &          1 &          0 &      20.96 &      19.24 &      17.97 &      17.26 &       0.01 &       0.01 &       0.01 &       0.01 &          0 \\
  -99.0000 &    -1 &     1 &      0.540 &      0.650 &     0 &       3.26 &          1 &          1 &          1 &          0 &      25.24 &      24.62 &      24.49 &      24.38 &       0.05 &       0.02 &       0.04 &       0.03 &          1 \\
    1.0970 &     9 &     0 &      0.000 &      0.000 &     0 &       2.54 &          1 &          1 &          1 &          0 &      25.06 &      24.19 &      23.32 &      22.71 &       0.06 &       0.02 &       0.02 &       0.01 &          1 \\
    0.3380 &     9 &     0 &      0.000 &      0.000 &     0 &       2.02 &          1 &          1 &          1 &          0 &      22.48 &      21.13 &      20.46 &      20.13 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2210 &     9 &     0 &      0.000 &      0.000 &     0 &       3.47 &          1 &          1 &          1 &          0 &      25.19 &      24.52 &      23.65 &      22.75 &       0.18 &       0.06 &       0.04 &       0.02 &          3 \\
    0.3100 &     2 &     1 &      0.079 &      0.790 &     0 &       2.69 &          1 &          1 &          1 &          0 &      21.49 &      19.78 &      18.97 &      18.58 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.21 &          1 &          1 &          9 &          0 &      25.92 &      25.90 &      24.66 &      23.79 &       0.18 &       0.15 &       0.08 &       0.05 &          1 \\
    0.9680 &     9 &     0 &      0.000 &      0.000 &     0 &       2.09 &          1 &          1 &          1 &          0 &      24.60 &      23.77 &      22.96 &      22.55 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1730 &    30 &     0 &      0.000 &      0.000 &     0 &       2.51 &          1 &          1 &          1 &          0 &      25.26 &      24.71 &      23.94 &      23.28 &       0.09 &       0.05 &       0.04 &       0.03 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.15 &          1 &          1 &          1 &          0 &      24.75 &      24.08 &      23.38 &      22.84 &       0.05 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.26 &          1 &          2 &          3 &          0 &      25.49 &      25.01 &      24.37 &      23.87 &       0.05 &       0.03 &       0.03 &       0.02 &          1 \\
    0.6190 &    72 &     0 &      0.000 &      0.000 &     0 &       2.71 &          1 &          1 &          1 &          0 &      24.07 &      22.94 &      22.09 &      21.76 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8160 &     2 &     0 &      0.000 &      0.000 &     0 &       3.90 &          1 &          1 &          1 &          0 &      24.10 &      23.13 &      22.18 &      21.86 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0360 &    30 &     0 &      0.000 &      0.000 &     0 &       2.25 &          1 &          1 &          1 &          0 &      27.46 &      26.06 &      24.25 &      23.48 &       0.60 &       0.14 &       0.05 &       0.02 &          1 \\
    0.6680 &     9 &     0 &      0.000 &      0.000 &     0 &       2.82 &          1 &          1 &         17 &          0 &      22.26 &      21.20 &      20.30 &      20.00 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.93 &          1 &          1 &          9 &          0 &      26.92 &      26.64 &      26.57 &      26.26 &       0.24 &       0.14 &       0.20 &       0.17 &          1 \\
    1.3140 &    30 &     0 &      0.000 &      0.000 &     0 &       1.74 &          1 &          1 &          1 &          0 &      26.80 &      25.54 &      24.16 &      23.06 &       0.49 &       0.13 &       0.06 &       0.03 &          1 \\
    0.9537 &    30 &     0 &      0.000 &      0.000 &     0 &       2.28 &          1 &          1 &          1 &          0 &      24.73 &      23.43 &      21.99 &      21.28 &       0.08 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.46 &          1 &          1 &          1 &          0 &      27.08 &      26.22 &      25.03 &      24.44 &       0.49 &       0.19 &       0.11 &       0.07 &          1 \\
    1.0450 &     9 &     0 &      0.000 &      0.000 &     0 &       4.32 &          1 &          2 &          7 &          0 &      23.70 &      23.26 &      22.63 &      22.13 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.72 &          1 &          1 &          1 &          0 &      26.33 &      24.40 &      23.33 &      22.87 &       0.28 &       0.04 &       0.03 &       0.02 &          1 \\
    0.5373 &    42 &     0 &      0.000 &      0.000 &     0 &       2.15 &          1 &          1 &          1 &          0 &      24.05 &      22.83 &      21.99 &      21.63 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.5700 &    30 &     0 &      0.000 &      0.000 &     0 &       1.86 &          1 &          1 &          1 &          0 &      24.17 &      24.04 &      23.73 &      23.46 &       0.06 &       0.04 &       0.05 &       0.04 &          1 \\
    0.7630 &     9 &     0 &      0.000 &      0.000 &     0 &       2.18 &          2 &          1 &          3 &          0 &      23.04 &      22.55 &      21.92 &      21.72 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3790 &    63 &     0 &      0.000 &      0.000 &     0 &       2.52 &          1 &          1 &          1 &          0 &      25.94 &      25.45 &      24.56 &      23.77 &       0.23 &       0.13 &       0.09 &       0.05 &          1 \\
    1.1120 &    70 &     0 &      0.000 &      0.000 &     0 &       2.61 &          1 &          1 &          1 &          0 &      23.03 &      22.64 &      22.02 &      21.44 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2980 &    30 &     0 &      0.000 &      0.000 &     0 &       2.42 &          1 &          1 &          1 &          0 &      25.71 &      25.47 &      24.80 &      24.16 &       0.07 &       0.05 &       0.05 &       0.03 &          1 \\
    0.3630 &     9 &     1 &      0.070 &      0.000 &     0 &       2.51 &          1 &          1 &          1 &          0 &      22.11 &      21.06 &      20.60 &      20.33 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2290 &     9 &     0 &      0.000 &      0.000 &     0 &       2.28 &          1 &          1 &          1 &          0 &      22.15 &      21.17 &      20.76 &      20.61 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5760 &     9 &     0 &      0.000 &      0.000 &     0 &       9.00 &          1 &          1 &          5 &          0 &      23.42 &      22.34 &      21.48 &      21.12 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5780 &     9 &     0 &      0.000 &      0.000 &     0 &       1.72 &          1 &          1 &          1 &          0 &      24.42 &      22.74 &      21.68 &      21.27 &       0.05 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7310 &     9 &     0 &      0.000 &      0.000 &     0 &       2.83 &          1 &          1 &          1 &          0 &      24.96 &      24.11 &      23.20 &      22.92 &       0.05 &       0.03 &       0.02 &       0.02 &          1 \\
    0.7340 &     9 &     0 &      0.000 &      0.000 &     0 &       2.44 &          1 &          1 &          1 &          0 &      23.00 &      22.21 &      21.41 &      21.17 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0980 &    30 &     0 &      0.000 &      0.000 &     0 &       2.14 &          1 &          1 &          1 &          0 &      26.00 &      25.43 &      24.53 &      23.77 &       0.17 &       0.09 &       0.07 &       0.04 &          1 \\
    0.7260 &     9 &     0 &      0.000 &      0.000 &     0 &       1.58 &          1 &          1 &          1 &          0 &      23.90 &      23.34 &      22.61 &      22.22 &       0.04 &       0.02 &       0.02 &       0.02 &          1 \\
    0.4160 &     9 &     0 &      0.000 &      0.000 &     0 &        NaN &          1 &          1 &          1 &          0 &      21.72 &      20.76 &      20.28 &      20.00 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    1.2200 &    30 &     0 &      0.000 &      0.000 &     0 &       7.22 &          2 &          2 &          7 &          0 &      24.96 &      24.67 &      24.08 &      23.57 &       0.07 &       0.04 &       0.04 &       0.03 &          1 \\
    0.9526 &    42 &     0 &      0.000 &      0.000 &     0 &       6.85 &          1 &          1 &          5 &          0 &      27.47 &      26.36 &      25.85 &      25.69 &       0.51 &       0.11 &       0.12 &       0.11 &          1 \\
    0.4380 &     2 &     1 &      0.096 &      0.000 &     0 &       5.21 &          1 &          2 &          7 &          0 &      22.75 &      21.57 &      20.85 &      20.47 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    1.0000 &     9 &     0 &      0.000 &      0.000 &     0 &       2.75 &          1 &          1 &         17 &          0 &      25.09 &      24.35 &      23.44 &      22.96 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
    0.6650 &     2 &     0 &      0.000 &      0.000 &     0 &       2.36 &          2 &          1 &          3 &          0 &      22.46 &      21.80 &      21.18 &      21.03 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3180 &    30 &     0 &      0.000 &      0.000 &     0 &       3.47 &          1 &          1 &          9 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    0.2130 &     2 &     0 &      0.000 &      0.000 &     0 &       3.23 &          1 &          2 &          3 &          0 &      20.23 &      19.19 &      18.67 &      18.47 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9980 &     9 &     0 &      0.000 &      0.000 &     0 &       1.74 &          1 &          1 &          1 &          0 &      23.53 &      23.11 &      22.44 &      22.07 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    1.4270 &    30 &     0 &      0.000 &      0.000 &     0 &       2.09 &          1 &          1 &          1 &          0 &      25.97 &      25.73 &      25.07 &      24.18 &       0.17 &       0.12 &       0.11 &       0.05 &          1 \\
    0.7370 &    30 &     1 &      0.071 &      0.000 &     0 &       3.36 &          2 &          2 &          3 &          0 &      22.98 &      22.39 &      21.73 &      21.53 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5440 &     9 &     1 &     47.000 &     56.000 &     0 &        NaN &          1 &          1 &          1 &          0 &      19.49 &      19.20 &      18.65 &      18.52 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4560 &     2 &     1 &      0.060 &      0.000 &     0 &       2.31 &          2 &          1 &          3 &          0 &      21.98 &      21.51 &      21.18 &      20.95 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3460 &     2 &     0 &      0.000 &      0.000 &     0 &       3.57 &          1 &          1 &          1 &          0 &      21.68 &      20.78 &      20.50 &      20.32 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9983 &    42 &     0 &      0.000 &      0.000 &     0 &       2.56 &          1 &          1 &          1 &          0 &      22.89 &      22.35 &      21.63 &      21.23 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8400 &     9 &     0 &      0.000 &      0.000 &     1 &        NaN &          2 &          1 &          3 &          0 &      23.67 &      22.80 &      21.82 &      21.46 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3830 &     9 &     0 &      0.000 &      0.000 &     0 &       2.72 &          1 &          1 &          1 &          0 &      25.23 &      24.65 &      23.89 &      23.27 &       0.07 &       0.03 &       0.03 &       0.02 &          1 \\
    1.0970 &     9 &     0 &      0.000 &      0.000 &     0 &       2.99 &          2 &          1 &          3 &          0 &      23.86 &      23.38 &      22.72 &      22.16 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.9980 &    30 &     0 &      0.000 &      0.000 &     0 &       2.21 &          1 &          1 &          1 &          0 &      26.30 &      25.49 &      25.04 &      24.52 &       0.16 &       0.06 &       0.07 &       0.05 &          1 \\
    0.6710 &     9 &     0 &      0.000 &      0.000 &     0 &       3.14 &          1 &          1 &          1 &          0 &      25.33 &      23.82 &      22.68 &      22.24 &       0.12 &       0.02 &       0.01 &       0.01 &          1 \\
    0.7370 &    30 &     0 &      0.000 &      0.000 &     0 &       3.06 &          1 &          1 &          1 &          0 &      25.83 &      23.64 &      22.21 &      21.71 &       0.16 &       0.02 &       0.01 &       0.01 &          2 \\
    0.6684 &    42 &     0 &      0.000 &      0.000 &     0 &       2.39 &          1 &          1 &          1 &          0 &      23.10 &      22.00 &      21.04 &      20.70 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    2.8100 &     2 &     1 &      1.100 &      5.300 &     0 &        NaN &          1 &          1 &          1 &          0 &      21.49 &      20.79 &      20.54 &      20.40 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.86 &          2 &          1 &          3 &          0 &      24.89 &      24.34 &      23.61 &      23.22 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
    0.6540 &     9 &     0 &      0.000 &      0.000 &     0 &        NaN &          1 &          1 &          1 &          0 &      24.91 &      23.44 &      22.40 &      21.96 &       0.06 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7340 &     9 &     0 &      0.000 &      0.000 &     0 &       2.81 &          1 &          1 &          1 &          0 &      25.31 &      24.23 &      23.08 &      22.59 &       0.11 &       0.03 &       0.02 &       0.01 &          1 \\
    0.4166 &     1 &     1 &      0.180 &      0.380 &     0 &       2.44 &          1 &          1 &          1 &          0 &      22.40 &      21.19 &      20.52 &      20.17 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.20 &          1 &          1 &          1 &          0 &      27.67 &      26.57 &      24.77 &      23.86 &       0.47 &       0.17 &       0.06 &       0.03 &          1 \\
    1.1730 &    30 &     0 &      0.000 &      0.000 &     0 &       3.35 &          1 &          1 &          1 &          0 &      25.30 &      24.54 &      23.78 &      23.13 &       0.08 &       0.03 &       0.03 &       0.02 &          1 \\
    0.6690 &     9 &     0 &      0.000 &      0.000 &     0 &       3.50 &          1 &          1 &          1 &          0 &      24.39 &      23.11 &      22.17 &      21.85 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3376 &    42 &     1 &      0.063 &      0.000 &     0 &       3.26 &          2 &          2 &          3 &          0 &      21.26 &      19.86 &      19.18 &      18.82 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       7.33 &          2 &          2 &          7 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    1.1080 &     9 &     0 &      0.000 &      0.000 &     0 &       2.84 &          1 &          1 &          1 &          0 &      23.86 &      23.30 &      22.52 &      21.93 &       0.04 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.78 &          1 &          1 &          1 &          0 &      29.09 &      28.38 &      27.14 &      26.30 &       1.06 &       0.51 &       0.28 &       0.14 &          1 \\
    0.0000 &    42 &     0 &      0.000 &      0.000 &     1 &       3.13 &          1 &          2 &          3 &          0 &      16.17 &      15.80 &      15.41 &      14.95 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.25 &          1 &          1 &          1 &          0 &      24.63 &      24.28 &      23.78 &      23.52 &       0.04 &       0.03 &       0.03 &       0.03 &          1 \\
    1.2450 &    30 &     0 &      0.000 &      0.000 &     0 &       2.53 &          1 &          1 &          1 &          0 &      24.63 &      24.29 &      23.63 &      23.00 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    0.7359 &    42 &     0 &      0.000 &      0.000 &     0 &       4.58 &          1 &          1 &          5 &          0 &      25.52 &      24.45 &      23.70 &      23.42 &       0.08 &       0.03 &       0.02 &       0.02 &          1 \\
    0.6660 &     1 &     0 &      0.000 &      0.000 &     0 &       2.79 &          1 &          1 &          1 &          0 &      22.21 &      21.62 &      20.99 &      20.87 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4570 &     2 &     0 &      0.000 &      0.000 &     0 &       3.56 &          1 &          1 &          1 &          0 &      21.87 &      20.32 &      19.45 &      19.10 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5350 &     9 &     0 &      0.000 &      0.000 &     0 &       2.45 &          1 &          1 &          1 &          0 &      22.84 &      21.89 &      21.23 &      20.99 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2140 &    72 &     0 &      0.000 &      0.000 &     0 &       3.23 &          1 &          1 &          1 &          0 &      20.43 &      19.23 &      18.71 &      18.48 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.47 &          1 &          1 &          9 &          0 &    -999.00 &      28.23 &      27.60 &      27.43 &    -999.00 &       0.29 &       0.28 &       0.28 &          1 \\
    0.5793 &    42 &     0 &      0.000 &      0.000 &     0 &       2.05 &          1 &          1 &          1 &          0 &      22.33 &      21.49 &      20.86 &      20.68 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.45 &          1 &          1 &          1 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          2 \\
    1.4130 &    30 &     0 &      0.000 &      0.000 &     0 &       2.39 &          1 &          1 &          1 &          0 &      29.45 &      26.14 &      24.89 &      23.99 &       6.17 &       0.21 &       0.11 &       0.05 &          1 \\
    3.0640 &     2 &     1 &      0.680 &      5.600 &     0 &       3.22 &          1 &          1 &          1 &          0 &      28.32 &      25.50 &      24.70 &      24.56 &       0.70 &       0.05 &       0.04 &       0.04 &          1 \\
    0.6706 &    42 &     0 &      0.000 &      0.000 &     0 &       4.64 &          1 &          2 &         15 &          0 &      23.52 &      22.74 &      21.99 &      21.74 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.46 &          1 &          2 &          3 &          0 &      23.54 &      22.81 &      21.94 &      21.61 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.26 &          1 &          1 &          1 &          0 &      27.03 &      28.14 &      26.11 &      25.78 &       0.22 &       0.54 &       0.14 &       0.12 &          1 \\
    1.3087 &    42 &     1 &      0.160 &      0.270 &     0 &       2.26 &          1 &          1 &          1 &          0 &      22.43 &      22.22 &      22.02 &      21.63 &       0.01 &       0.01 &       0.01 &       0.01 &          0 \\
    0.3374 &    42 &     0 &      0.000 &      0.000 &     0 &       3.05 &          1 &          1 &          1 &          0 &      22.55 &      21.23 &      20.59 &      20.27 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3800 &    30 &     0 &      0.000 &      0.000 &     0 &       4.31 &          1 &          1 &          5 &          0 &      27.00 &      26.39 &      25.72 &      25.28 &       0.30 &       0.16 &       0.14 &       0.11 &          1 \\
    0.2329 &     1 &     0 &      0.000 &      0.000 &     0 &       1.68 &          1 &          1 &          1 &          0 &      21.93 &      21.10 &      20.69 &      20.57 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.035 &      0.000 &     0 &       3.73 &          1 &          1 &          1 &          0 &      26.34 &      25.78 &      25.07 &      24.50 &       0.16 &       0.08 &       0.07 &       0.05 &          1 \\
    0.6693 &    42 &     0 &      0.000 &      0.000 &     0 &       3.09 &          1 &          1 &          9 &          0 &      24.46 &      23.72 &      22.93 &      22.73 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.29 &          2 &          1 &          3 &          0 &      27.44 &      27.27 &      26.79 &      26.13 &       0.25 &       0.19 &       0.21 &       0.13 &          1 \\
    1.0940 &    30 &     0 &      0.000 &      0.000 &     0 &       2.93 &          1 &          1 &          1 &          0 &      22.75 &      22.12 &      21.30 &      20.60 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.9200 &     2 &     1 &      3.000 &      3.900 &     0 &       1.69 &          1 &          1 &          1 &          0 &      22.42 &      22.90 &      22.68 &      22.70 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    2.5780 &     2 &     1 &      0.043 &      0.500 &     0 &       2.48 &          1 &          1 &          1 &          0 &      25.76 &      25.24 &      24.75 &      24.43 &       0.11 &       0.06 &       0.07 &       0.06 &          1 \\
    1.0380 &    30 &     0 &      0.000 &      0.000 &     0 &       2.77 &          1 &          1 &          1 &          0 &      25.57 &      24.78 &      23.48 &      22.72 &       0.11 &       0.05 &       0.02 &       0.01 &          1 \\
    0.3400 &     2 &     1 &      0.000 &      0.470 &     0 &       3.35 &          1 &          1 &          1 &          0 &      22.09 &      20.33 &      19.52 &      19.19 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.2465 &    42 &     0 &      0.000 &      0.000 &     0 &       1.69 &          1 &          1 &          1 &          0 &      24.43 &      24.24 &      23.95 &      23.33 &       0.04 &       0.03 &       0.04 &       0.02 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.51 &          1 &          1 &          1 &          0 &      24.51 &      23.59 &      22.73 &      22.43 &       0.05 &       0.02 &       0.02 &       0.01 &          1 \\
    1.1200 &    30 &     0 &      0.000 &      0.000 &     0 &       3.64 &          2 &          1 &          3 &          0 &      26.12 &      27.58 &      24.94 &      23.93 &       0.23 &       0.68 &       0.10 &       0.04 &          0 \\
    0.5470 &     2 &     1 &      0.120 &      0.000 &     0 &       2.49 &          1 &          1 &          1 &          0 &      22.76 &      21.47 &      20.63 &      20.25 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7329 &    42 &     0 &      0.000 &      0.000 &     0 &       2.54 &          1 &          1 &          1 &          0 &      24.93 &      23.39 &      22.05 &      21.54 &       0.11 &       0.02 &       0.01 &       0.01 &          1 \\
    0.6801 &    42 &     0 &      0.000 &      0.000 &     0 &       2.32 &          1 &          1 &          1 &          0 &      24.29 &      22.89 &      21.83 &      21.45 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5780 &    72 &     1 &      0.049 &      0.000 &     0 &       2.43 &          1 &          1 &          1 &          0 &      22.98 &      22.09 &      21.41 &      21.17 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6640 &     2 &     1 &      0.087 &      0.000 &     0 &       3.11 &          2 &          1 &          3 &          0 &      23.56 &      21.92 &      20.68 &      20.23 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5420 &    70 &     0 &      0.000 &      0.000 &     0 &       2.21 &          1 &          1 &          1 &          0 &      22.61 &      21.80 &      21.25 &      21.11 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2149 &     1 &     0 &      0.000 &      0.000 &     0 &       2.78 &          1 &          1 &          1 &          0 &      20.17 &      19.23 &      18.85 &      18.71 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    1.2198 &    42 &     0 &      0.000 &      0.000 &     0 &       2.98 &          1 &          1 &          9 &          0 &      24.17 &      24.05 &      23.45 &      22.74 &       0.05 &       0.04 &       0.03 &       0.02 &          2 \\
    0.2410 &     2 &     1 &      0.047 &      0.000 &     0 &       2.60 &          1 &          1 &          1 &          0 &      21.96 &      20.63 &      19.93 &      19.62 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4590 &     2 &     0 &      0.000 &      0.000 &     0 &       2.70 &          1 &          1 &          1 &          0 &      22.57 &      21.31 &      20.63 &      20.34 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7358 &    42 &     0 &      0.000 &      0.000 &     0 &       2.44 &          1 &          1 &          1 &          0 &      22.99 &      22.16 &      21.41 &      21.17 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6713 &    42 &     0 &      0.000 &      0.000 &     0 &       2.85 &          1 &          1 &          1 &          0 &      23.15 &      21.62 &      20.47 &      20.05 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7340 &     2 &     1 &      0.063 &      0.500 &     0 &       1.94 &          1 &          1 &          1 &          0 &      25.84 &      24.06 &      22.63 &      22.05 &       0.16 &       0.03 &       0.01 &       0.01 &          1 \\
    1.0960 &    30 &     0 &      0.000 &      0.000 &     0 &       3.72 &          2 &          1 &          3 &          0 &      26.02 &      25.48 &      24.22 &      23.68 &       0.21 &       0.13 &       0.07 &       0.05 &          2 \\
    1.6190 &    30 &     0 &      0.000 &      0.000 &     0 &       2.62 &          2 &          1 &          3 &          0 &      24.90 &      24.48 &      23.81 &      23.35 &       0.07 &       0.04 &       0.04 &       0.03 &          1 \\
    0.8534 &    42 &     0 &      0.000 &      0.000 &     0 &       2.19 &          1 &          1 &          1 &          0 &      23.61 &      22.88 &      22.04 &      21.74 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.6160 &    30 &     0 &      0.000 &      0.000 &     0 &       2.84 &          1 &          1 &          1 &          0 &      26.05 &      26.45 &      24.97 &      24.11 &       0.28 &       0.30 &       0.13 &       0.07 &          1 \\
    0.6880 &    72 &     0 &      0.000 &      0.000 &     0 &       2.47 &          2 &          1 &          3 &          0 &      22.98 &      22.31 &      21.61 &      21.46 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.95 &          1 &          1 &          1 &          0 &      23.59 &      22.98 &      22.25 &      21.87 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6676 &    42 &     0 &      0.000 &      0.000 &     0 &       2.57 &          1 &          1 &          1 &          0 &      22.32 &      21.62 &      20.90 &      20.69 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1400 &    30 &     0 &      0.000 &      0.000 &     0 &       2.50 &          1 &          1 &          1 &          0 &      25.88 &      25.18 &      24.43 &      23.59 &       0.14 &       0.06 &       0.05 &       0.03 &          2 \\
    0.8528 &    42 &     1 &      0.045 &      0.000 &     0 &       2.16 &          1 &          1 &          1 &          0 &      22.39 &      21.95 &      21.33 &      21.12 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0950 &    30 &     1 &      0.030 &      0.000 &     0 &       2.65 &          1 &          1 &          1 &          0 &      23.21 &      22.69 &      22.04 &      21.56 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5590 &    30 &     0 &      0.000 &      0.000 &     0 &       2.55 &          1 &          1 &          1 &          0 &      22.24 &      21.42 &      20.75 &      20.52 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5780 &    11 &     0 &      0.000 &      0.000 &     0 &       3.38 &          1 &          1 &          1 &          0 &      21.41 &      20.58 &      19.92 &      19.71 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.6130 &    30 &     0 &      0.000 &      0.000 &     0 &       3.22 &          1 &          1 &          1 &          0 &      26.36 &      25.60 &      24.53 &      23.94 &       0.27 &       0.12 &       0.07 &       0.05 &          1 \\
    1.3840 &    30 &     0 &      0.000 &      0.000 &     0 &       2.49 &          1 &          1 &          1 &          0 &      24.03 &      23.84 &      23.39 &      22.79 &       0.05 &       0.03 &       0.03 &       0.02 &          1 \\
    0.6700 &    30 &     1 &      0.058 &      0.000 &     0 &       2.58 &          1 &          1 &          1 &          0 &      23.74 &      22.39 &      21.30 &      20.85 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    1.6150 &    81 &     1 &      0.000 &      0.760 &     0 &       3.10 &          1 &          1 &          1 &          0 &      25.65 &      25.37 &      24.34 &      23.78 &       0.16 &       0.12 &       0.07 &       0.05 &          1 \\
    1.0970 &    30 &     0 &      0.000 &      0.000 &     0 &       2.90 &          1 &          1 &          1 &          0 &      23.91 &      23.08 &      22.16 &      21.43 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0150 &    30 &     0 &      0.000 &      0.000 &     0 &       2.48 &          2 &          1 &          3 &          0 &      23.34 &      22.69 &      21.83 &      21.21 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
    0.8410 &    30 &     0 &      0.000 &      0.000 &     0 &       2.39 &          1 &          1 &          1 &          0 &      23.15 &      22.78 &      22.24 &      22.01 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.1285 &    42 &     0 &      0.000 &      0.000 &     0 &       2.62 &          1 &          1 &          1 &          0 &      20.38 &      18.96 &      18.36 &      18.06 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.1239 &     1 &     0 &      0.000 &      0.000 &     0 &       3.24 &          1 &          1 &          1 &          1 &      20.40 &      19.10 &      18.44 &      18.11 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5147 &    42 &     0 &      0.000 &      0.000 &     0 &       1.56 &          1 &          1 &          1 &          0 &      24.60 &      23.01 &      22.00 &      21.58 &       0.05 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9910 &    30 &     0 &      0.000 &      0.000 &     0 &       2.93 &          1 &          1 &          9 &          0 &      25.87 &      24.94 &      23.94 &      23.55 &       0.08 &       0.03 &       0.02 &       0.02 &          1 \\
    1.2240 &    30 &     0 &      0.000 &      0.000 &     0 &       2.56 &          1 &          1 &          1 &          0 &      25.13 &      24.17 &      23.04 &      22.14 &       0.09 &       0.03 &       0.02 &       0.01 &          1 \\
    0.0010 &    42 &     0 &      0.000 &      0.000 &     1 &       2.08 &          1 &          1 &          1 &          0 &      18.35 &      17.35 &      16.49 &      15.68 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7350 &    30 &     0 &      0.000 &      0.000 &     0 &       3.08 &          1 &          1 &          1 &          0 &      25.77 &      24.02 &      22.56 &      22.06 &       0.12 &       0.02 &       0.01 &       0.01 &          2 \\
    1.2220 &    30 &     0 &      0.000 &      0.000 &     0 &       2.60 &          2 &          1 &          3 &          0 &      24.94 &      24.28 &      23.61 &      22.73 &       0.07 &       0.04 &       0.03 &       0.02 &          1 \\
    1.0020 &    30 &     0 &      0.000 &      0.000 &     0 &       3.43 &          1 &          2 &          3 &          0 &      23.89 &      22.88 &      21.85 &      21.22 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6711 &    42 &     0 &      0.000 &      0.000 &     0 &       2.59 &          1 &          1 &          1 &          0 &      23.32 &      22.41 &      21.45 &      21.10 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3592 &     1 &     0 &      0.000 &      0.000 &     0 &       3.23 &          1 &          1 &          1 &          0 &      21.71 &      20.72 &      20.30 &      20.04 &       0.01 &       0.01 &       0.01 &       0.01 &          0 \\
    1.2270 &     2 &     1 &      2.900 &      4.600 &     0 &       6.13 &          1 &          2 &         15 &          0 &      23.66 &      22.90 &      22.36 &      21.87 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.28 &          2 &          1 &          3 &          0 &      25.98 &      25.46 &      24.76 &      24.01 &       0.13 &       0.07 &       0.06 &       0.04 &          1 \\
    0.7350 &    30 &     0 &      0.000 &      0.000 &     0 &       2.15 &          1 &          1 &          9 &          0 &      24.48 &      23.16 &      21.84 &      21.39 &       0.06 &       0.02 &       0.01 &       0.01 &          2 \\
    0.9045 &     1 &     0 &      0.000 &      0.000 &     0 &       3.14 &          1 &          1 &          1 &          0 &      23.61 &      23.14 &      22.28 &      21.92 &       0.02 &       0.01 &       0.01 &       0.01 &          0 \\
    0.5230 &    72 &     0 &      0.000 &      0.000 &     0 &       2.95 &          1 &          1 &          1 &          0 &      22.84 &      21.80 &      21.00 &      20.58 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6461 &    42 &     0 &      0.000 &      0.000 &     0 &       4.14 &          1 &          2 &          7 &          0 &      24.39 &      22.83 &      21.68 &      21.24 &       0.05 &       0.01 &       0.01 &       0.01 &          2 \\
    0.7362 &    42 &     0 &      0.000 &      0.000 &     0 &       1.89 &          2 &          1 &          3 &          0 &      22.96 &      22.17 &      21.29 &      21.03 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.340 &      0.840 &     0 &       3.41 &          1 &          1 &          1 &          0 &      26.70 &      26.09 &      24.92 &      24.09 &       0.26 &       0.13 &       0.07 &       0.04 &          1 \\
    0.2734 &     1 &     1 &      0.490 &      0.000 &     0 &       3.06 &          2 &          2 &          3 &          0 &      21.67 &      20.19 &      19.48 &      19.17 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2790 &     2 &     0 &      0.000 &      0.000 &     0 &       6.38 &          2 &          2 &          7 &          0 &      21.17 &      19.62 &      18.86 &      18.50 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6792 &    42 &     0 &      0.000 &      0.000 &     0 &       2.61 &          2 &          1 &          3 &          0 &      22.12 &      21.40 &      20.70 &      20.53 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9640 &    30 &     0 &      0.000 &      0.000 &     0 &       0.63 &          1 &          1 &          5 &          0 &      24.70 &      24.19 &      23.37 &      22.99 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
    0.6733 &    42 &     0 &      0.000 &      0.000 &     0 &       3.00 &          1 &          1 &          1 &          0 &      22.64 &      21.78 &      21.01 &      20.76 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4130 &    70 &     0 &      0.000 &      0.000 &     0 &       2.69 &          1 &          1 &          1 &          0 &      21.91 &      21.18 &      20.82 &      20.62 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.34 &          1 &          1 &          1 &          0 &      24.04 &      22.42 &      21.61 &      21.23 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1010 &    72 &     0 &      0.000 &      0.000 &     0 &       2.48 &          1 &          1 &          1 &          0 &      23.42 &      22.98 &      22.32 &      21.82 &       0.04 &       0.02 &       0.02 &       0.01 &          1 \\
    1.1230 &    30 &     0 &      0.000 &      0.000 &     0 &       3.13 &          2 &          2 &          3 &          0 &      24.98 &      24.18 &      23.35 &      22.66 &       0.05 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       4.92 &          1 &          1 &          5 &          0 &      24.75 &      24.35 &      23.79 &      23.15 &       0.06 &       0.04 &       0.04 &       0.02 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.07 &          1 &          1 &          1 &          0 &      25.84 &      24.35 &      23.01 &      22.52 &       0.12 &       0.03 &       0.01 &       0.01 &          1 \\
    0.7620 &    30 &     0 &      0.000 &      0.000 &     0 &       3.26 &          1 &          1 &          1 &          0 &      24.51 &      23.18 &      21.78 &      21.25 &       0.06 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4143 &     1 &     0 &      0.000 &      0.000 &     0 &       2.08 &          1 &          1 &          1 &          0 &      23.04 &      21.82 &      21.16 &      20.84 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5300 &    72 &     0 &      0.000 &      0.000 &     0 &       1.95 &          1 &          1 &          1 &          0 &      23.48 &      22.38 &      21.63 &      21.32 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.6030 &     2 &     1 &      5.600 &      7.400 &     0 &       2.56 &          1 &          2 &          3 &          0 &      25.23 &      24.81 &      24.14 &      23.50 &       0.05 &       0.03 &       0.03 &       0.02 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.86 &          3 &          1 &          3 &          0 &      24.90 &      24.17 &      23.31 &      22.84 &       0.07 &       0.03 &       0.02 &       0.02 &          1 \\
    1.0970 &     2 &     1 &      0.400 &     14.000 &     0 &       2.66 &          1 &          1 &          1 &          0 &      24.80 &      23.81 &      22.64 &      21.77 &       0.06 &       0.02 &       0.01 &       0.01 &          2 \\
    1.1020 &    72 &     0 &      0.000 &      0.000 &     0 &       3.59 &          2 &          1 &         11 &          0 &      25.47 &      24.52 &      23.54 &      22.84 &       0.12 &       0.05 &       0.03 &       0.02 &          1 \\
    0.3430 &     2 &     0 &      0.000 &      0.000 &     0 &       2.68 &          1 &          1 &          1 &          0 &      21.98 &      20.82 &      20.20 &      19.81 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7610 &    30 &     0 &      0.000 &      0.000 &     0 &       2.45 &          1 &          1 &          1 &          0 &      24.78 &      23.63 &      22.29 &      21.82 &       0.07 &       0.02 &       0.01 &       0.01 &          1 \\
    0.7396 &    42 &     1 &      0.039 &      0.000 &     0 &       2.80 &          1 &          1 &          1 &          0 &      23.96 &      23.20 &      22.48 &      22.21 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.057 &      0.000 &     0 &       2.90 &          1 &          1 &          1 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\
    0.7550 &    70 &     0 &      0.000 &      0.000 &     0 &       2.30 &          1 &          1 &          1 &          0 &      23.10 &      22.47 &      21.59 &      21.36 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0980 &    30 &     0 &      0.000 &      0.000 &     0 &       2.86 &          1 &          1 &          1 &          0 &      23.76 &      22.93 &      21.93 &      21.18 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1580 &    30 &     0 &      0.000 &      0.000 &     0 &       3.75 &          2 &          2 &          3 &          0 &      25.61 &      24.95 &      23.94 &      23.06 &       0.14 &       0.07 &       0.05 &       0.03 &          1 \\
    0.3311 &     1 &     0 &      0.000 &      0.000 &     0 &       2.73 &          1 &          1 &          1 &          0 &      21.96 &      20.83 &      20.33 &      20.06 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.7062 &    42 &     0 &      0.000 &      0.000 &     0 &       2.52 &          1 &          1 &          9 &          0 &      24.77 &      23.26 &      22.04 &      21.54 &       0.06 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0459 &    42 &     0 &      0.000 &      0.000 &     0 &       1.39 &          2 &          1 &          3 &          0 &      24.01 &      23.62 &      22.86 &      22.41 &       0.03 &       0.02 &       0.02 &       0.02 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.97 &          1 &          1 &          1 &          0 &      25.55 &      24.73 &      23.57 &      22.74 &       0.11 &       0.05 &       0.03 &       0.02 &          1 \\
    0.3669 &    42 &     0 &      0.000 &      0.000 &     0 &       3.25 &          1 &          2 &          3 &          0 &      23.98 &      22.39 &      21.54 &      21.12 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.07 &          2 &          1 &          3 &          0 &      25.51 &      24.82 &      23.82 &      23.16 &       0.12 &       0.06 &       0.04 &       0.03 &          1 \\
    0.5608 &    42 &     0 &      0.000 &      0.000 &     0 &       2.05 &          1 &          1 &          1 &          0 &      24.58 &      23.13 &      22.20 &      21.86 &       0.05 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1030 &    72 &     0 &      0.000 &      0.000 &     0 &       4.27 &          2 &          2 &          7 &          0 &      23.31 &      22.83 &      22.11 &      21.46 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    3.4742 &    42 &     0 &      0.000 &      0.000 &     0 &       3.66 &          1 &          1 &          9 &          0 &      26.48 &      24.07 &      22.80 &      22.40 &       0.17 &       0.02 &       0.01 &       0.01 &          1 \\
    1.0189 &    42 &     0 &      0.000 &      0.000 &     0 &       1.98 &          1 &          1 &          1 &          0 &      24.83 &      24.11 &      23.25 &      22.74 &       0.05 &       0.03 &       0.02 &       0.01 &          1 \\
    0.6670 &     1 &     1 &      0.500 &      2.100 &     0 &       3.33 &          1 &          1 &          9 &          0 &      23.71 &      21.64 &      20.32 &      19.91 &       0.05 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6451 &     1 &     0 &      0.000 &      0.000 &     0 &       4.06 &          1 &          2 &          7 &          0 &      24.04 &      22.94 &      22.14 &      21.86 &       0.03 &       0.01 &       0.01 &       0.01 &          2 \\
    0.6480 &     2 &     0 &      0.000 &      0.000 &     0 &       5.00 &          1 &          2 &          7 &          0 &      22.24 &      21.76 &      21.27 &      21.25 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.44 &          1 &          1 &          9 &          0 &      23.58 &      23.29 &      22.79 &      22.38 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6459 &    42 &     0 &      0.000 &      0.000 &     0 &       3.49 &          1 &          1 &          1 &          0 &      23.77 &      22.60 &      21.77 &      21.47 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0170 &    30 &     0 &      0.000 &      0.000 &     0 &       4.22 &          1 &          1 &          5 &          0 &      25.51 &      24.67 &      23.59 &      22.97 &       0.08 &       0.04 &       0.02 &       0.01 &          2 \\
    0.9795 &    42 &     0 &      0.000 &      0.000 &     0 &       2.92 &          1 &          1 &          1 &          0 &      23.49 &      23.04 &      22.21 &      21.81 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
    0.3660 &     2 &     1 &      0.200 &      0.000 &     0 &       3.18 &          2 &          1 &          3 &          0 &      20.57 &      20.14 &      20.27 &      19.92 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1070 &    30 &     0 &      0.000 &      0.000 &     0 &       2.67 &          2 &          1 &          3 &          0 &      23.31 &      22.92 &      22.35 &      21.96 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1013 &    42 &     0 &      0.000 &      0.000 &     0 &       2.56 &          1 &          1 &          1 &          0 &      22.88 &      22.53 &      21.98 &      21.59 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5320 &    30 &     0 &      0.000 &      0.000 &     0 &       2.86 &          2 &          1 &          3 &          0 &      23.52 &      21.83 &      20.81 &      20.43 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.19 &          2 &          1 &          3 &          0 &      25.79 &      25.29 &      25.06 &      24.63 &       0.16 &       0.08 &       0.10 &       0.08 &          1 \\
    1.3820 &    30 &     0 &      0.000 &      0.000 &     0 &       2.92 &          1 &          2 &          3 &          0 &      26.14 &      25.82 &      24.68 &      23.57 &       0.26 &       0.17 &       0.10 &       0.04 &          1 \\
    0.9830 &    30 &     0 &      0.000 &      0.000 &     0 &       2.52 &          1 &          1 &          1 &          0 &      23.44 &      22.83 &      21.99 &      21.49 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8330 &    30 &     0 &      0.000 &      0.000 &     0 &       2.75 &          1 &          2 &          3 &          0 &      24.17 &      23.26 &      21.86 &      21.18 &       0.06 &       0.02 &       0.01 &       0.01 &          1 \\
    0.6704 &    42 &     0 &      0.000 &      0.000 &     0 &       5.21 &          2 &          2 &          7 &          0 &      25.62 &      24.14 &      23.00 &      22.62 &       0.11 &       0.03 &       0.02 &       0.01 &          1 \\
    0.2810 &    30 &     0 &      0.000 &      0.000 &     0 &       2.33 &          1 &          1 &          1 &          0 &      22.93 &      22.15 &      21.75 &      21.41 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       1.55 &          1 &          1 &          1 &          0 &      24.63 &      23.95 &      23.19 &      22.42 &       0.03 &       0.02 &       0.01 &       0.01 &          1 \\
    0.9720 &    70 &     0 &      0.000 &      0.000 &     0 &       2.39 &          1 &          1 &          1 &          0 &      23.79 &      23.15 &      22.36 &      22.02 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4040 &    42 &     0 &      0.000 &      0.000 &     0 &       3.17 &          1 &          1 &          1 &          0 &      22.56 &      21.50 &      20.98 &      20.69 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5620 &    72 &     0 &      0.000 &      0.000 &     0 &       2.78 &          1 &          1 &          1 &          0 &      24.12 &      22.32 &      21.39 &      21.10 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.18 &          1 &          1 &          1 &          0 &      19.95 &      19.04 &      18.62 &      18.44 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       3.32 &          1 &          1 &          1 &          0 &      23.26 &      22.87 &      22.15 &      21.59 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     1 &       2.85 &          1 &          1 &          1 &          0 &      15.99 &      15.62 &      15.19 &      14.71 &       0.01 &       0.20 &       0.01 &       0.01 &          0 \\
    0.8233 &    42 &     0 &      0.000 &      0.000 &     0 &       4.91 &          1 &          2 &          7 &          0 &      24.15 &      23.26 &      22.35 &      22.04 &       0.03 &       0.01 &       0.01 &       0.01 &          2 \\
    0.6508 &     1 &     0 &      0.000 &      0.000 &     0 &       2.75 &          2 &          1 &          3 &          0 &      22.71 &      21.85 &      21.09 &      20.87 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     1 &       2.40 &          1 &          1 &          1 &          0 &      18.31 &      17.56 &      16.36 &      15.61 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.3430 &    30 &     0 &      0.000 &      0.000 &     0 &       4.28 &          1 &          1 &          5 &          0 &      24.70 &      24.32 &      23.71 &      23.01 &       0.07 &       0.03 &       0.03 &       0.02 &          1 \\
    1.0880 &    30 &     0 &      0.000 &      0.000 &     0 &       3.25 &          1 &          2 &          3 &          0 &      24.19 &      23.51 &      22.69 &      22.08 &       0.04 &       0.02 &       0.02 &       0.01 &          0 \\
    0.8240 &    72 &     0 &      0.000 &      0.000 &     0 &       2.67 &          1 &          1 &          1 &          0 &      25.06 &      24.27 &      23.35 &      23.12 &       0.09 &       0.03 &       0.02 &       0.02 &          1 \\
    1.2950 &    30 &     0 &      0.000 &      0.000 &     0 &       2.64 &          1 &          1 &          1 &          0 &      25.44 &      24.59 &      23.33 &      22.18 &       0.19 &       0.08 &       0.04 &       0.02 &          1 \\
    0.2810 &    30 &     0 &      0.000 &      0.000 &     0 &       2.81 &          1 &          1 &          1 &          0 &      21.20 &      20.27 &      19.92 &      19.74 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8409 &     1 &     0 &      0.000 &      0.000 &     0 &       2.54 &          1 &          1 &          1 &          0 &      23.14 &      22.36 &      21.39 &      21.06 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6640 &     2 &     1 &      0.270 &      1.000 &     0 &       2.69 &          1 &          1 &          1 &          0 &      23.07 &      21.28 &      20.01 &      19.58 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2031 &    42 &     0 &      0.000 &      0.000 &     0 &       2.93 &          1 &          1 &          1 &          0 &      20.82 &      19.76 &      19.26 &      19.05 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3155 &    42 &     0 &      0.000 &      0.000 &     0 &       3.88 &          1 &          1 &          1 &          0 &      22.21 &      20.82 &      20.24 &      20.01 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4039 &    42 &     0 &      0.000 &      0.000 &     0 &       2.13 &          2 &          1 &          3 &          0 &      23.53 &      22.11 &      21.36 &      21.00 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6479 &    42 &     0 &      0.000 &      0.000 &     0 &       2.30 &          1 &          1 &          9 &          0 &      23.43 &      22.63 &      21.98 &      21.82 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.1256 &     1 &     0 &      0.000 &      0.000 &     0 &       3.31 &          1 &          1 &          1 &          0 &      20.14 &      19.33 &      18.94 &      18.80 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.5610 &    72 &     0 &      0.000 &      0.000 &     0 &       2.92 &          1 &          1 &          1 &          0 &      23.60 &      22.23 &      21.28 &      20.91 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    0.2021 &    41 &     1 &      0.093 &      0.000 &     0 &       2.49 &          1 &          1 &          1 &          0 &      20.49 &      19.67 &      19.27 &      19.17 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.1232 &     1 &     0 &      0.000 &      0.000 &     0 &       2.69 &          1 &          1 &          1 &          0 &      20.39 &      19.55 &      19.10 &      18.92 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.4584 &     1 &     1 &      0.170 &      0.000 &     0 &       3.08 &          1 &          1 &          1 &          1 &      20.86 &      19.88 &      19.31 &      19.00 &       0.01 &       0.01 &       0.01 &       0.01 &          2 \\
    0.6590 &    70 &     0 &      0.000 &      0.000 &     0 &       2.45 &          1 &          1 &          1 &          0 &      22.18 &      21.58 &      21.06 &      20.94 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3830 &    30 &     0 &      0.000 &      0.000 &     0 &       1.75 &          1 &          1 &          1 &          0 &      24.00 &      22.23 &      21.34 &      20.92 &       0.03 &       0.01 &       0.01 &       0.01 &          1 \\
    0.8390 &     2 &     1 &      1.600 &      2.900 &     0 &       3.37 &          1 &          1 &          1 &          0 &      23.78 &      23.14 &      22.20 &      21.80 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.9780 &    30 &     0 &      0.000 &      0.000 &     0 &       2.37 &          1 &          1 &          1 &          0 &      23.44 &      22.55 &      21.56 &      21.04 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0361 &    42 &     0 &      0.000 &      0.000 &     0 &       2.47 &          1 &          1 &          1 &          0 &      23.33 &      22.77 &      22.08 &      21.69 &       0.02 &       0.01 &       0.01 &       0.01 &          1 \\
    0.1249 &     1 &     0 &      0.000 &      0.000 &     0 &       3.24 &          1 &          2 &         11 &          0 &      20.37 &      19.75 &      19.46 &      19.37 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.3661 &     1 &     0 &      0.000 &      0.000 &     0 &       5.56 &          1 &          2 &          7 &          0 &      22.37 &      21.51 &      21.18 &      20.94 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.79 &          1 &          1 &          1 &          0 &      27.23 &      25.80 &      24.77 &      24.14 &       0.49 &       0.13 &       0.08 &       0.05 &          1 \\
    0.1273 &    41 &     0 &      0.000 &      0.000 &     0 &       2.67 &          1 &          1 &          1 &          0 &      20.42 &      19.59 &      19.16 &      19.00 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.35 &          1 &          1 &          1 &          0 &      23.96 &      22.66 &      21.56 &      21.17 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    1.0363 &     1 &     0 &      0.000 &      0.000 &     0 &       2.58 &          1 &          1 &          9 &          0 &      23.89 &      23.47 &      22.78 &      22.28 &       0.03 &       0.02 &       0.02 &       0.01 &          1 \\
    0.0380 &     2 &     1 &      0.140 &      0.310 &     0 &       4.69 &          1 &          1 &          5 &          1 &      17.74 &      16.65 &      16.06 &      15.71 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    1.1460 &    30 &     0 &      0.000 &      0.000 &     0 &       2.88 &          1 &          1 &          1 &          0 &      24.64 &      23.94 &      23.15 &      22.45 &       0.06 &       0.03 &       0.02 &       0.01 &          1 \\
    0.6596 &    42 &     0 &      0.000 &      0.000 &     0 &       3.00 &          1 &          1 &          1 &          0 &      22.29 &      21.40 &      20.66 &      20.40 &       0.04 &       0.01 &       0.01 &       0.01 &          1 \\
    1.4690 &    30 &     0 &      0.000 &      0.000 &     0 &       4.87 &          2 &          1 &          7 &          0 &      24.15 &      23.54 &      22.75 &      22.31 &       0.05 &       0.03 &       0.02 &       0.02 &          2 \\
    0.6660 &    30 &     0 &      0.000 &      0.000 &     0 &       3.05 &          1 &          1 &          1 &          0 &      22.79 &      22.06 &      21.39 &      21.23 &       0.01 &       0.01 &       0.01 &       0.01 &          1 \\
    0.6620 &    72 &     0 &      0.000 &      0.000 &     0 &       2.89 &          1 &          1 &          1 &          0 &      24.14 &      23.04 &      21.94 &      21.55 &       0.05 &       0.02 &       0.01 &       0.01 &          1 \\
  -99.0000 &    -1 &     1 &      0.530 &      6.700 &     0 &       3.09 &          1 &          1 &          1 &          0 &      27.95 &      26.17 &      25.41 &      25.35 &       0.47 &       0.11 &       0.09 &       0.10 &          1 \\
  -99.0000 &    -1 &     0 &      0.000 &      0.000 &     0 &       2.93 &          2 &          1 &          3 &          0 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &    -999.00 &          1 \\

